Strongly Tail-Optimal Scheduling in the Light-Tailed M/G/1

We study the problem of scheduling jobs in a queueing system, specifically an M/G/1 with light-tailed job sizes, to asymptotically optimize the response time tail. This means scheduling to make $\mathbf{P}[T > t]$, the chance a job's response time exceeds $t$, decay as quickly as possible in the $t \to \infty$ limit. For some time, the best known policy was First-Come First-Served (FCFS), which has an asymptotically exponential tail: $\mathbf{P}[T > t] \sim C e^{-\gamma t}$. FCFS achieves the optimal *decay rate* $\gamma$, but its *tail constant* $C$ is suboptimal. Only recently have policies that improve upon FCFS's tail constant been discovered. But it is unknown what the optimal tail constant is, let alone what policy might achieve it. In this paper, we derive a closed-form expression for the optimal tail constant $C$, and we introduce *$\gamma$-Boost*, a new policy that achieves this optimal tail constant. Roughly speaking, $\gamma$-Boost operates similarly to FCFS, but it pretends that small jobs arrive earlier than their true arrival times. This significantly reduces the response time of small jobs without unduly delaying large jobs, improving upon FCFS's tail constant by up to 50% with only moderate job size variability, with even larger improvements for higher variability. While these results are for systems with full job size information, we also introduce and analyze a version of $\gamma$-Boost that works in settings with partial job size information, showing it too achieves significant gains over FCFS. Finally, we show via simulation that $\gamma$-Boost has excellent practical performance.

==> ACM-ish-short.tex <==
%%% -*-BibTeX-*-
%%% ====================================================================
%%%  @BibTeX-style-file{
%%%     author          = "Nelson H. F. Beebe, Boris Veytsman and Gerald Murray",
%%%     version         = "2.1",
%%%     acmart-version  = "1.79",
%%%     date            = "14 June 2017",
%%%     filename        = "ACM-Reference-Format.bst",
%%%     email           = "borisv@lk.net, boris@varphi.com",
%%%     codetable       = "ISO/ASCII",
%%%     keywords        = "ACM Transactions bibliography style; BibTeX",
%%%     license         = "public domain",
%%%     supported       = "yes",
%%%     abstract        = "",
%%%  }
%%% ====================================================================

%%% Revision history:  see source in git

ENTRY
  { address
    advisor
    archiveprefix
    author
    booktitle
    chapter
    city
    date
    edition
    editor
    eprint
    eprinttype
    eprintclass
    howpublished
    institution
    journal
    key
    location
    month
    note
    number
    organization
    pages
    primaryclass
    publisher
    school
    series
    title
    type
    volume
    year
        % New keys recognized
        issue         % UTAH: used in, e.g., ACM SIGSAM Bulletin and ACM Communications in Computer Algebra
        articleno
        eid
        day           % UTAH: needed for newspapers, weeklies, bi-weeklies
        doi           % UTAH
        url           % UTAH
        bookpages     % UTAH
        numpages
        lastaccessed  % UTAH: used only for @Misc{...}
        coden         % UTAH
        isbn          % UTAH
        isbn-13       % UTAH
        issn          % UTAH
        lccn          % UTAH
  }
  {}
  { label.year extra.label sort.year sort.label basic.label.year}

INTEGERS { output.state before.all mid.sentence after.sentence after.block }

INTEGERS { show-isbn-10-and-13 }  % initialized below in begin.bib

INTEGERS { nameptr namesleft numnames }

INTEGERS { multiresult }

INTEGERS { len }

INTEGERS { last.extra.num }

STRINGS { s t t.org u }

STRINGS { last.label next.extra }

STRINGS { p1 p2 p3 page.count }


FUNCTION { not }
{
    { #0 }
    { #1 }
  if$
}

FUNCTION { and }
{
    'skip$
    { pop$ #0 }
  if$
}

FUNCTION { or }
{
   { pop$ #1 }
    'skip$
  if$
}


FUNCTION { dump.stack.1 }
{
    duplicate$ "STACK[top] = [" swap$ * "]" * warning$
}

FUNCTION { dump.stack.2 }
{
    duplicate$ "STACK[top  ] = [" swap$ * "]" * warning$
    swap$
    duplicate$ "STACK[top-1] = [" swap$ * "]" * warning$
    swap$
}

FUNCTION { empty.or.unknown }
{
  %% Examine the top stack entry, and push 1 if it is empty, or
  %% consists only of whitespace, or is a string beginning with two
  %% queries (??), and otherwise, push 0.
  %%
  %% This function provides a replacement for empty$, with the
  %% convenient feature that unknown values marked by two leading
  %% queries are treated the same as missing values, and thus, do not
  %% appear in the output .bbl file, and yet, their presence in .bib
  %% file(s) serves to mark values which are temporarily missing, but
  %% are expected to be filled in eventually once more data is
  %% obtained.  The TeX User Group and BibNet bibliography archives
  %% make extensive use of this practice.
  %%
  %% An empty string cannot serve the same purpose, because just as in
  %% statistics data processing, an unknown value is not the same as an
  %% empty value.
  %%
  %% At entry: stack = ... top:[string]
  %% At exit:  stack = ... top:[0 or 1]

  duplicate$ empty$
    { pop$ #1 }
    { #1 #2 substring$ "??" = }
  if$
}

FUNCTION { writeln }
{
  %% In BibTeX style files, the sequences
  %%
  %%     ... "one" "two" output
  %%     ... "one" "two" output.xxx
  %%
  %% ship "one" to the output file, possibly following by punctuation,
  %% leaving the stack with
  %%
  %%     ... "two"
  %%
  %% There is thus a one-string lag in output processing that must be
  %% carefully handled to avoid duplicating a string in the output
  %% file.  Unless otherwise noted, all output.xxx functions leave
  %% just one new string on the stack, and that model should be born
  %% in mind when reading or writing function code.
  %%
  %% BibTeX's asynchronous buffering of output from strings from the
  %% stack is confusing because newline$ bypasses the buffer.  It
  %% would have been so much easier for newline to be a character
  %% rather than a state of the output-in-progress.
  %%
  %% The documentation in btxhak.dvi is WRONG:  it says
  %%
  %%    newline$ Writes onto the bbl file what's accumulated in the
  %%             output buffer. It writes a blank line if and only
  %%             if the output buffer is empty. Since write$ does
  %%             reasonable line breaking, you should use this
  %%             function only when you want a blank line or an
  %%             explicit line break.
  %%
  %%    write$   Pops the top (string) literal and writes it on the
  %%             output buffer (which will result in stuff being
  %%             written onto the bbl file when the buffer fills
  %%             up).
  %%
  %% Examination of the BibTeX source code shows that write$ does
  %% indeed behave as claimed, but newline$ sends a newline character
  %% directly to the output file, leaving the stack unchanged.  The
  %% first line "Writes onto ... buffer." is therefore wrong.
  %%
  %% The original BibTeX style files almost always use "write$ newline$"
  %% in that order, so it makes sense to hide that pair in a private
  %% function like this one, named after a statement in Pascal,
  %% the programming language embedded in the BibTeX Web program.

  write$                % output top-of-stack string
  newline$              % immediate write of newline (not via stack)
}

FUNCTION { init.state.consts }
{
  #0 'before.all :=
  #1 'mid.sentence :=
  #2 'after.sentence :=
  #3 'after.block :=
}

FUNCTION { output.nonnull }
{ % Stack in: ... R S T  Stack out: ... R T   File out: S<comma><space>
  's :=
  output.state mid.sentence =
    {
      ", " * write$
    }
    {
      output.state after.block =
        {
          add.period$ writeln
          "\newblock " write$
        }
        {
          output.state before.all =
            {
              write$
            }
            {
              add.period$ " " * write$
            }
          if$
        }
      if$
      mid.sentence 'output.state :=
    }
  if$
  s
}

FUNCTION { output.nonnull.dot.space }
{ % Stack in: ... R S T  Stack out: ... R T   File out: S<dot><space>
  's :=
  output.state mid.sentence =           % { "<DEBUG output.nonnull.dot.space>. " * write$ }
    {
      ". " * write$
    }
    {
      output.state after.block =
        {
          add.period$ writeln "\newblock " write$
        }
        {
          output.state before.all =
            {
              write$
            }
            {
              add.period$ " " * write$
            }
          if$
        }
      if$
      mid.sentence 'output.state :=
    }
  if$
  s
}

FUNCTION { output.nonnull.remove }
{ % Stack in: ... R S T  Stack out: ... R T   File out: S<space>
  's :=
  output.state mid.sentence =
    {
      " " * write$
    }
    {
      output.state after.block =
        {
          add.period$ writeln "\newblock " write$
        }
        {
          output.state before.all =
            {
              write$
            }
            {
              add.period$ " " * write$
            }
          if$
        }
      if$
      mid.sentence 'output.state :=
    }
  if$
  s
}

FUNCTION { output.nonnull.removenospace }
{ % Stack in: ... R S T  Stack out: ... R T   File out: S
  's :=
  output.state mid.sentence =
    {
      "" * write$
    }
    {
      output.state after.block =
        {
          add.period$ writeln "\newblock " write$
        }
        {
          output.state before.all =
            {
              write$
            }
            {
              add.period$ " " * write$
            }
          if$
        }
      if$
      mid.sentence 'output.state :=
    }
  if$
  s
}

FUNCTION { output }
{ % discard top token if empty, else like output.nonnull
  duplicate$ empty.or.unknown
    'pop$
    'output.nonnull
  if$
}

FUNCTION { output.dot.space }
{ % discard top token if empty, else like output.nonnull.dot.space
  duplicate$ empty.or.unknown
    'pop$
    'output.nonnull.dot.space
  if$
}

FUNCTION { output.removenospace }
{ % discard top token if empty, else like output.nonnull.removenospace
  duplicate$ empty.or.unknown
    'pop$
    'output.nonnull.removenospace
  if$
}

FUNCTION { output.check }
{ % like output, but warn if key name on top-of-stack is not set
  't :=
  duplicate$ empty.or.unknown
    { pop$ "empty " t * " in " * cite$ * warning$ }
    'output.nonnull
  if$
}

FUNCTION { bibinfo.output.check }
{ % like output.check, adding bibinfo field
  't :=
  duplicate$ empty.or.unknown
    { pop$ "empty " t * " in " * cite$ * warning$ }
    { "\bibinfo{" t "}{" * * swap$ * "}" *
      output.nonnull }
  if$
}

FUNCTION { output.check.dot.space }
{ % like output.dot.space, but warn if key name on top-of-stack is not set
  't :=
  duplicate$ empty.or.unknown
    { pop$ "empty " t * " in " * cite$ * warning$ }
    'output.nonnull.dot.space
  if$
}

FUNCTION { fin.block }
{ % functionally, but not logically, identical to fin.entry
   add.period$
   writeln
}

FUNCTION { fin.entry }
{
   add.period$
   writeln
}

FUNCTION { new.sentence }
{ % update sentence state, with neither output nor stack change
  output.state after.block =
    'skip$
    {
      output.state before.all =
        'skip$
        { after.sentence 'output.state := }
      if$
    }
  if$
}

FUNCTION { fin.sentence }
{
   add.period$
   write$
   new.sentence
   ""
}

FUNCTION { new.block }
{
  output.state before.all =
    'skip$
    { after.block 'output.state := }
  if$
}

FUNCTION { output.coden }       % UTAH
{ % output non-empty CODEN as one-line sentence (stack untouched)
  coden empty.or.unknown
    { }
    { "\showCODEN{" coden * "}" * writeln }
  if$
}

%
% Sometimes articleno starts with the word 'Article' or 'Paper.
% (this is a bug of acmdl, sigh)
% We strip them.  We assume eid or articleno is already on stack
%

FUNCTION { strip.articleno.or.eid }
{
  't :=
  t #1 #7 substring$ "Article" =
    {t #8 t text.length$ substring$ 't :=}
    { }
  if$
  t #1 #7 substring$ "article" =
    {t #8 t text.length$ substring$ 't :=}
    { }
  if$
  t #1 #5 substring$ "Paper" =
    {t #6 t text.length$ substring$ 't :=}
    { }
  if$
  t #1 #5 substring$ "paper" =
    {t #6 t text.length$ substring$ 't :=}
    { }
  if$
  % Strip any left trailing space or
  t #1 #1 substring$ " " =
    {t #2 t text.length$ substring$ 't :=}
    { }
  if$
  t #1 #1 substring$ "~" =
    {t #2 t text.length$ substring$ 't :=}
    { }
  if$
  t
}


FUNCTION { format.articleno }
{
  articleno empty.or.unknown not eid empty.or.unknown not and
     { "Both articleno and eid are defined for " cite$ * warning$ }
     'skip$
  if$
  articleno empty.or.unknown eid empty.or.unknown and
     { "" }
     {
        numpages empty.or.unknown
          { "articleno or eid field, but no numpages field, in "
            cite$ * warning$ }
          { }
        if$
        eid empty.or.unknown
          { "Article \bibinfo{articleno}{" articleno strip.articleno.or.eid * "}" * }
          { "Article \bibinfo{articleno}{" eid strip.articleno.or.eid * "}" * }
        if$
     }
  if$
}

FUNCTION { format.year }
{ % push year string or "[n.\,d.]" onto output stack
  %% Because year is a mandatory field, we always force SOMETHING
  %% to be output
  "\bibinfo{year}{"
  year empty.or.unknown
    { "[n.\,d.]" }
    { year }
  if$
  *  "}" *
}

FUNCTION { format.day.month }
{ % push "day month " or "month " or "" onto output stack
  day empty.or.unknown
    {
      month empty.or.unknown
        { "" }
        { "\bibinfo{date}{" month * "} " *}
      if$
    }
    {
      month empty.or.unknown
        { "" }
        { "\bibinfo{date}{" day * " " * month * "} " *}
      if$
    }
  if$
}

FUNCTION { format.day.month.year }     % UTAH
{ % if month is empty, push "" else push "(MON.)" or "(DD MON.)"
  % Needed for frequent periodicals: 2008. ... New York Times C-1, C-2, C-17 (23 Oct.)
  % acm-*.bst addition: prefix parenthesized date string with
  % ", Article nnn "
  articleno empty.or.unknown eid empty.or.unknown and
    { "" }
    { output.state after.block =
       {", " format.articleno * }
       { format.articleno  }
      if$
    }
  if$
  " (" * format.day.month * format.year * ")" *
}

FUNCTION { output.day.month.year }     % UTAH
{ % if month is empty value, do nothing; else output stack top and
  % leave with new top string "(MON.)" or "(DD MON.)"
  % Needed for frequent periodicals: 2008. ... New York Times C-1, C-2, C-17 (23 Oct.)
  format.day.month.year
  output.nonnull.remove
}

FUNCTION { strip.doi } % UTAH
{ % Strip any Web address prefix to recover the bare DOI, leaving the
  % result on the output stack, as recommended by CrossRef DOI
  % documentation.
  % For example, reduce "http://doi.acm.org/10.1145/1534530.1534545" to
  % "10.1145/1534530.1534545".  A suitable URL is later typeset and
  % displayed as the LAST item in the reference list entry.  Publisher Web
  % sites wrap this with a suitable link to a real URL to resolve the DOI,
  % and the master https://doi.org/ address is preferred, since publisher-
  % specific URLs can disappear in response to economic events.  All
  % journals are encouraged by the DOI authorities to use that typeset
  % format and link procedures for uniformity across all publications that
  % include DOIs in reference lists.
  % The numeric prefix is guaranteed to start with "10.", so we use
  % that as a test.
  % 2017-02-04 Added stripping of https:// (Boris)
  doi #1 #3 substring$ "10." =
    { doi }
    {
      doi 't :=  % get modifiable copy of DOI

      % Change https:// to http:// to strip both prefixes (BV)

      t #1 #8 substring$ "https://" =
        { "http://"  t #9 t text.length$ #8 - substring$ * 't := }
        { }
      if$

      t #1 #7 substring$ "http://" =
        {
            t #8 t text.length$ #7 - substring$ 't :=

            "INTERNAL STYLE-FILE ERROR" 's :=

            % search for next "/" and assign its suffix to s

            { t text.length$ }
            {
              t #1 #1 substring$ "/" =
                {
                  % save rest of string as true DOI (should be 10.xxxx/yyyy)
                  t #2 t text.length$ #1 - substring$ 's :=
                  "" 't :=    % empty string t terminates the loop
                }
                {
                  % discard first character and continue loop: t <= substring(t,2,last)
                  t #2 t text.length$ #1 - substring$ 't :=
                }
              if$
            }
            while$

            % check for valid DOI (should be 10.xxxx/yyyy)
            s #1 #3 substring$ "10." =
              { }
              { "unrecognized DOI substring " s * " in DOI value [" * doi * "]" * warning$ }
            if$

            s   % push the stripped DOI on the output stack

        }
        {
          "unrecognized DOI value [" doi * "]" * warning$
          doi   % push the unrecognized original DOI on the output stack
        }
      if$
    }
  if$
}

%
% Change by BV: added standard prefix to URL
%
FUNCTION { output.doi } % UTAH
{ % output non-empty DOI as one-line sentence (stack untouched)
  doi empty.or.unknown
    { }
    {
      %% Use \urldef here for the same reason it is used in output.url,
      %% see output.url for further discussion.
      "\urldef\tempurl%" writeln
      "\doi{" strip.doi * "}%" * writeln
      "\showDOI{\tempurl}" writeln
    }
  if$
}

FUNCTION { output.isbn }                % UTAH
{ % output non-empty ISBN-10 and/or ISBN-13 as one-line sentences (stack untouched)
  show-isbn-10-and-13
    {
      %% show both 10- and 13-digit ISBNs
      isbn empty.or.unknown
        { }
        {
          "\showISBNx{" isbn * "}" * writeln
        }
      if$
      isbn-13 empty.or.unknown
        { }
        {
          "\showISBNxiii{" isbn-13 * "}" * writeln
        }
      if$
    }
    {
      %% show 10-digit ISBNs only if 13-digit ISBNs not available
      isbn-13 empty.or.unknown
        {
          isbn empty.or.unknown
            { }
            {
              "\showISBNx{" isbn * "}" * writeln
            }
          if$
        }
        {
          "\showISBNxiii{" isbn-13 * "}" * writeln
        }
      if$
    }
  if$
}

FUNCTION { output.issn } % UTAH
{ % output non-empty ISSN as one-line sentence (stack untouched)
  issn empty.or.unknown
    { }
    { "\showISSN{" issn * "}" * writeln }
  if$
}

FUNCTION { output.issue }
{ % output non-empty issue number as a one-line sentence (stack untouched)
  issue empty.or.unknown
    { }
    { "Issue " issue * "." * writeln }
  if$
}

FUNCTION { output.lccn } % UTAH
{ % return with stack untouched
  lccn empty.or.unknown
    { }
    { "\showLCCN{" lccn * "}" * writeln }
  if$
}

FUNCTION { output.note } % UTAH
{ % return with stack empty
  note empty.or.unknown
    { }
    { "\shownote{" note * "}" add.period$ * writeln }
  if$
}

FUNCTION { output.note.check } % UTAH
{ % return with stack empty
  note empty.or.unknown
    { "empty note in " cite$ * warning$ }
    { "\shownote{" note * "}" add.period$ * writeln }
  if$
}

% Changed by Ziv in 2022
% - Use \showeprint
% - Don't output if DOI is defined
FUNCTION { output.eprint } %
{ % return with stack empty
  doi empty.or.unknown
  {
    eprint empty.or.unknown
      { }
      { "\showeprint"
          archiveprefix empty.or.unknown
            { eprinttype empty.or.unknown
                { "{}" * }
                { "{" eprinttype "}" * * * }
              if$
            }
            { "{" archiveprefix "}" * * * }
          if$
        "{" eprint "}" * * *
          primaryclass empty.or.unknown
            { eprintclass empty.or.unknown
              { "{}" * }
              { "{" eprintclass "}" * * * }
              if$
            }
            { "{" primaryclass "}" * * * }
          if$
        writeln
      }
    if$
  }
  { }
  if$
}


%
% Changes by BV 2011/04/15.  Do not output
% url if doi is defined
%
FUNCTION { output.url } % UTAH
{ % return with stack untouched
  % output URL and associated lastaccessed fields
  doi empty.or.unknown
  {
    url empty.or.unknown
      { }
      {
          %% Use \urldef, outside \showURL, so that %nn, #, etc in URLs work
          %% correctly.  Put the actual URL on its own line to reduce the
          %% likelihood of BibTeX's nasty line wrapping after column 79.
          %% \url{} can undo this, but if that doesn't work for some reason
          %% the .bbl file would have to be repaired manually.
          "\urldef\tempurl%" writeln
          "\url{" url * "}%" * writeln

          "\showURL{%" writeln
          lastaccessed empty.or.unknown
            { "" }
            { "Retrieved " lastaccessed * " from " * }
          if$
          "\tempurl}" * writeln
      }
      if$
  }
  { }
  if$
}

FUNCTION { output.year.check }
{ % warn if year empty, output top string and leave " YEAR<label>" on stack in mid-sentence
  year empty.or.unknown
     { "empty year in " cite$ * warning$
       write$
       " \bibinfo{year}{[n.\,d.]}"
       "\natexlab{" extra.label * "}" * *
       mid.sentence 'output.state :=
     }
     { write$
       " \bibinfo{year}{" year * "}"  *
       "\natexlab{" extra.label * "}" * *
       mid.sentence 'output.state :=
     }
  if$
}


FUNCTION { le }
{
  %% test whether first number is less than or equal to second number
  %% stack in:  n1 n2
  %% stack out: if n1 <= n2 then 1 else 0

  %% "DEBUG: le " cite$ * warning$
  > { #0 } { #1 } if$
}

FUNCTION { ge }
{
  %% test whether first number is greater than or equal to second number
  %% stack in:  n1 n2
  %% stack out: if n1 >= n2 then 1 else 0

  %% "DEBUG: ge " cite$ * warning$
  < { #0 } { #1 } if$
}

FUNCTION { is.leading.digit }
{
  %% test whether first character of string is a digit
  %% stack in:  string
  %% stack out: if first-char-is-digit then 1 else 0

  #1 #1 substring$                      % replace string by string[1:1]
  duplicate$                            % string[1:1] string[1:1]
  chr.to.int$
  "0" chr.to.int$ swap$ le              % "0" <= string[1:1] --> 0-or-1
  swap$                                 % 0-or-1 string[1:1]
  chr.to.int$
  "9" chr.to.int$ le                    % string[1:1} <= "9" --> 0-or-1
  and
}

FUNCTION { skip.digits }
{
  %% skip over leading digits in string
  %% stack in:  string
  %% stack out: rest-of-string leading-digits

  %% "DEBUG: enter skip.digits " cite$ * warning$

  %% dump.stack.1

  duplicate$
  't :=
  't.org :=
  "" 'u :=

  { t text.length$ }
  {
    %% "=================DEBUG: skip.digits   t = [" t * "]" * warning$
    t is.leading.digit
      { t #2 t text.length$ #1 - substring$ }
      {
        t 'u :=
        ""
      }
    if$
    't :=
  }
  while$

  u                                                             % rest of string
  t.org #1 t.org text.length$ u text.length$ - substring$       % leading digits

  %% "DEBUG: t.org = [" t.org * "]" * warning$
  %% "DEBUG: u     = [" u * "]" * warning$

  %% dump.stack.2

  %% "DEBUG: leave skip.digits " cite$ * warning$
}

FUNCTION { skip.nondigits }
{
  %% skip over leading nondigits in string
  %% stack in:  string
  %% stack out: rest-of-string

  %% "DEBUG: enter skip.nondigits " cite$ * warning$

  't :=
  "" 'u :=

  { t text.length$ }
  {
    %% "=================DEBUG: skip.nondigits   t = [" t * "]" * warning$
    t is.leading.digit
      {
        t 'u :=
        ""
      }
      { t #2 t text.length$ #1 - substring$ }
    if$
    't :=
  }
  while$

  u                     % rest of string

  %% dump.stack.1
  %% "DEBUG: leave skip.nondigits " cite$ * warning$
}

FUNCTION { parse.next.number }
{
  %% stack in:  string
  %% stack out: rest-of-string next-numeric-part-of-string
  %% Example:
  %% stack in:  "123:1--123:59"
  %% stack out: ":1--123:59" "123"

  's :=
  s skip.nondigits 's :=
  s skip.digits
}

FUNCTION { reduce.pages.to.page.count }
{
  %% Stack in:  arbitrary-and-unused
  %% Stack out: unchanged
  %%
  %% For the new-style pagination with article number and numpages or
  %% pages, we expect to have BibTeX entries containing something like
  %%     articleno = "17",
  %%     pages     = "1--23",
  %% with output "Article 17, 23 pages",
  %% or
  %%     articleno = "17",
  %%     numpages  = "23",
  %% with output "Article 17, 23 pages",
  %% or
  %%     articleno = "17",
  %%     pages     = "17:1--17:23",
  %% with output "Article 17, 23 pages",
  %%
  %% If articleno is missing or empty, then we should output "1--23",
  %% "23" (with a warning of a missing articleno), or "17:1--17:23",
  %% respectively.

  %% "DEBUG: enter reduce.pages.to.page.count " cite$ * warning$

  %% "DEBUG: pages = [" pages * "]" * warning$

  pages
  parse.next.number 'p1 :=
  parse.next.number 'p2 :=
  parse.next.number 'p3 :=
  parse.next.number 'page.count :=

  duplicate$
  empty.or.unknown
    {  }
    {
      duplicate$ "unexpected trailing garbage [" swap$ *
      "] after n:p1--n:p2 in pages = [" *
      pages *
      "] in " *
      cite$ *
      warning$
    }
  if$

  pop$

  %% "DEBUG: reduce.pages.to.page.count: "
  %% " p1 = " p1 * *
  %% " p2 = " p2 * *
  %% " p3 = " p3 * *
  %% " p4 = " page.count * *
  %% " in " cite$ * * warning$

  p1 p3 =   p2 "1" =   and   numpages empty.or.unknown   and
    { "INFO: reduced pages = [" pages * "] to numpages = [" * page.count * "]" * warning$ }
    {
      numpages empty.or.unknown
        { pages }
        { numpages }
      if$
      'page.count :=
    }
  if$

  p1 "1" =   p3 empty.or.unknown   and   numpages empty.or.unknown   and
    {
      p2 'page.count :=
      "INFO: reduced pages = [" pages * "] to numpages = [" * page.count * "]" * warning$
    }
    {
      numpages empty.or.unknown
        { pages }
        { numpages }
      if$
      'page.count :=
    }
  if$

  %% "DEBUG: leave reduce.pages.to.page.count " cite$ * warning$
}

FUNCTION { new.block.checkb }
{ % issue a new.block only if at least one of top two stack strings is not empty
  empty.or.unknown
  swap$ empty.or.unknown
  and
    'skip$
    'new.block
  if$
}

FUNCTION { field.or.null }
{ % convert empty value to null string, else return value
  duplicate$ empty.or.unknown
    { pop$ "" }
    'skip$
  if$
}



FUNCTION { emphasize }
{ % emphasize a non-empty top string on the stack
  duplicate$ empty.or.unknown
    { pop$ "" }
    { "\emph{" swap$ * "}" * }
  if$
}

FUNCTION { comma }
{ % convert empty string to null string, or brace string and add trailing comma
  duplicate$ empty.or.unknown
    { pop$ "" }
    { "{" swap$ * "}," * }
  if$
}

FUNCTION { format.names }
{
  % Format bibliographical entries with the first author last name first,
  % and subsequent authors with initials followed by last name.
  % All names are formatted in this routine.

  's :=
  #1 'nameptr :=               % nameptr = 1;
  s num.names$ 'numnames :=    % numnames = num.name$(s);
  numnames 'namesleft :=
    { namesleft #0 > }
    { nameptr #1 =
        %NO: BAD ORDER: {"{" s nameptr "{ff~}{ll}{, jj}{, vv}" format.name$ * "}" * 't := }
        %NO: BAD ORDER: {"{" s nameptr "{ff~}{ll}{, jj}{, vv}" format.name$ * "}" * 't := }
        {"\bibinfo{person}{" s nameptr "{ff }{vv }{ll}{, jj}" format.name$ * "}" * 't := }
        {"\bibinfo{person}{" s nameptr "{ff }{vv }{ll}{, jj}" format.name$ * "}" * 't := }
      if$
      nameptr #1 >
        {
          namesleft #1 >
            { ", " * t * }
            {
              numnames #2 >
                { "," * }
                'skip$
              if$
              t "\bibinfo{person}{others}" =
                { " {et~al\mbox{.}}" * } % jrh: avoid spacing problems
                { " {and} " * t * } % from Chicago Manual of Style
              if$
            }
          if$
        }
        't
      if$
      nameptr #1 + 'nameptr :=          % nameptr += 1;
      namesleft #1 - 'namesleft :=      % namesleft =- 1;
    }
  while$
}

FUNCTION { my.full.label }
{
  's :=
  #1 'nameptr :=               % nameptr = 1;
  s num.names$ 'numnames :=    % numnames = num.name$(s);
  numnames 'namesleft :=
    { namesleft #0 > }

    { s nameptr "{vv~}{ll}" format.name$ 't :=  % get the next name
      nameptr #1 >
        {
          namesleft #1 >
            { ", " * t * }
            {
              numnames #2 >
                { "," * }
                'skip$
              if$
              t "others" =
                { " et~al\mbox{.}" * } % jrh: avoid spacing problems
                { " and " * t * } % from Chicago Manual of Style
              if$
            }
          if$
        }
        't
      if$
      nameptr #1 + 'nameptr :=          % nameptr += 1;
      namesleft #1 - 'namesleft :=      % namesleft =- 1;
    }
  while$

}

FUNCTION { format.names.fml }
{
  % Format names in "familiar" format, with first initial followed by
  % last name. Like format.names, ALL names are formatted.
  % jtb: The names are NOT put in small caps

  's :=
  #1 'nameptr :=               % nameptr = 1;
  s num.names$ 'numnames :=    % numnames = num.name$(s);
  numnames 'namesleft :=
    { namesleft #0 > }

    {
      "\bibinfo{person}{" s nameptr "{ff~}{vv~}{ll}{, jj}" format.name$ * "}" * 't :=

      nameptr #1 >
        {
          namesleft #1 >
            { ", " * t * }
            {
              numnames #2 >
                { "," * }
                'skip$
              if$
              t "\bibinfo{person}{others}" =
                { " {et~al\mbox{.}}" * }
                { " {and} " * t * }
              if$
            }
          if$
        }
        't
      if$
      nameptr #1 + 'nameptr :=          % nameptr += 1;
      namesleft #1 - 'namesleft :=      % namesleft =- 1;
    }
  while$
}

FUNCTION { format.authors }
{
  author empty.or.unknown
    { "" }
    {
      "\bibfield{author}{"
      author format.names add.period$ * "}" *} % jtb: add period if none before
  if$
}

FUNCTION { format.key }
{
  empty.or.unknown
    { key field.or.null }
    { "" }
  if$
}

FUNCTION { format.no.key }
{
  empty.or.unknown
    { "" }
    { "" }
  if$
}

FUNCTION { format.editors.fml }
{
  % Format editor names for use in the "in" types: inbook, incollection,
  % inproceedings: first initial, then last names. When editors are the
  % LABEL for an entry, then format.editor is used which lists editors
  % by last name first.

  editor empty.or.unknown
    { "" }
    {
      "\bibfield{editor}{"
      editor format.names.fml
      *  "}" *
      editor num.names$ #1 >
        { " (Eds.)" * }
        { " (Ed.)" * }
      if$
    }
  if$
}

FUNCTION { format.editors }
{ % format editor names for use in labels, last names first.
  editor empty.or.unknown
    { "" }
    {
      "\bibfield{editor}{"
      editor format.names
      *  "}" *
      editor num.names$ #1 >
        { " (Eds.)." * }
        { " (Ed.)." * }
      if$
    }
  if$
}

FUNCTION { format.articletitle }
{
  title empty.or.unknown
    { "" }
    % Use this to preserve lettercase in titles:
    { "\showarticletitle{" title * "}" * }
    % Use this for downcase title style:
    % { \showarticletitle{" title "t" change.case$ * "}" * }
  if$
}

FUNCTION { format.title }
{
  title empty.or.unknown
    { "" }
    % Use this to preserve lettercase in titles:
    { "\bibinfo{title}{" title * "}" * }
    % Use this for downcase title style:
    % { title "t" change.case$ }
  if$
}

FUNCTION { n.dashify }
{
  't :=
  ""
    { t empty.or.unknown not }
    {
      t #1 #1 substring$ "-" =
        {
          t #1 #2 substring$ "--" = not
            { "--" *
              t #2 global.max$ substring$ 't :=
            }
            {
              { t #1 #1 substring$ "-" = }
              {
                "-" *
                t #2 global.max$ substring$ 't :=
              }
              while$
            }
          if$
        }
        {
          t #1 #1 substring$ *
          t #2 global.max$ substring$ 't :=
        }
      if$
    }
  while$
}

FUNCTION { format.a.title.with.edition }
{
  "\bibinfo{booktitle}{"
  swap$ emphasize *
  edition empty.or.unknown
    'skip$
    { " (\bibinfo{edition}{" * edition "l" change.case$ *
      "} ed.)" * } % jtb: no parens for ed.
  if$
  "}" *
}

FUNCTION { format.btitle }
{ title format.a.title.with.edition }

FUNCTION { format.emphasize.booktitle }
{ booktitle format.a.title.with.edition }



FUNCTION { format.city }
{
  % jtb: if the preceding string (the title of the conference) is non-empty,
  % jtb: append the location, otherwise leave empty (so as to trigger the
  % jtb: error message in output.check

  duplicate$ empty.or.unknown
    { }
    {
      city empty.or.unknown location empty.or.unknown and
        {
          date empty.or.unknown
            { }
            { " (" * date * ")" * }
          if$
        }
        {
          location empty.or.unknown
            {
              date empty.or.unknown
                { " (" * city * ")" * }
                { " (" * city * ", " * date * ")" * }
              if$
            }
            {
              date empty.or.unknown
                { " (" * location * ")" * }
                { " (" * location * ", " * date * ")" * }
              if$
            }
          if$
        }
      if$
    }
  if$
}

FUNCTION { tie.or.space.connect }
{
  duplicate$ text.length$ #3 <
    { "~" }
    { " " }
  if$
  swap$ * *
}

FUNCTION { either.or.check }
{
  empty.or.unknown
    'pop$
    { "can't use both " swap$ * " fields in " * cite$ * warning$ }
  if$
}

FUNCTION { format.bvolume }
{
  % jtb: If there is a series, this is added and the volume trails after it.
  % jtb: Otherwise, "Vol" is Capitalized.

  volume empty.or.unknown
    { "" }
    {
      series empty.or.unknown
        { "Vol.~\bibinfo{volume}{" volume "}" * *}
        { "\bibinfo{series}{" series "}, " * *
          "Vol.~\bibinfo{volume}{" volume "}" * * *}
      if$
      "volume and number" number either.or.check
    }
  if$
}

FUNCTION { format.bvolume.noseries }
{
  volume empty.or.unknown
    { "" }
    { "Vol.~\bibinfo{volume}{" volume "}" * *
      "volume and number" number either.or.check
    }
  if$
}

FUNCTION { format.series }
{
  series empty.or.unknown
    {""}
    {" \emph{(\bibinfo{series}{" * series "}" *
     volume empty.or.unknown
       {
         number empty.or.unknown
            {")}" *}
            {", \bibinfo{number}{" number "})}" * * *}
          if$
       }
       {", Vol.~\bibinfo{volume}{" volume "})}" * * *
        "volume and number" number either.or.check
       }
     if$
    }
  if$
}

FUNCTION { format.number.series }
{
  volume empty.or.unknown
    {
      number empty.or.unknown
        {
          volume empty.or.unknown
          { "" }
          {
            series empty.or.unknown
              { "" }
              { " (\bibinfo{series}{" series * "})" * }
            if$
          }
          if$
        }                                       %    { series field.or.null }
        {
          output.state mid.sentence =
            { "Number" }                        % gnp - changed to mixed case always
            { "Number" }
          if$
          number tie.or.space.connect series empty.or.unknown
            { "there's a number but no series in " cite$ * warning$ }
            { " in \bibinfo{series}{" * series * "}" * }
          if$
        }
      if$
    }
    {
      ""
    }
  if$
}

FUNCTION { multi.page.check }
{
  't :=
  #0 'multiresult :=
    { multiresult not
      t empty.or.unknown not
      and
    }
    { t #1 #1 substring$
      duplicate$ "-" =
      swap$ duplicate$ "," =
      swap$ "+" =
      or or
    { #1 'multiresult := }
    { t #2 global.max$ substring$ 't := }
      if$
    }
  while$
  multiresult
}

FUNCTION { format.pages }
{
  pages empty.or.unknown
    { "" }
    { "\bibinfo{pages}{"
      pages multi.page.check
        { pages n.dashify } % gnp - removed () % jtb: removed pp.
        { pages }
      if$
      * "}" *
    }
  if$
}

FUNCTION { format.pages.check.without.articleno }
{ %% format pages field only if articleno is absent
  %% Stack out: pages-specification
  numpages missing$ pages missing$ and
    { "page numbers missing in both pages and numpages fields in " cite$ * warning$ }
    { }
  if$

  articleno empty.or.unknown eid empty.or.unknown and
    {
      pages missing$
        {
	   numpages empty.or.unknown
	     {""}
             { "\bibinfo{numpages}{" numpages * "}~pages" * }
	  if$
	}
        { format.pages }
      if$
    }
    { "" }
  if$
}

FUNCTION { format.pages.check }
{
  pages empty.or.unknown
    { "page numbers missing in " cite$ * warning$ "" }
    { pages n.dashify }
  if$
}

FUNCTION { format.bookpages }
{
  bookpages empty.or.unknown
    { "" }
    { bookpages "book pages" tie.or.space.connect }
  if$
}

FUNCTION { format.named.pages }
{
  pages empty.or.unknown
    { "" }
    { format.pages "pages" tie.or.space.connect }
  if$
}

%
% Changed by Boris Veytsman, 2011-03-13
% Now the word "pages" is printed even if
% there field pages is not empty.
%

FUNCTION { format.page.count }
{
  page.count empty.or.unknown
    { "" }
    { "\bibinfo{numpages}{" page.count * "}~pages" * }
  if$
}

FUNCTION { format.articleno.numpages }
{
  %% There are seven possible outputs, depending on which fields are set.
  %%
  %% These four are handled here:
  %%
  %%     articleno, numpages, pages     -> "Article articleno-value, numpages-value pages"
  %%     articleno, numpages            -> "Article articleno-value, numpages-value pages"
  %%     articleno, pages               -> "Article articleno-value, reduced-pages-value pages"
  %%     articleno                      -> "Article articleno-value" and warn about missing numpages
  %%
  %% The remaining three have already been handled by
  %% format.pages.check.without.articleno:
  %%
  %%     numpages, pages                -> "pages-value"
  %%     numpages                       -> "numpages-value"
  %%     pages                          -> "pages-value"
  %%
  %% We no longer issue warninig when missing articleno, but having numpages

  articleno empty.or.unknown eid empty.or.unknown and
    {
%%      numpages empty.or.unknown
%%        { }
%%        { "numpages field, but no articleno or eid field, in "
%%          cite$ * warning$ }
%%      if$
      ""
    }
    {
      numpages empty.or.unknown
        {
          pages empty.or.unknown
            {
              "articleno or eid, but no pages or numpages field in "
                 cite$ * warning$
              "" 'page.count :=
            }
            { reduce.pages.to.page.count }
          if$
        }
        { numpages 'page.count := }
      if$

      %% The Article number is now handled in format.day.month.year because
      %% ACM prefers the style "Digital Libraries 12, 3, Article 5 (July 2008)"
      %% over "Digital Libraries 12, 3 (July 2008), Article 5"
      %% format.articleno output
      format.page.count
    }
  if$
}

FUNCTION {calc.format.page.count}
{
  numpages empty.or.unknown
   {
     pages empty.or.unknown
        {
        "" 'page.count :=
        }
        { reduce.pages.to.page.count }
     if$
   }
   { numpages 'page.count := }
  if$
  format.page.count
}


FUNCTION { journal.canon.abbrev }
{
  % Returns a canonical abbreviation for 'journal', or else 'journal'
  % unchanged.
  journal "ACM Computing Surveys"                                                                       = { "Comput. Surveys"                                 } {
  journal "{ACM} Computing Surveys"                                                                     = { "Comput. Surveys"                                 } {
  journal "ACM Transactions on Mathematical Software"                                                   = { "ACM Trans. Math. Software"                       } {
  journal "{ACM} Transactions on Mathematical Software"                                                 = { "ACM Trans. Math. Software"                       } {
  journal "ACM SIGNUM Newsletter"                                                                       = { "ACM SIGNUM Newslett."                            } {
  journal "ACM {SIGNUM} Newsletter"                                                                     = { "ACM SIGNUM Newslett."                            } {
  journal "{ACM} SIGNUM Newsletter"                                                                     = { "ACM SIGNUM Newslett."                            } {
  journal "{ACM} {SIGNUM} Newsletter"                                                                   = { "ACM SIGNUM Newslett."                            } {
  journal "American Journal of Sociology"                                                               = { "Amer. J. Sociology"                              } {
  journal "American Mathematical Monthly"                                                               = { "Amer. Math. Monthly"                             } {
  journal "American Mathematical Society Translations"                                                  = { "Amer. Math. Soc. Transl."                        } {
  journal "Applied Mathematics and Computation"                                                         = { "Appl. Math. Comput."                             } {
  journal "British Journal of Mathematical and Statistical Psychology"                                  = { "Brit. J. Math. Statist. Psych."                  } {
  journal "Bulletin of the American Mathematical Society"                                               = { "Bull. Amer. Math. Soc."                          } {
  journal "Canadian Mathematical Bulletin"                                                              = { "Canad. Math. Bull."                              } {
  journal "Communications of the ACM"                                                                   = { "Commun. ACM"                                     } {
  journal "Communications of the {ACM}"                                                                 = { "Commun. ACM"                                     } {
  journal "Computers and Structures"                                                                    = { "Comput. \& Structures"                           } {
  journal "Contemporary Mathematics"                                                                    = { "Contemp. Math."                                  } {
  journal "Crelle's Journal"                                                                            = { "Crelle's J."                                     } {
  journal "Giornale di Mathematiche"                                                                    = { "Giorn. Mat."                                     } {
  journal "IEEE Transactions on Aerospace and Electronic Systems"                                       = { "IEEE Trans. Aerospace Electron. Systems"         } {
  journal "{IEEE} Transactions on Aerospace and Electronic Systems"                                     = { "IEEE Trans. Aerospace Electron. Systems"         } {
  journal "IEEE Transactions on Automatic Control"                                                      = { "IEEE Trans. Automat. Control"                    } {
  journal "{IEEE} Transactions on Automatic Control"                                                    = { "IEEE Trans. Automat. Control"                    } {
  journal "IEEE Transactions on Computers"                                                              = { "IEEE Trans. Comput."                             } {
  journal "{IEEE} Transactions on Computers"                                                            = { "IEEE Trans. Comput."                             } {
  journal "IMA Journal of Numerical Analysis"                                                           = { "IMA J. Numer. Anal."                             } {
  journal "{IMA} Journal of Numerical Analysis"                                                         = { "IMA J. Numer. Anal."                             } {
  journal "Information Processing Letters"                                                              = { "Inform. Process. Lett."                          } {
  journal "International Journal for Numerical Methods in Engineering"                                  = { "Internat. J. Numer. Methods Engrg."              } {
  journal "International Journal of Control"                                                            = { "Internat. J. Control"                            } {
  journal "International Journal of Supercomputing Applications"                                        = { "Internat. J. Supercomputing Applic."             } {
  journal "Journal of Computational Physics"                                                            = { "J. Comput. Phys."                                } {
  journal "Journal of Computational and Applied Mathematics"                                            = { "J. Comput. Appl. Math."                          } {
  journal "Journal of Computer and System Sciences"                                                     = { "J. Comput. System Sci."                          } {
  journal "Journal of Mathematical Analysis and Applications"                                           = { "J. Math. Anal. Appl."                            } {
  journal "Journal of Mathematical Physics"                                                             = { "J. Math. Phys."                                  } {
  journal "Journal of Parallel and Distributed Computing"                                               = { "J. Parallel and Distrib. Comput."                } {
  journal "Journal of Research of the National Bureau of Standards"                                     = { "J. Res. Nat. Bur. Standards"                     } {
  journal "Journal of VLSI and Computer Systems"                                                        = { "J. VLSI Comput. Syst."                           } {
  journal "Journal of {VLSI} and Computer Systems"                                                      = { "J. VLSI Comput. Syst."                           } {
  journal "Journal of the ACM"                                                                          = { "J. ACM"                                          } {
  journal "Journal of the American Statistical Association"                                             = { "J. Amer. Statist. Assoc."                        } {
  journal "Journal of the Institute of Mathematics and its Applications"                                = { "J. Inst. Math. Appl."                            } {
  journal "Journal of the Society for Industrial and Applied Mathematics"                               = { "J. Soc. Indust. Appl. Math."                     } {
  journal "Journal of the Society for Industrial and Applied Mathematics, Series B, Numerical Analysis" = { "J. Soc. Indust. Appl. Math. Ser. B Numer. Anal." } {
  journal "Linear Algebra and its Applications"                                                         = { "Linear Algebra Appl."                            } {
  journal "Mathematica Scandinavica"                                                                    = { "Math. Scand."                                    } {
  journal "Mathematical Tables and Other Aids to Computation"                                           = { "Math. Tables Aids Comput."                       } {
  journal "Mathematics of Computation"                                                                  = { "Math. Comp."                                     } {
  journal "Mathematische Annalen"                                                                       = { "Math. Ann."                                      } {
  journal "Numerische Mathematik"                                                                       = { "Numer. Math."                                    } {
  journal "Pacific Journal of Mathematics"                                                              = { "Pacific J. Math."                                } {
  journal "Parallel Computing"                                                                          = { "Parallel Comput."                                } {
  journal "Philosophical Magazine"                                                                      = { "Philos. Mag."                                    } {
  journal "Proceedings of the American Mathematical Society"                                            = { "Proc. Amer. Math. Soc."                          } {
  journal "Proceedings of the IEEE"                                                                     = { "Proc. IEEE"                                      } {
  journal "Proceedings of the {IEEE}"                                                                   = { "Proc. IEEE"                                      } {
  journal "Proceedings of the National Academy of Sciences of the USA"                                  = { "Proc. Nat. Acad. Sci. U. S. A."                  } {
  journal "Quarterly Journal of Mathematics, Oxford, Series (2)"                                        = { "Quart. J. Math. Oxford Ser. (2)"                 } {
  journal "Quarterly of Applied Mathematics"                                                            = { "Quart. Appl. Math."                              } {
  journal "Review of the International Statisical Institute"                                            = { "Rev. Inst. Internat. Statist."                   } {
  journal "SIAM Journal on Algebraic and Discrete Methods"                                              = { "SIAM J. Algebraic Discrete Methods"              } {
  journal "{SIAM} Journal on Algebraic and Discrete Methods"                                            = { "SIAM J. Algebraic Discrete Methods"              } {
  journal "SIAM Journal on Applied Mathematics"                                                         = { "SIAM J. Appl. Math."                             } {
  journal "{SIAM} Journal on Applied Mathematics"                                                       = { "SIAM J. Appl. Math."                             } {
  journal "SIAM Journal on Computing"                                                                   = { "SIAM J. Comput."                                 } {
  journal "{SIAM} Journal on Computing"                                                                 = { "SIAM J. Comput."                                 } {
  journal "SIAM Journal on Matrix Analysis and Applications"                                            = { "SIAM J. Matrix Anal. Appl."                      } {
  journal "{SIAM} Journal on Matrix Analysis and Applications"                                          = { "SIAM J. Matrix Anal. Appl."                      } {
  journal "SIAM Journal on Numerical Analysis"                                                          = { "SIAM J. Numer. Anal."                            } {
  journal "{SIAM} Journal on Numerical Analysis"                                                        = { "SIAM J. Numer. Anal."                            } {
  journal "SIAM Journal on Scientific and Statistical Computing"                                        = { "SIAM J. Sci. Statist. Comput."                   } {
  journal "{SIAM} Journal on Scientific and Statistical Computing"                                      = { "SIAM J. Sci. Statist. Comput."                   } {
  journal "SIAM Review"                                                                                 = { "SIAM Rev."                                       } {
  journal "{SIAM} Review"                                                                               = { "SIAM Rev."                                       } {
  journal "Software Practice and Experience"                                                            = { "Software Prac. Experience"                       } {
  journal "Statistical Science"                                                                         = { "Statist. Sci."                                   } {
  journal "The Computer Journal"                                                                        = { "Comput. J."                                      } {
  journal "Transactions of the American Mathematical Society"                                           = { "Trans. Amer. Math. Soc."                         } {
  journal "USSR Computational Mathematics and Mathematical Physics"                                     = { "U. S. S. R. Comput. Math. and Math. Phys."       } {
  journal "{USSR} Computational Mathematics and Mathematical Physics"                                   = { "U. S. S. R. Comput. Math. and Math. Phys."       } {
  journal "Zeitschrift fur Angewandte Mathematik und Mechanik"                                          = { "Z. Angew. Math. Mech."                           } {
  journal "Zeitschrift fur Angewandte Mathematik und Physik"                                            = { "Z. Angew. Math. Phys."                           } {
  journal
  } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$
  } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$
  } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$
  } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$
  } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$
  } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$
  } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$
  } if$ } if$ } if$ } if$ } if$ } if$ } if$ } if$
}

FUNCTION { format.journal.volume.number.day.month.year }
{
  % By Young (and Spencer)
  % GNP - fixed bugs with missing volume, number, and/or pages
  %
  % Format journal, volume, number, pages for article types.
  %
  journal empty.or.unknown
    { "no journal in " cite$ * warning$ "" }
    { "\bibinfo{journal}{"
      journal.canon.abbrev emphasize *
      "}" * }
  if$

  number empty.or.unknown
    {
      volume empty.or.unknown
        { "no number and no volume in " cite$ * warning$ "" * }
        { " " * " \bibinfo{volume}{" * volume * "}" * }
      if$
    }
    {
      volume empty.or.unknown
        {
          "unusual to have number, but no volume, for " cite$ * warning$
          " \bibinfo{number}{" * number * "}" *
        }
        { " \bibinfo{volume}{" * volume  * "}, \bibinfo{number}{" *
          number * "}" *}
      if$
    }
  if$
  after.block 'output.state :=

  % Sometimes proceedings are published in journals
  % In this case we do not want to put year, day and month here

  type$ "inproceedings" =
    { }
    {format.day.month.year * }
  if$
}

FUNCTION { format.chapter.pages }
{
  chapter empty.or.unknown
    'format.pages
    { type empty.or.unknown
        { "Chapter" } % gnp - changed to mixed case
        { type "t" change.case$ }
      if$
      chapter tie.or.space.connect
      pages empty.or.unknown
        {"page numbers missing in " cite$ * warning$} % gnp - added check
        { ", " * format.pages * }
      if$
    }
  if$
}

FUNCTION { format.in.emphasize.booktitle }
{ % jtb: format for collections or proceedings not appearing in a journal
  booktitle empty.or.unknown
  { "" }
  { "In " format.emphasize.booktitle * }
  if$
}

FUNCTION { format.in.booktitle }
{ % jtb: format for proceedings appearing in a journal
  booktitle empty.or.unknown
  { "" }
  { "In \bibinfo{booktitle}{" booktitle * "}" * }
  if$
}

FUNCTION { format.in.ed.booktitle }
{
  booktitle empty.or.unknown
  { "" }
  { editor empty.or.unknown
    { "In " format.emphasize.booktitle * }
                % jtb: swapped editor location
    { "In " format.emphasize.booktitle * ", " * format.editors.fml * }
    if$
  }
  if$
}

FUNCTION { format.thesis.type }
{ % call with default type on stack top
  type empty.or.unknown
    'skip$    % use default type
    {
      pop$    % discard default type
      % NO: it is silly to have to brace protect every degree type!:  type "t" change.case$
      type
    }
  if$
}

FUNCTION { format.tr.number }
{
  "\bibinfo{type}{"
  type empty.or.unknown
    { "{T}echnical {R}eport" }
    'type
  if$
  "}" * *
  number empty.or.unknown
    { "t" change.case$ }
    %% LOOKS BAD: { "." * number tie.or.space.connect }
    %% Prefer "Research report RJ687." to "Research report. RJ687."
    { number tie.or.space.connect }
  if$
}

FUNCTION { format.advisor }
{
  advisor empty.or.unknown
    { "" }
    { "Advisor(s) " advisor * }
  if$
}

FUNCTION { format.article.crossref }
{ "See"
  "\citeN{" * crossref * "}" *
}

FUNCTION { format.crossref.editor }
{
  editor #1 "{vv~}{ll}" format.name$
  editor num.names$ duplicate$
  #2 >
    { pop$ " et~al\mbox{.}" * }         % jrh: avoid spacing problems
    { #2 <
    'skip$
    { editor #2 "{ff }{vv }{ll}{ jj}" format.name$ "others" =
        { " et~al\mbox{.}" * }          % jrh: avoid spacing problems
        { " and " * editor #2 "{vv~}{ll}" format.name$ * }
      if$
    }
      if$
    }
  if$
}

FUNCTION { format.book.crossref }
{
  volume empty.or.unknown
    { "empty volume in " cite$ * "'s crossref of " * crossref * warning$
      "In "
    }
    { "Volume" volume tie.or.space.connect % gnp - changed to mixed case
      " of " *
    }
  if$
  editor empty.or.unknown
  editor field.or.null author field.or.null =
  or
    { key empty.or.unknown
    { series empty.or.unknown
        { "need editor, key, or series for " cite$ * " to crossref " *
          crossref * warning$
          "" *
        }
        { series emphasize * }
      if$
    }
    { key * }
      if$
    }
    { format.crossref.editor * }
  if$
  " \citeN{" * crossref * "}" *
}

FUNCTION { format.incoll.inproc.crossref }
{ "See"
  " \citeN{" * crossref * "}" *
}

FUNCTION { format.lab.names }
{
  % format.lab.names:
  %
  % determines "short" names for the abbreviated author information.
  % "Long" labels are created in calc.label, using the routine my.full.label
  % to format author and editor fields.
  %
  % There are 4 cases for labels.   (n=3 in the example)
  % a) one author             Foo
  % b) one to n               Foo, Bar and Baz
  % c) use of "and others"    Foo, Bar et al.
  % d) more than n            Foo et al.

  's :=
  s num.names$ 'numnames :=
  numnames #2 >    % change number to number of others allowed before
                   % forcing "et al".
    { s #1 "{vv~}{ll}" format.name$ " et~al\mbox{.}" * } % jrh: \mbox{} added
    {
      numnames #1 - 'namesleft :=
      #2 'nameptr :=
      s #1 "{vv~}{ll}" format.name$
        { namesleft #0 > }
        { nameptr numnames =
            { s nameptr "{ff }{vv }{ll}{ jj}" format.name$ "others" =
                { " et~al\mbox{.}" * }          % jrh: avoid spacing problems
                { " and " * s nameptr "{vv~}{ll}" format.name$ * }
              if$
            }
            { ", " * s nameptr "{vv~}{ll}" format.name$ * }
          if$
          nameptr #1 + 'nameptr :=
          namesleft #1 - 'namesleft :=
        }
      while$
    }
  if$
}

FUNCTION { author.key.label }
{
  author empty.or.unknown
    { key empty.or.unknown
          { "no key, author in " cite$ * warning$
            cite$ #1 #3 substring$ }
         'key
      if$
    }
    { author format.lab.names }
  if$
}

FUNCTION { editor.key.organization.label }
{ % added - gnp. Provide label formatting by organization if editor is null.
  editor empty.or.unknown
    { organization empty.or.unknown
        { key empty.or.unknown
            { "no key, editor or organization in " cite$ * warning$
              cite$ #1 #3 substring$ }
            'key
          if$
        }
        { organization }
      if$
    }
    { editor format.lab.names }
  if$
}

FUNCTION { author.editor.key.label }
{
  author empty.or.unknown
    { editor empty.or.unknown
          { key empty.or.unknown
               { "no key, author, or editor in " cite$ * warning$
                 cite$ #1 #3 substring$ }
             'key
           if$
         }
          { editor format.lab.names }
      if$
    }
    { author format.lab.names }
  if$
}

FUNCTION { author.editor.key.organization.label }
{ % added - gnp. Provide label formatting by organization if author is null.
  author empty.or.unknown
    { editor empty.or.unknown
        { organization empty.or.unknown
            { key empty.or.unknown
               { "no key, author, editor or organization in " cite$ * warning$
                 cite$ #1 #3 substring$ }
               'key
              if$
            }
            { organization }
          if$
        }
        { editor format.lab.names }
      if$
    }
    { author format.lab.names }
  if$
}

% Calculate label and leave it on stack
FUNCTION { calc.basic.label }
{
  type$ "book" =
  type$ "inbook" =
  or
  type$ "article" =
  or
    'author.editor.key.label
    { type$ "proceedings" =
      type$ "periodical" =
      or
        'editor.key.organization.label
        { type$ "manual" =
            'author.editor.key.organization.label
            'author.key.label
          if$
        }
      if$
    }
  if$
  duplicate$
  year empty.or.unknown
    { "[n.\,d.]" }
    { year field.or.null purify$ #-1 #4 substring$}
  if$
  *
  'basic.label.year :=
}

FUNCTION { calc.label }
{
  % Changed - GNP. See also author.editor.organization.sort, editor.organization.sort
  % Form label for BibTeX entry. The classification of which fields are used
  % for which type of entry (book, inbook, etc.) are taken from alpha.bst.
  % The change here from newapa is to also include organization as a
  % citation label if author or editor is missing.

  calc.basic.label

  author empty.or.unknown  % generate the full label citation information.
    {
      editor empty.or.unknown
        {
          organization empty.or.unknown
            {
              key empty.or.unknown
                {
                  "no author, editor, organization, or key in " cite$ * warning$
                  "??"
                }
                { key }
              if$
            }
            { organization }
          if$
        }
        { editor my.full.label }
      if$
    }
    { author my.full.label }
  if$

  % leave label on the stack, to be popped when required.

  "}{" * swap$ * "}{" *
  %  year field.or.null purify$ #-1 #4 substring$ *
  %
  % save the year for sort processing afterwards (adding a, b, c, etc.)
  %
  year empty.or.unknown
    { "[n.\,d.]" }
    { year field.or.null purify$ #-1 #4 substring$}
  if$
  'label.year :=
}


FUNCTION { output.bibitem }
{
  newline$
  "\bibitem[\protect\citeauthoryear{" write$
  calc.label write$
  sort.year write$
  "}]%" writeln
  "        {" write$
  cite$ write$
  "}" writeln
  ""
  before.all 'output.state :=
}


FUNCTION { output.issue.doi.coden.isxn.lccn.url.eprint }
{ % enter and return with stack empty
  %% We switch now from buffered output to output of complete lines, so
  %% that the Issue .. URL data have their own lines, and are less likely
  %% to be line-wrapped by BibTeX's short-sighted algorithm, which wraps
  %% lines longer than 79 characters, backtracking to what it thinks is
  %% a break point in the string.  Any such wrapping MUST be undone to
  %% prevent percent-newline from appearing in DOIs and URLs.  The
  %% output data are intentionally wrapped in \showxxx{} macros at
  %% beginning of line, and that supply their own punctuation (if they
  %% are not defined to suppress output entirely), to make it easier for
  %% other software to recover them from .bbl files.
  %%
  %% It also makes it possible to later change the macro definitions
  %% to suppress particular output values, or alter their appearance.
  %%
  %% Note that it is possible for theses, technical reports, and
  %% manuals to have ISBNs, and anything that has an ISBN may also
  %% have an ISSN.  When there are no values for these keys, there
  %% is no output generated for them here.

  "\newblock" writeln
  after.block 'output.state :=

  output.issue
  output.isbn
  output.coden  % CODEN is functionally like ISSN, so output them sequentially
  output.issn
  output.lccn
  output.eprint
  output.doi    % DOI is ALWAYS last according to CrossRef DOI documentation
  output.url    % but ACM wants URL last
}

FUNCTION { output.issue.doi.coden.isxn.lccn.url.eprint.note }
{ % enter with stack empty, return with empty string on stack
  output.issue.doi.coden.isxn.lccn.url.eprint
  note empty.or.unknown
    { }
    {
      "\newblock" writeln
      output.note
    }
  if$
  ""
}

FUNCTION { output.issue.doi.coden.isxn.lccn.url.eprint.note.check }
{ % enter with stack empty, return with empty string on stack
  output.issue.doi.coden.isxn.lccn.url.eprint
  note empty.or.unknown
    { }
    {
      "\newblock" writeln
      output.note.check
    }
  if$
  ""
}

FUNCTION { article }
{
  output.bibitem

  author empty.or.unknown
    {
      editor empty.or.unknown
        { "neither author and editor supplied for " cite$ * warning$ }
        { format.editors "editor" output.check }
      if$
    }
    { format.authors "author" output.check }
  if$

  author format.no.key output       % added
  output.year.check                 % added
  new.block
  format.articletitle "title" output.check
  new.block
  howpublished empty.or.unknown
    { }
    { "\bibinfo{howpublished}{" howpublished "}" * * output }
  if$

  crossref missing$
    { format.journal.volume.number.day.month.year output}
    {
      "cross reference in @Article{...} is unusual" warning$
      format.article.crossref output.nonnull
    }
  if$

  format.pages.check.without.articleno output
  format.articleno.numpages output
  fin.block
  output.issue.doi.coden.isxn.lccn.url.eprint.note
  fin.entry
}

FUNCTION { book }
{
  output.bibitem
  author empty.or.unknown
    { format.editors "author and editor" output.check }
    { format.authors output.nonnull
      crossref missing$
        { "author and editor" editor either.or.check }
        'skip$
      if$
    }
  if$
  output.year.check       % added
  new.block
  format.btitle "title" output.check
  crossref missing$
    { new.sentence              % jtb: start a new sentence for series/volume
      format.bvolume output
      new.block
      format.number.series output
      new.sentence
      publisher "publisher" bibinfo.output.check
      address "address" bibinfo.output.check    % jtb: require address
      fin.sentence
      pages empty.or.unknown
        { format.bookpages }    % use bookpages when pages empty
        { format.pages.check "pages" tie.or.space.connect }
      if$
      output
    }
    { new.block
      format.book.crossref output.nonnull
    }
  if$
  fin.block
  output.issue.doi.coden.isxn.lccn.url.eprint.note
  fin.entry
}

FUNCTION { booklet }
{
  output.bibitem
  format.authors output
  author format.key output          % added
  output.year.check                 % added
  new.block
  format.title "title" output.check
  new.block
    howpublished empty.or.unknown
    { }
    { "\bibinfo{howpublished}{" howpublished "}" * * output }
  if$
  address output
  fin.block
  output.issue.doi.coden.isxn.lccn.url.eprint.note
  fin.entry
}

FUNCTION { inbook }
{
  output.bibitem
  author empty.or.unknown
    { format.editors
      "author and editor" output.check
    }
    { format.authors output.nonnull
      crossref missing$
    { "author and editor" editor either.or.check }
    'skip$
      if$
    }
  if$
  output.year.check                 % added
  new.block
  format.btitle "title" output.check
  crossref missing$
    { new.sentence              % jtb: start a new sentence for series/volume
      format.bvolume output
      new.block
      format.number.series output
      new.sentence
      publisher "publisher" bibinfo.output.check
      address "address" bibinfo.output.check    % jtb: require address
      format.bookpages output
      format.chapter.pages
      "chapter and pages" output.check  % jtb: moved from before publisher
    }
    {
      format.bookpages output
      format.chapter.pages "chapter and pages" output.check
      new.block
      format.book.crossref output.nonnull
    }
  if$
  fin.block
  output.issue.doi.coden.isxn.lccn.url.eprint.note
  fin.entry
}

FUNCTION { incollection }
{
  output.bibitem
  format.authors "author" output.check
  author format.key output       % added
  output.year.check              % added
  new.block
  format.articletitle "title" output.check
  new.block
  crossref missing$
    { format.in.ed.booktitle "booktitle" output.check
      new.sentence                % jtb: start a new sentence for series/volume
      format.bvolume output
      format.number.series output
      new.sentence
      publisher "publisher" bibinfo.output.check
      address "address" bibinfo.output.check      % jtb: require address
      format.bookpages output
      format.chapter.pages output % gnp - was special.output.nonnull
                                  % left out comma before page numbers
                                  % jtb: moved from before publisher
    }
    {
      format.incoll.inproc.crossref output.nonnull
      format.chapter.pages output
    }
  if$
  fin.block
  output.issue.doi.coden.isxn.lccn.url.eprint.note
  fin.entry
}

FUNCTION { inproceedings }
{
  output.bibitem
  format.authors "author" output.check
  author format.key output            % added
  output.year.check                   % added
  new.block
  format.articletitle "title" output.check
  howpublished empty.or.unknown
    { }
    { "\bibinfo{howpublished}{" howpublished "}" * * output.dot.space }
  if$
  crossref missing$
    {
      journal missing$          % jtb: proceedings appearing in journals
        { format.in.emphasize.booktitle format.city "booktitle"  output.check.dot.space
          format.series output.removenospace
          format.editors.fml output % BV 2011/09/27 Moved dot to comma
          series empty.or.unknown
              { format.bvolume.noseries output }
              {}
          if$
          new.sentence
          organization output
          publisher "publisher" bibinfo.output.check % jtb: require publisher (?)
          address "address" bibinfo.output.check  % jtb: require address
          format.bookpages output
        }
        {
           format.in.booktitle format.city "booktitle" output.check
           format.editors.fml output
           new.sentence
           format.journal.volume.number.day.month.year output
        }
      if$
      format.articleno output
      format.pages.check.without.articleno output
    }
    {
      format.incoll.inproc.crossref output.nonnull
      format.articleno output
      format.pages.check.without.articleno output
    }
  if$
  format.articleno.numpages output
  fin.block
  output.issue.doi.coden.isxn.lccn.url.eprint.note
  fin.entry
}

FUNCTION { conference } { inproceedings }

FUNCTION { manual }
{
  output.bibitem
  author empty.or.unknown
    { editor empty.or.unknown
      { organization "organization" output.check
        organization format.key output }  % if all else fails, use key
      { format.editors "author and editor" output.check }
      if$
    }
    { format.authors output.nonnull }
    if$
  output.year.check                 % added
  new.block
  format.btitle "title" output.check
  organization address new.block.checkb
  % jtb: back to normal style: organization, address
  organization "organization" output.check
  address output
  fin.block
  output.issue.doi.coden.isxn.lccn.url.eprint.note
  fin.entry
}

FUNCTION { mastersthesis }
{
  output.bibitem
  format.authors "author" output.check
  author format.key output          % added
  output.year.check                 % added
  new.block
  format.title emphasize "title" output.check  % NB: ACM style requires emphasized thesis title
  new.block
  "\bibinfo{thesistype}{Master's\ thesis}" format.thesis.type output
  new.sentence
  school "school" bibinfo.output.check
  address empty.or.unknown
     { }
     { "\bibinfo{address}{" address * "}" * output }
  if$
  new.block
  format.advisor output
  fin.block
  output.issue.doi.coden.isxn.lccn.url.eprint.note
  fin.entry
}

FUNCTION { misc }
{
  output.bibitem
  format.authors "author" output.check
  author format.key output            % added
  output.year.check                   % added
  title howpublished new.block.checkb
  format.title output
  new.block
  howpublished empty.or.unknown
    { }
    { "\bibinfo{howpublished}{" howpublished "}" * * output }
  if$
  "" output.nonnull.dot.space
  calc.format.page.count output
  fin.block
  output.issue.doi.coden.isxn.lccn.url.eprint.note
  fin.entry
}

FUNCTION { online } { manual }

FUNCTION { game } { manual }

FUNCTION { artifactsoftware } { manual }

FUNCTION { artifactdataset } { manual }

FUNCTION { software } { manual }

FUNCTION { dataset } { manual }

FUNCTION { phdthesis }
{
  output.bibitem
  format.authors "author" output.check
  author format.key output          % added
  output.year.check                 % added
  new.block
  format.title emphasize "title" output.check  % NB: ACM style requires emphasized thesis title
  new.block
  "\bibinfo{thesistype}{Ph.\,D. Dissertation}" format.thesis.type output
  new.sentence
  school "school" bibinfo.output.check
  address empty.or.unknown
     { }
     { "\bibinfo{address}{" address * "}" * output }
  if$
  new.block
  format.advisor output
  fin.block
  output.issue.doi.coden.isxn.lccn.url.eprint.note
  fin.entry
}

FUNCTION {format.date}
{ year empty.or.unknown
    { month empty.or.unknown
        {
          ""                    % output empty date if year/month both empty
          day empty.or.unknown
            {  }
            { "there's a day but no month or year in " cite$ * warning$ }
          if$
        }
        { "there's a month but no year in " cite$ * warning$
          month
          day empty.or.unknown
            { }
            { " " * day * }
          if$
        }
      if$
    }
    { month empty.or.unknown
        {
          year                  % output only year if month empty
          day empty.or.unknown
            {  }
            { "there's a day and year but no month in " cite$ * warning$ }
          if$
        }
        {
          month " " *
          day empty.or.unknown
            { }
            { day * ", " * }
          if$
          year *
        }
      if$
    }
  if$
}

FUNCTION {new.block.checka}
{
  empty.or.unknown
    'skip$
    'new.block
  if$
}

FUNCTION { periodical }
{
  output.bibitem
  editor empty.or.unknown
    { organization output }
    { format.editors output.nonnull }
  if$
  new.block
  output.year.check
  new.sentence
  format.articletitle "title" output.check
  format.journal.volume.number.day.month.year output
  calc.format.page.count output
  fin.entry
}

FUNCTION { proceedings }
{
  output.bibitem
  editor empty.or.unknown
    { organization output
      organization format.key output }  % gnp - changed from author format.key
    { format.editors output.nonnull }
  if$
  % author format.key output             % gnp - removed (should be either
  %                                        editor or organization
  output.year.check                    % added (newapa)
  new.block
  format.btitle format.city "title" output.check        % jtb: added city
  new.sentence
  format.bvolume output
  format.number.series output
  new.sentence
  organization output
  % jtb: normal order: publisher, address
  publisher empty.or.unknown
     { }
     { "\bibinfo{publisher}{" publisher * "}" * output }
  if$
  address empty.or.unknown
     { }
     { "\bibinfo{address}{" address * "}" * output }
  if$
  fin.block
  output.issue.doi.coden.isxn.lccn.url.eprint.note
  fin.entry
}

FUNCTION { collection } { proceedings }

FUNCTION { techreport }
{
  output.bibitem
  format.authors "author" output.check
  author format.key output             % added
  output.year.check                    % added
  new.block
  format.btitle "title" output.check
  new.block
%   format.tr.number output               % jtb: moved month ...
  format.tr.number output new.sentence    % Gerry  - need dot 2011/09/28
  institution "institution" bibinfo.output.check
  address empty.or.unknown
    { }
    { "\bibinfo{address}{" address "}" * * output }
  if$
  new.sentence
  format.named.pages output
  % ACM omits year at end in transactions style
  % format.day.month.year output.nonnull.dot.space  % jtb: ... to here (no parens)
  fin.block
  output.issue.doi.coden.isxn.lccn.url.eprint.note
  fin.entry
}

FUNCTION { unpublished }
{
  output.bibitem
  format.authors
  "author" output.check
  author format.key output              % added
  output.year.check                     % added
  new.block
  format.title "title" output.check
  fin.sentence
  output.day.month.year                 % UTAH
  calc.format.page.count output
  fin.block
  output.issue.doi.coden.isxn.lccn.url.eprint.note.check
  fin.entry
}

FUNCTION { default.type } { misc }

%%% ACM journal-style month definitions: full name if 1--5 letters, else
%%% abbreviation of 3 or 4 characters and a dot

MACRO {jan}             {"Jan."}

MACRO {feb}             {"Feb."}

MACRO {mar}             {"March"}

MACRO {apr}             {"April"}

MACRO {may}             {"May"}

MACRO {jun}             {"June"}

MACRO {jul}             {"July"}

MACRO {aug}             {"Aug."}

MACRO {sep}             {"Sept."}

MACRO {oct}             {"Oct."}

MACRO {nov}             {"Nov."}

MACRO {dec}             {"Dec."}

%%% ACM journal names

MACRO {cie}  {"ACM Computers in Entertainment"}
MACRO {csur}  {"ACM Computing Surveys"}
MACRO {dgov}  {"Digital Government: Research and Practice"}
MACRO {dtrap}  {"Digital Threats: Research and Practice"}
MACRO {health}  {"ACM Transactions on Computing for Healthcare"}
MACRO {imwut}  {"PACM on Interactive, Mobile, Wearable and Ubiquitous Technologies"}
MACRO {jacm}  {"Journal of the ACM"}
MACRO {jdiq}  {"ACM Journal of Data and Information Quality"}
MACRO {jea}  {"ACM Journal of Experimental Algorithmics"}
MACRO {jeric}  {"ACM Journal of Educational Resources in Computing"}
MACRO {jetc}  {"ACM Journal on Emerging Technologies in Computing Systems"}
MACRO {jocch}  {"ACM Journal on Computing and Cultural Heritage"}
MACRO {pacmcgit}  {"Proceedings of the ACM on Computer Graphics and Interactive Techniques"}
MACRO {pacmhci}  {"PACM on Human-Computer Interaction"}
MACRO {pacmpl}  {"PACM on Programming Languages"}
MACRO {pomacs}  {"PACM on Measurement and Analysis of Computing Systems"}
MACRO {taas}  {"ACM Transactions on Autonomous and Adaptive Systems"}
MACRO {taccess}  {"ACM Transactions on Accessible Computing"}
MACRO {taco}  {"ACM Transactions on Architecture and Code Optimization"}
MACRO {talg}  {"ACM Transactions on Algorithms"}
MACRO {tallip}  {"ACM Transactions on Asian and Low-Resource Language Information Processing"}
MACRO {tap}  {"ACM Transactions on Applied Perception"}
MACRO {tcps}  {"ACM Transactions on Cyber-Physical Systems"}
MACRO {tds}  {"ACM/IMS Transactions on Data Science"}
MACRO {teac}  {"ACM Transactions on Economics and Computation"}
MACRO {tecs}  {"ACM Transactions on Embedded Computing Systems"}
MACRO {telo}  {"ACM Transactions on Evolutionary Learning"}
MACRO {thri}  {"ACM Transactions on Human-Robot Interaction"}
MACRO {tiis}  {"ACM Transactions on Interactive Intelligent Systems"}
MACRO {tiot}  {"ACM Transactions on Internet of Things"}
MACRO {tissec}  {"ACM Transactions on Information and System Security"}
MACRO {tist}  {"ACM Transactions on Intelligent Systems and Technology"}
MACRO {tkdd}  {"ACM Transactions on Knowledge Discovery from Data"}
MACRO {tmis}  {"ACM Transactions on Management Information Systems"}
MACRO {toce}  {"ACM Transactions on Computing Education"}
MACRO {tochi}  {"ACM Transactions on Computer-Human Interaction"}
MACRO {tocl}  {"ACM Transactions on Computational Logic"}
MACRO {tocs}  {"ACM Transactions on Computer Systems"}
MACRO {toct}  {"ACM Transactions on Computation Theory"}
MACRO {todaes}  {"ACM Transactions on Design Automation of Electronic Systems"}
MACRO {tods}  {"ACM Transactions on Database Systems"}
MACRO {tog}  {"ACM Transactions on Graphics"}
MACRO {tois}  {"ACM Transactions on Information Systems"}
MACRO {toit}  {"ACM Transactions on Internet Technology"}
MACRO {tomacs}  {"ACM Transactions on Modeling and Computer Simulation"}
MACRO {tomm}   {"ACM Transactions on Multimedia Computing, Communications and Applications"}
MACRO {tompecs}  {"ACM Transactions on Modeling and Performance Evaluation of Computing Systems"}
MACRO {toms}  {"ACM Transactions on Mathematical Software"}
MACRO {topc}  {"ACM Transactions on Parallel Computing"}
MACRO {toplas}  {"ACM Transactions on Programming Languages and Systems"}
MACRO {tops}  {"ACM Transactions on Privacy and Security"}
MACRO {tos}  {"ACM Transactions on Storage"}
MACRO {tosem}  {"ACM Transactions on Software Engineering and Methodology"}
MACRO {tosn}  {"ACM Transactions on Sensor Networks"}
MACRO {tqc}  {"ACM Transactions on Quantum Computing"}
MACRO {trets}  {"ACM Transactions on Reconfigurable Technology and Systems"}
MACRO {tsas}  {"ACM Transactions on Spatial Algorithms and Systems"}
MACRO {tsc}  {"ACM Transactions on Social Computing"}
MACRO {tslp}  {"ACM Transactions on Speech and Language Processing"}
MACRO {tweb}  {"ACM Transactions on the Web"}

%%% Some traditional macros
MACRO {acmcs} {"ACM Computing Surveys"}

MACRO {acta} {"Acta Informatica"}

MACRO {cacm} {"Communications of the ACM"}

MACRO {ibmjrd} {"IBM Journal of Research and Development"}

MACRO {ibmsj} {"IBM Systems Journal"}

MACRO {ieeese} {"IEEE Transactions on Software Engineering"}

MACRO {ieeetc} {"IEEE Transactions on Computers"}

MACRO {ieeetcad}
 {"IEEE Transactions on Computer-Aided Design of Integrated Circuits"}

MACRO {ipl} {"Information Processing Letters"}

MACRO {jcss} {"Journal of Computer and System Sciences"}

MACRO {scp} {"Science of Computer Programming"}

MACRO {sicomp} {"SIAM Journal on Computing"}

MACRO {toois} {"ACM Transactions on Office Information Systems"}

MACRO {tcs} {"Theoretical Computer Science"}



READ

FUNCTION { sortify }
{
  purify$
  "l" change.case$
}

FUNCTION { chop.word }
{
  's :=
  'len :=
  s #1 len substring$ =
    { s len #1 + global.max$ substring$ }
    's
  if$
}

FUNCTION { sort.format.names }
{
  's :=
  #1 'nameptr :=
  ""
  s num.names$ 'numnames :=
  numnames 'namesleft :=
    { namesleft #0 > }
    { nameptr #1 >
          { "   " * }
         'skip$
      if$
      s nameptr "{vv{ } }{ll{ }}{  f{ }}{  jj{ }}" format.name$ 't :=
      nameptr numnames = t "others" = and
          { " et~al" * }
          { t sortify * }
      if$
      nameptr #1 + 'nameptr :=
      namesleft #1 - 'namesleft :=
    }
  while$
}

FUNCTION { sort.format.title }
{
  't :=
  "A " #2
    "An " #3
      "The " #4 t chop.word
    chop.word
  chop.word
  sortify
  #1 global.max$ substring$
}

FUNCTION { author.sort }
{
  author empty.or.unknown
    { key empty.or.unknown
         { "to sort, need author or key in " cite$ * warning$
           "" }
         { key sortify }
      if$
    }
    { author sort.format.names }
  if$
}

FUNCTION { author.editor.sort }
{
  author empty.or.unknown
    {
      editor empty.or.unknown
         {
           key empty.or.unknown
             { "to sort, need author, editor, or key in " cite$ * warning$
               ""
             }
             { key sortify }
           if$
         }
         { editor sort.format.names }
      if$
    }
    { author sort.format.names }
  if$
}

FUNCTION { editor.organization.sort }
{
  % added - GNP. Stack editor or organization for sorting (from alpha.bst).
  % Unlike alpha.bst, we need entire names, not abbreviations

  editor empty.or.unknown
    { organization empty.or.unknown
        { key empty.or.unknown
            { "to sort, need editor, organization, or key in " cite$ * warning$
              ""
            }
            { key sortify }
          if$
        }
        { organization sortify }
      if$
    }
    { editor sort.format.names }
  if$
}

FUNCTION { author.editor.organization.sort }
{
  % added - GNP. Stack author or organization for sorting (from alpha.bst).
  % Unlike alpha.bst, we need entire names, not abbreviations

  author empty.or.unknown
    {
      editor empty.or.unknown
        { organization empty.or.unknown
            { key empty.or.unknown
                { "to sort, need author, editor, or key in " cite$ * warning$
                ""
                }
                { key sortify }
              if$
            }
            { organization sortify }
          if$
        }
        { editor sort.format.names }
      if$
    }
    { author sort.format.names }
  if$
}

FUNCTION { presort }
{
  % Presort creates the bibentry's label via a call to calc.label, and then
  % sorts the entries based on entry type. Chicago.bst adds support for
  % including organizations as the sort key; the following is stolen from
  % alpha.bst.

  calc.label
  basic.label.year
  swap$
  "    "
  swap$
  * *
  "    "
  *
  sortify
  year field.or.null purify$ #-1 #4 substring$ * % add year
  "    "
  *
  type$ "book" =
  type$ "inbook" =
  or
  type$ "article" =
  or
    'author.editor.sort
    { type$ "proceedings" =
      type$ "periodical" =
      or
        'editor.organization.sort
        { type$ "manual" =
            'author.editor.organization.sort
            'author.sort
          if$
        }
      if$
    }
  if$
  #1 entry.max$ substring$        % added for newapa
  'sort.label :=                  % added for newapa
  sort.label                      % added for newapa
  *
  "    "
  *
  title field.or.null
  sort.format.title
  *
  #1 entry.max$ substring$
  'sort.key$ :=
}



ITERATE { presort }

SORT             % by label, year, author/editor, title

% From plainnat.bst
STRINGS { longest.label }

INTEGERS { longest.label.width number.label }

FUNCTION {initialize.longest.label}
{ "" 'longest.label :=
  #0 int.to.chr$ 'last.label :=
  "" 'next.extra :=
  #0 'longest.label.width :=
  #0 'last.extra.num :=
  #0 'number.label :=
}



FUNCTION { initialize.extra.label.stuff }
{ #0 int.to.chr$ 'last.label :=
  "" 'next.extra :=
  #0 'last.extra.num :=
}

FUNCTION { forward.pass }
{
  % Pass through all entries, comparing current entry to last one.
  % Need to concatenate year to the stack (done by calc.label) to determine
  % if two entries are the same (see presort)

  last.label
  calc.basic.label year field.or.null purify$ #-1 #4 substring$ * % add year
  #1 entry.max$ substring$ =     % are they equal?
     { last.extra.num #1 + 'last.extra.num :=
       last.extra.num int.to.chr$ 'extra.label :=
     }
     { "a" chr.to.int$ 'last.extra.num :=
       "" 'extra.label :=
       calc.basic.label year field.or.null purify$ #-1 #4 substring$ * % add year
       #1 entry.max$ substring$ 'last.label := % assign to last.label
     }
  if$
  number.label #1 + 'number.label :=
}

FUNCTION { reverse.pass }
{
  next.extra "b" =
    { "a" 'extra.label := }
     'skip$
  if$
  label.year extra.label * 'sort.year :=
  extra.label 'next.extra :=
}

EXECUTE {initialize.extra.label.stuff}
EXECUTE {initialize.longest.label}


ITERATE {forward.pass}

REVERSE {reverse.pass}

FUNCTION { bib.sort.order }
{
  sort.label
  "    "
  *
  year field.or.null sortify
  *
  "    "
  *
  title field.or.null
  sort.format.title
  *
  #1 entry.max$ substring$
  'sort.key$ :=
}

ITERATE { bib.sort.order }

SORT             % by sort.label, year, title --- giving final bib. order.

FUNCTION { begin.bib }
{
  %% Set to #0 show 13-digit ISBN in preference to 10-digit ISBN.
  %% Set to #1 to show both 10-digit and 13-digit ISBNs.
  #1 'show-isbn-10-and-13 :=

  "%%% -*-BibTeX-*-" writeln
  "%%% Do NOT edit. File created by BibTeX with style" writeln
  "%%% ACM-Reference-Format-Journals [18-Jan-2012]." writeln
  "" writeln

  preamble$ empty.or.unknown
    'skip$
    { preamble$ writeln }
  if$
  "\begin{thebibliography}{" number.label int.to.str$ * "}" * writeln
  ""                                                                         writeln
  "%%% ====================================================================" writeln
  "%%% NOTE TO THE USER: you can override these defaults by providing"       writeln
  "%%% customized versions of any of these macros before the \bibliography"  writeln
  "%%% command.  Each of them MUST provide its own final punctuation,"       writeln
  "%%% except for \shownote{}, \showDOI{}, and \showURL{}.  The latter two"  writeln
  "%%% do not use final punctuation, in order to avoid confusing it with"    writeln
  "%%% the Web address."                                                     writeln
  "%%%"                                                                      writeln
  "%%% To suppress output of a particular field, define its macro to expand" writeln
  "%%% to an empty string, or better, \unskip, like this:"                   writeln
  "%%%"                                                                      writeln
  "%%% \newcommand{\showDOI}[1]{\unskip}   % LaTeX syntax"                   writeln
  "%%%"                                                                      writeln
  "%%% \def \showDOI #1{\unskip}           % plain TeX syntax"               writeln
  "%%%"                                                                      writeln
  "%%% ====================================================================" writeln
  ""                                                                         writeln

  %% ACM publications do not use CODEN, ISSN, and LCCN data, so their default
  %% macro wrappers expand to \unskip, discarding their values and unwanted
  %% space.
  %%
  %% For other publications, prior definitions like these may be useful:
  %%
  %%     Plain TeX:
  %%         \def \showCODEN     #1{CODEN #1.}
  %%         \def \showISSN      #1{ISSN #1.}
  %%         \def \showLCCN      #1{LCCN #1.}
  %%
  %%     LaTeX:
  %%         \newcommand{\showCODEN}[1]{CODEN #1.}
  %%         \newcommand{\showISSN}[1]#1{ISSN #1.}
  %%         \newcommand{\showLCCN}[1]{LCCN #1.}

  "\ifx \showCODEN    \undefined \def \showCODEN     #1{\unskip}     \fi" writeln
  % \showDOI changed by Ziv (just to add a period)
  "\ifx \showDOI      \undefined \def \showDOI       #1{#1.}\fi" writeln
  % ACM styles omit ISBNs, but they can be included by suitable definitions of
  % \showISBNx and \showISBNxiii before the .bbl file is read
  "\ifx \showISBNx    \undefined \def \showISBNx     #1{\unskip}     \fi" writeln
  "\ifx \showISBNxiii \undefined \def \showISBNxiii  #1{\unskip}     \fi" writeln
  "\ifx \showISSN     \undefined \def \showISSN      #1{\unskip}     \fi" writeln
  "\ifx \showLCCN     \undefined \def \showLCCN      #1{\unskip}     \fi" writeln
  "\ifx \shownote     \undefined \def \shownote      #1{#1}          \fi" writeln % NB: final period supplied by add.period$ above
  "\ifx \showarticletitle \undefined \def \showarticletitle #1{#1}   \fi" writeln
  % \showURL changed by Ziv to \unskip
  "\ifx \showURL      \undefined \def \showURL       #1{\unskip}     \fi" writeln
  "% The following commands are used for tagged output and should be " writeln
  "% invisible to TeX" writeln
  "\providecommand\bibfield[2]{#2}" writeln
  "\providecommand\bibinfo[2]{#2}" writeln
  "\providecommand\natexlab[1]{#1}" writeln
  "" writeln
  % \showeprint changed by Ziv
  "\providecommand\showeprint[3]{\hrefeprint{#1}{#2}{#1:\texttt{#2}}.}" writeln
  "\providecommand\hrefeprint[3]{%" writeln
  "  \IfEqCase{#1}{%" writeln
  "    {arXiv}{\href{https://arxiv.org/abs/#2}{#3}}%" writeln
  "    {arxiv}{\href{https://arxiv.org/abs/#2}{#3}}%" writeln
  "  }[#3]%" writeln
  "}" writeln
  "\DeclareUrlCommand\doi{\urlstyle{same}%" writeln
  "  \def\UrlLeft##1\UrlRight{\href{https://doi.org/##1}{doi:\texttt{##1}}}}" writeln
}

EXECUTE {begin.bib}

EXECUTE {init.state.consts}

ITERATE {call.type$}

FUNCTION { end.bib }
{
  newline$
  "\end{thebibliography}"
  writeln
}

EXECUTE {end.bib}


==> old/main_results.tex <==
\subsection{Tail asymptotics for arbitrary boost functions.}
\george{Maybe this subsection goes first. (5->7) in order.} In \cref{sec:tail_asymptotics} we derive \cref{lem:transform_ratio}, which allows us to compute the ratio of the asymptotic coefficients for an arbitrary boost policy $r(S)$ wrt $C_\fcfs$. Using this expression for the optimal boost policy, we can show that this ratio is less than one.

\begin{lemma}
    For arbitrary $\epsilon > 0$, define the event $L = \{ \epsilon\text{-large}, W(-r_{\gamma - \epsilon}(S)) > r_{\gamma - \epsilon}(S) \}$, define $WC(r) = V((-\infty, a - r(S)), (a - r(S), \infty))$. Let $C_{r} = \frac{1}{\gamma}\lim_{\theta\to\gamma} (\gamma - \theta) \E*{ e^{\theta T_{r}}}$ and $C_{FCFS} = \frac{1}{\gamma}\lim_{\theta \to \gamma} (\gamma - \theta) \E*{e^{\theta T_{FCFS}}}$. Then:
    \[
        \label{eq:transform_ratio}
        \frac{C_r}{C_{FCFS}} = \frac{\E*{e^{\gamma (S - r(S))}} e^{\lambda\E*{r(S)\gp*{e^{\gamma S} - 1}}}}{\E*{e^{\gamma S}}}
    \]
\end{lemma}

\george{We may not need work-crossing if we are looking at bounded boost policies (still working through the details for the transform).}

\subsection{Deriving the optimal boost policy.}
The definition of boost policies given in \cref{sec:model} is general and admits a variety of possible boost functions (e.g. $r(s) = 1 / s$). Our main goal is to show that within this family of policies, there is a policy that gives the optimal asymptotic tail performance for Class~I distributions.

In \cref{sec:sample_path}, we derive the form of the optimal boost function,
\[
    r_\beta(s) = \frac{1}{\beta}\log \frac{1}{1 - e^{-\beta s}},
\]
with $\beta = \gamma$. This is done by observing that optimizing the transform of the response time is equivalent to optimizing the transform under certain conditions (i.e. cheating policy conditions). We then optimize the transform via an interchange argument which finds an optimal service order for the jobs based on their arrival times and sizes. This is formalized via sample-path analysis in \cref{sec:sample_path}.

\subsection{Proving optimality of the derived policy.}
\george{We may change this to proving optimality of the bounded boost policy frst? And put the unbounded boost case in the appendix.}
Our main result is to show that the boost policy characterized by the above boost function minimizes \cref{eq:asymptotic_tail_ratio}. We prove \cref{thm:optimality_thm} in \cref{sec:optimality}, answering an open question as to the form of the asymptotically optimal policy for Class~I job distributions. We briefly discuss several key ideas in the proof below.

\begin{theorem}\label{thm:optimality_thm}
    Suppose that $S$ is a Class~I job size distribution, with asymptotic tail decay rate $\gamma$, and let $C_\pi$ denote the asymptotic coefficient, as in \cref{eq:asymptotic_constant_def}. Then for any work-conserving, nonanticipative policy $\pi$, \[
        C_\pi - C_\boost{\gamma} \geq 0.
    \]
\end{theorem}

\textbf{Idea of cheating policies and cheating jobs.} To prove \cref{thm:optimality_thm} we introduce the idea of cheating policies, which are policies which can serve jobs \textit{before their arrival time}. In particular, the \textit{cheating variant} of a boost policy is the policy that, for each busy period of jobs, serves those jobs in order of boosted arrival time, allocating service at the start of the busy period, regardless of arrival time.
\textbf{Lower bound using sample-path analysis + cheating jobs.} We observe that a cheating version of a boost policy using the form of the optimal boost derived in \cref{sec:sample_path} must optimize the transform compared to any non-cheating policy.
\textbf{Legit = cheating and getting the actual lower bound.} It then suffices to show that asymptotically, the non-cheating version of the optimal boost policy has asymptotically equivalent performance to the cheating version of the optimal boost policy. Since the policy is characterized by its choice of $\beta$, we must look at the sequence of policies as $\theta\to\gamma$. Specifically, we must show the following:
\[
    \limsup_{\theta\to\gamma} (\gamma - \theta) \E*{e^{\theta T_\cheat{\gamma}} - e^{\theta T_\cheat{\theta}}}\leq 0,
\]
where $\cheat{\beta}$ is the optimal boost function with parameter $\beta$. We show that this sequence converges to the asymptotic limit given by taking $\beta = \gamma$, proving optimality.


==> old/optimality.tex <==
In this section we will first show that the asymptotic coefficient of a boost policy is the same as the asymptotic coefficient of its cheating variant. We then show that for a family of boost policies that share the same boost function, parameterized by $\beta$, that their performance converges. Formally, we show that:

\begin{lemma}\label{lem:legit_cheating_convergence}
Consider a non-cheating boost policy defined by boost function $r$ and its cheating variant defined as $\cheat{r}$. Then:
    \[
        \limsup_{\theta \to \gamma} (\gamma - \theta) \E*{e^{\theta T_r} - e^{\theta T_{\cheat{r}}}} \leq 0.
    \]
\end{lemma}

\begin{lemma}\label{lem:gamma_theta_convergence}
\george{This is the known sizes version.} Consider the boost policies defined by the family of boost functions
\[
    r_\beta(s) = \frac{1}{\beta}\log\gp*{\frac{1}{1 - e^{-\theta s}}},
\]
parameterized by $\beta$. Consider the cheating varirant of each boost policy, denoted by $\cheat{\beta}$. Then we have
\[
    \limsup_{\theta\to\gamma} (\gamma - \theta) \E*{e^{\theta T_{\cheat{\gamma}}} - e^{\theta T_{\cheat{\theta}}}} \leq 0.
\]
% \george{I think we do want to actually prove this specifically for the optimal boost function. For the arrivals part of the lemma we want a function of $r_{max}$ but it's hard to characterize that function without characterizing how the boost function varies with $L$.}. For a family of boost policies defined by boost function $r_\beta$, with parameter $\beta > 0$, s/t $\alpha \leq \beta \implies r_\alpha(l) \geq r_\beta(l)$, consider their cheating variants, denoted by $\cheat{\beta}$. Suppose that there exists a $\beta' < \gamma$ s/t for all $\beta \geq \beta'$, the work-crossing of $r_\beta$ is finite, and that $r_\beta (l)$ is continuous in $\beta\geq \beta'$ for all $l$. \george{I think we want cheating specifically here so that we can use the full work crossing for both $\cheat{\gamma}$ and $\cheat{\theta}$ terms. Otherwise we have to deal with departure time for e.g. $\cheat{\theta}$ b/c we want a lower bound for that term. Also, maybe we want to make some of these conditions part of the boost function definition?} Then we have:
    % \[
    %     \limsup_{\theta\to\gamma} (\gamma - \theta) \E*{e^{\theta T_{\cheat{\gamma}}} - e^{\theta T_{\cheat{\theta}}}} \leq 0.
    % \]
\end{lemma}

\subsection{Proof of \cref{lem:legit_cheating_convergence}}
We begin by proving the following lemma:

\george{We might not need $r_{max}$ here or in \cref{lem:legit_cheating_convergence}.}
\begin{lemma}\label{lem:legit_leq_cheat_for_noncheating_job}
    Consider an arbitrary $r_{max} > 0$. Then:
    \[
        \E*{e^{\theta T_r} \1\gp*{W(-r(L)) > r(L), r(L) \leq r_{max}}} \leq \E*{e^{\theta T_\cheat{r}} \1\gp*{W(-r(L)) > r(L), r(L) \leq r_{max}}}.
    \]
\end{lemma}

\begin{proof}
    We perform a sample-path analysis. Consider the tagged job, with label $L$ s/t $r(L) \leq r_{max}$. The response time under the boost policy characterized by $r$ is going to be a) service provided to the amount of work that arrived before the tagged job with lower boosted arrival time, plus b) service provided to the work that arrives after the tagged job with lower boosted arrival time, that arrives before the tagged job departs, plus the size of the job itself. a) is given by $W(-r(L)) - r(L) + V_r((-\infty, -r(L)), (-r(L), 0))$, and b) is given by a subset of $V_r((-\infty, -r(L)), (0, B))$, where $B$ denotes the end of the busy period of arrivals. In particular, note that no arrivals in time $(-r(L), 0)$ with boosted arrival time after $-r(L)$ receive service, due to the condition $W(-r(L)) > r(L)$. Therefore, $W(-r(L)) - r(L) + V_r((-\infty, -r(L)), (-r(L), B)) + S$ is an upper bound to the response time of the tagged job.

    Now consider the cheating version of the boost policy characterized by $r$. The response time under this policy is going to be given by a) the amount of work that arrived before the tagged job with lower boosted arrival time, plus b) all the work that arrives after the tagged job with lower boosted arrival time, plus the size of the job itself. Under the conditions $W(-r(L)) > r(L)$, we still have that a) is given by $W(-r(L)) - r(L) + V_r((-\infty, -r(L)), (-r(L), 0))$ and now b) is given exactly by $V_r((-\infty, -r(L)), (0, B))$. So the upper bound above is exactly the response time of the tagged job under the cheating system.
\end{proof}

\begin{proof}[Proof of \cref{lem:legit_cheating_convergence}.]
    For any arbitrary $r_{max} > 0$, we can write:
    \[
        \E*{e^{\theta T_r} - e^{\theta T_\cheat{r}}} &= \E*{\gp*{e^{\theta T_r} - e^{\theta T_\cheat{r}}} \1\gp*{W(-r(L)) > r(L), r(L) \leq r_{max}}}\\
        &\; \; \; \; + \E*{\gp*{e^{\theta T_r} - e^{\theta T_\cheat{r}}}\1\gp*{W(-r(L)) \leq r(L), r(L) \leq r_{max}}}\\
        &\; \; \; \; + \E*{\gp*{e^{\theta T_r} - e^{\theta T_\cheat{r}}}\1\gp*{r(L) > r_{max}}}\\
        &= \E*{\gp*{e^{\theta T_r} - e^{\theta T_\cheat{r}}} \1\gp*{W(-r(L)) > r(L), r(L) \leq r_{max}}}\\
        &\; \; \; \; + B_r + B_\cheat{r} + \E*{\gp*{e^{\theta T_r} - e^{\theta T_\cheat{r}}}\1\gp*{r(L) > r_{max}}}. \tag{By \cref{lem:cheating_bounded}.}\\
        &\leq B_r + B_\cheat{r} + \E*{\gp*{e^{\theta T_r} - e^{\theta T_\cheat{r}}}\1\gp*{r(L) > r_{max}}}. \tag{By \cref{lem:legit_leq_cheat_for_noncheating_job}.}
    \]
    Multiplying both sides by $(\gamma - \theta)$, and taking $\theta\to\gamma$ yields
    \[
        \lim_{\theta\to\gamma} (\gamma - \theta)\E*{e^{\theta T_r} - e^{\theta T_\cheat{r}}} &\leq \lim_{\theta\to\gamma} (\gamma - \theta)\gp*{B_r + B_\cheat{r}} + A\E*{\gp*{e^{\theta T_r} - e^{\theta T_\cheat{r}}} \1\gp*{r(L) > r_{max}}} \tag{By \cref{lem:r>r_max}.}\\
        % Known sizes version.
        % \lim_{\theta\to\gamma} (\gamma - \theta)\E*{e^{\theta T_r} - e^{\theta T_\cheat{r}}} &\leq \lim_{\theta\to\gamma} (\gamma - \theta)\gp*{B_r + B_\cheat{r}} + A\P*{r(L) > r_{max}} \tag{By \cref{lem:r>r_max}.}\\
        &= A\E*{\gp*{e^{\theta T_r} - e^{\theta T_\cheat{r}}} \1\gp*{r(L) > r_{max}}}.
        % Known sizes version.
        % &= A\P*{r(L) > r_{max}.
    \]
    Since our choice of $r_{max} > 0$ was arbitrary, and $\E*{\gp*{e^{\theta T_r} - e^{\theta T_\cheat{r}}} \1\gp*{r(L) > r_{max}}} \to 0$ as $r_{max} \to \infty$, that implies $\limsup_{\theta\to\gamma} (\gamma - \theta) \E*{e^{\theta T_r} - e^{\theta T_\cheat{r}}} \leq 0$, as desired.
    % Known sizes version.
    % Since our choice of $r_{max} > 0$ was arbitrary, and $\P*{r(L) > r_{max}} \to 0$ as $r_{max} \to \infty$, that implies $\limsup_{\theta\to\gamma} (\gamma - \theta) \E*{e^{\theta T_r} - e^{\theta T_\cheat{r}}} \leq 0$, as desired.
\end{proof}

\subsection{Proof of \cref{lem:gamma_theta_convergence}.}
We need some lemmas before we can prove \cref{lem:gamma_theta_convergence}. We first prove the following lemma:

\begin{lemma}\label{lem:o3_deriv_bound}
    Consider a boost policy using boost function $r$, the response time under boost policy $r$ to be $T_r$, and some positive number $b_{max}$. Suppose that the work-crossing is finite. Then there is a constant $A > 0$ s/t:
    \[
        \lim_{b_{max} \to \infty} \lim_{\theta \to \gamma} (\gamma - \theta)\E*{e^{\theta T_{\boost{\gamma}}}\1\gp*{\E*{S_L e^{\gamma S_L}} \geq b_{max}}} = 0.
    \]
\end{lemma}

\begin{proof}
    Observe that the response time of the job is upper bounded by the amount of work in the system at its arrival time, plus the job size, plus the work-crossing amount at the arrival time. That is, we can write
    \[
        T_r \leq W + S + V_{\boost{\gamma}}\gp*{-\infty, 0; 0, \infty},
    \]
    which implies
    \[
        \E*{e^{\theta T_r}\1\gp*{r > r_{max}}} &\leq \E*{e^{\theta \gp*{W + S + V_{\boost{\gamma}}\gp*{-\infty, 0; 0, \infty}}}\1\gp*{\E*{S_L e^{\gamma S_L}} \geq b_{max}}}\\
        &\leq \E*{e^{\theta W}}\E*{e^{\theta S} \1\gp*{\E*{S_L e^{\gamma S_L}} \geq b_{max}}} B \tag{By independence, and finiteness of work-crossing.}\\
    \]
    Observe that as $\theta\to\gamma$, the last line becomes
    \[
        \frac{C_\fcfs}{\E*{e^{\gamma S}}} B \E*{e^{\gamma S} \1\gp*{\E*{S_L e^{\gamma S_L}} \geq b_{max}}}.
    \]
    Now it suffices to show that
    \[
        \lim_{b_{max} \to \infty} \E*{e^{\gamma S} \1\gp*{\E*{S_L e^{\gamma S_L}} \geq b_{max}}} = 0.
    \]
    We can write
    \[
        \E*{e^{\gamma S} \1\gp*{\E*{S_L e^{\gamma S_L}} \geq b_{max}}} &= \E*{e^{\gamma S} \given \E*{S_L e^{\gamma S_L}} \geq b_{max}}\P*{\E*{S_L e^{\gamma S_L}} \geq b_{max}}\\
        &= \E*{\E*{e^{\gamma S} \given L} \given \E*{S_L e^{\gamma S_L}} \geq b_{max}}\P*{\E*{S_L e^{\gamma S_L}} \geq b_{max}} \tag{Tower rule.}\\
        &= \E*{\E*{e^{\gamma S} \given L} \1\gp*{\E*{S_L e^{\gamma S_L}} \geq b_{max}}}.
    \]
    Dominated Convergence Theorem yields \george{Maybe?}
    \[
        \lim_{b_{max} \to \infty} \E*{\E*{e^{\gamma S} \given L} \1\gp*{\E*{S_L e^{\gamma S_L}} \geq b_{max}}} &= \E*{ \lim_{b_{max} \to \infty} \E*{e^{\gamma S} \given L} \1\gp*{\E*{S_L e^{\gamma S_L}} \geq b_{max}}}\\
        &= 0.
    \]
\end{proof}

% Known sizes only version.
% \begin{lemma}\label{lem:known_size_bound_r_diff}
%     Consider arbitrary $r_{max} > 0$. For all $s$ s/t $r_\gamma(s) \leq r_{max}$, we have $r_\theta(s) - r_\gamma(s) \leq \gp*{\frac{(\gamma - \theta)\theta}{2\theta - \gamma}}\gp*{\frac{1}{\theta^2} + \frac{r_{max}}{\theta}}$. \george{The label version would need the assumption that $r_\theta (L)$ is convex in $\theta$. Haven't been able to show that $r_\theta (L)$ is convex in $\theta$.}
% \end{lemma}

% \begin{proof}
%     We first write $\theta = \gamma - \epsilon$. Now observe that
%     \[
%         \frac{\partial}{\partial \epsilon} r_{\gamma - \epsilon}(s) = \frac{s e^{-(\gamma - \epsilon)}}{(\gamma - \epsilon)\gp*{1 - e^{-(\gamma - \epsilon)s}}} + \frac{1}{(\gamma - \epsilon)^2}\log\gp*{\frac{1}{1 - e^{-(\gamma - \epsilon) s}}}.
%     \]
%     We have
%     \[
%         \frac{s e^{-(\gamma - \epsilon)}}{(\gamma - \epsilon)\gp*{1 - e^{-(\gamma - \epsilon)s}}} = \frac{s}{e^{(\gamma - \epsilon) s} - 1}.
%     \]
%     Since $(\gamma - \epsilon) s \leq e^{(\gamma - \epsilon) s} - 1$, we know that $\frac{s}{e^{(\gamma - \epsilon) s} - 1} \leq \frac{1}{\gamma - \epsilon}$. Now taking the second derivative wrt $\epsilon$,
%     \[
%         \frac{\partial}{\partial \epsilon^2} r_{\gamma - \epsilon}(s) = \frac{s^2 e^{-s(\gamma - \epsilon)}}{(\gamma - \epsilon) \gp*{1 - e^{-s (\gamma - \epsilon)}}} + \frac{s^2 e^{-2s(\gamma - \epsilon)}}{(\gamma - \epsilon)\gp*{1 - e^{-s(\gamma - \epsilon)}}^2} + \frac{2se^{-s(\gamma - \epsilon)}}{(\gamma - \epsilon)^2 \gp*{1 - e^{-(\gamma - \epsilon) s}}} + \frac{2r_{\gamma - \epsilon}(s)}{(\gamma - \epsilon)^2}.
%     \]
%     Each term here is nonnegative, so we know that $r$ is convex in $\epsilon$. By the convexity of $r$, we have
%     \[
%         \frac{r_{\gamma - \epsilon}(s) - r_\gamma(s)}{\epsilon} &\leq \frac{1}{\gamma - \epsilon}\gp*{\frac{1}{\gamma - \epsilon} + r_{\gamma - \epsilon}(s)}\\
%         &\leq \frac{1}{\gamma - \epsilon}\gp*{\frac{1}{\gamma - \epsilon} + r_{\gamma - \epsilon}(s) + r_\gamma(s) - r_\gamma(s)}\\
%         \frac{r_{\gamma - \epsilon}(s) - r_\gamma(s)}{\epsilon} - \frac{r_{\gamma - \epsilon}(s) - r_\gamma(s)}{\gamma - \epsilon} &\leq \frac{1}{(\gamma - \epsilon)^2} + \frac{r_\gamma(s)}{\gamma - \epsilon}\\
%         \frac{(\gamma - 2\epsilon)\gp*{r_{\gamma - \epsilon}(s) - r_\gamma(s)}}{\epsilon(\gamma - \epsilon)} &\leq \frac{1}{(\gamma - \epsilon)^2} + \frac{r_\gamma(s)}{\gamma - \epsilon}\\
%         r_{\gamma - \epsilon}(s) - r_\gamma(s) &\leq \gp*{\frac{\epsilon(\gamma - \epsilon)}{\gamma - 2\epsilon}}\gp*{\frac{1}{(\gamma - \epsilon)^2} + \frac{r_\gamma(s)}{\gamma - \epsilon}}\\
%         &\leq \gp*{\frac{(\gamma - \theta)\theta}{2\theta - \gamma}}\gp*{\frac{1}{\theta^2} + \frac{r_{max}}{\theta}}.
%     \]
% \end{proof}

\begin{lemma}\label{lem:o1}
    Consider some arbitrary $\epsilon > 0$. Let $R_{\theta} = r_\theta(L)$. \george{I don't see why we need to tie $\epsilon$ to the arrivals bound.}
    \[
        \lim_{b_{max} \to \infty} \limsup_{\theta\to\gamma} (\gamma - \theta) \E*{\gp*{e^{\theta T_\boost{\gamma}} - e^{\theta T_\cheat{\theta}}} \1\gp*{W(-R_{\gamma - \epsilon}) > R_{\gamma - \epsilon}, \E*{S_L e^{\gamma S_L}} \leq b_{max}}}.
    \]
\end{lemma}

\begin{proof}
    We perform a tagged job analysis. Observe that $W(-R_{\gamma - \epsilon}) > R_{\gamma - \epsilon}$ implies for any $\theta\in[\gamma - \epsilon, \gamma]$ that $W(-R_\theta) > R_\theta$. Let $B$ denote the random time that is the end of the busy period under the non-cheating policy. Now we can lower bound $T_\cheat{\theta}$ by:
    \[
        T_{\cheat{\theta}} &= W(-R_\theta) - R_\theta + V_{r_\theta}(-\infty, -R_\theta; -R_\theta, 0) + V_{r_\theta}(-\infty, -R_\theta ; 0, B) + S\\
        &= W(-R_\theta) - R_\theta + V_{r_\theta}(-\infty, -R_\theta;-R_\theta, B) + S\\
        &\geq W(-R_\theta) - R_\theta + V_{r_\gamma}(-\infty, -R_\theta; -R_\theta, B) + S.
    \]
    We can upper bound $T_\boost{\gamma}$ by:
    \[
        T_{\boost{\gamma}} &\leq W(-R_\theta) - R_\theta + V_{r_\gamma}\gp*{-\infty, -R_\gamma; -R_\theta, B} + S\\
        % T_{r_\gamma} &= W(-r_\theta(L)) - r_\theta(L) + V_{r_\gamma}\gp*{(-\infty, -r_\gamma (L)), (-r_\gamma (L), B)} + V_{r_\gamma}\gp*{(-\infty, -r_\gamma(L)), (-r_\theta(L), -r_\gamma(L)]} + S\\
        &= W(-R_\theta) - R_\theta + V_{r_\gamma}\gp*{-\infty, -R_\theta; -R_\theta, B} + V_{r_{\gamma}}\gp*{-R_\theta, -R_\gamma; -R_\theta, B} + S.
    \]
    This allows us to write:
    \[
        \MoveEqLeft\E*{\gp*{e^{\theta T_\boost{\gamma}} - e^{\theta T_\cheat{\theta}}} \1\gp*{W(-R_{\gamma - \epsilon}) > R_{\gamma - \epsilon}, \E*{S_L e^{\gamma S_L}} \leq b_{max}}}\\
        &\leq \E*{e^{\theta \gp*{W(-R_\theta) + V_{r_\gamma}\gp*{-\infty, -R_\theta; -R_\theta, B} + S}}\gp*{e^{\theta V_{r_{\gamma}}\gp*{-R_\theta, -R_\gamma; -R_\theta, B}} - 1}\1\gp*{W(-R_{\gamma - \epsilon}) > R_{\gamma - \epsilon}, \E*{S_L e^{\gamma S_L}} \leq b_{max}}}.
    \]
    For shorthand, write the condition $\{W(-R_\theta) > R_\theta, \E*{S_L e^{\gamma S_L}} \leq b_{max}\}$ as $Q$. By independence of the $V$increments, we have:
    \[
        \MoveEqLeft \E*{e^{\theta \gp*{W(-R_\theta) + V_{r_\gamma}\gp*{-\infty, -R_\theta; -R_\theta, B} + S}}\gp*{e^{\theta V_{r_{\gamma}}\gp*{-R_\theta, -R_\gamma; -R_\theta, B}} - 1}\1\gp*{Q}}\\
        &\leq \E*{e^{\theta W(-R_\theta)} \given Q}\E*{e^{\gamma X_\boost{\gamma}}}\E*{e^{\theta S} \given Q}\E*{e^{\theta\gp*{e^{\theta V_{r_{\gamma}}\gp*{-R_\theta, -R_\gamma; -R_\theta, B}} - 1}} \given Q}\P*{Q}\\
        &\leq \E*{e^{\theta \gp*{W(-R_\theta) + S}}}\E*{e^{\gamma X_\boost{\gamma}}}\E*{e^{\theta\gp*{e^{\theta V_{r_{\gamma}}\gp*{-R_\theta, -R_\gamma; -R_\theta, B}} - 1}} \given Q}\\
        &\leq \E*{e^{\theta \gp*{W(-R_\theta) + S}}}\E*{e^{\gamma X_\boost{\gamma}}}\E*{e^{\theta\gp*{e^{\theta V_{r_{\gamma}}\gp*{-R_\theta, -R_\gamma; -R_\theta, \infty}} - 1}} \given Q}\\
        &\leq \E*{e^{\theta \gp*{W(-R_\theta) + S}}}\E*{e^{\gamma X_\boost{\gamma}}}\E*{e^{\theta\gp*{e^{\theta V_{r_{\gamma}}\gp*{-R_\theta, -R_\gamma; \mathbb{R}}} - 1}} \given Q}.
    \]
    The last term can be seen as the transform for the number of arrivals for a Poisson process with arrival rate $\lambda$, arrivals distributed as $S$, and over the random time period $R_\theta - R_\gamma$, subject to the condition $Q$. It can be written as:
    \[
        \E*{e^{\lambda\gp*{\E*{e^{\theta S} - 1}}\gp*{R_\theta - R_\gamma}}} &\leq \E*{e^{\gamma\gp*{R_\theta - R_\gamma}}}\\
        &= 
    \]
\end{proof}

Next we prove the following:

\begin{lemma}\label{lem:gamma_theta_convergence_for_noncheating_job}
    Let $\cheat{\beta}$ be defined as in the statement of \cref{lem:gamma_theta_convergence}. Then:
    \[
        \lim_{\theta\to\gamma} (\gamma - \theta) \E*{\gp*{e^{\theta T_{\cheat{\gamma}}} - e^{\theta T_{\cheat{\theta}}}} \1\gp*{W(-r_\theta (L)) > r_\theta (L), r_\theta (L) \leq r_{max}}} \leq 0.
    \]
\end{lemma}

% We lower bound $T_{\cheat{\theta}}$ in this version.
\begin{proof}
    We perform a tagged job analysis. Consider a job arriving into steady state. Let $B$ denote the random time that is the end of the busy period under the non-cheating policy. Under these conditions, $T_{r_\theta}$ can be lower bounded as
    \[
        T_{r_\theta} &= W(-r_\theta (L)) - r_\theta (L) + V_{r_\theta}((-\infty, -r_\theta (L)), (-r_\theta(L), 0)) + V_{r_\theta}((-\infty, -r_\theta (L)), (0, B)) + S\\
        &= W(-r_\theta (L)) - r_\theta (L) + V_{r_\theta}((-\infty, -r_\theta (L)), (-r_\theta(L), B)) + S\\
        &\geq W(-r_\theta (L)) - r_\theta (L) + V_{r_\gamma}((-\infty, -r_\theta (L)), (-r_\theta(L), B)) + S.
    \]
    \george{We use $V_{r_\theta} \geq V_{r_\gamma}$ in the last line (we would alternatively use the same to upper bound for $T_{r_\gamma}$.} \ziv{At least for this specific instance, yep, seems legit! More generally, seems legit as long as the boosted-time set is of the form $(-\infty, t)$ for some $t$.} We can write $T_{r_\gamma}$ as \ziv{Is the sum of $V$s on the first line the same as $V_{r_\gamma}\gp*{(-\infty, -r_\gamma(L)), (-r_\theta(L), B)}$? I then feel like that more nicely segues into the second line.}\george{Yes, the sum of $V$s is $V_{r_\gamma}\gp*{(-\infty, -r_\gamma(L)), (-r_\theta(L), B)}$.}
    \[
        T_{r_\gamma} &= W(-r_\theta(L)) - r_\theta(L) + V_{r_\gamma}\gp*{(-\infty, -r_\gamma (L)), (-r_\theta (L), B)} + S\\
        % T_{r_\gamma} &= W(-r_\theta(L)) - r_\theta(L) + V_{r_\gamma}\gp*{(-\infty, -r_\gamma (L)), (-r_\gamma (L), B)} + V_{r_\gamma}\gp*{(-\infty, -r_\gamma(L)), (-r_\theta(L), -r_\gamma(L)]} + S\\
        &= W(-r_\theta(L)) - r_\theta(L) + V_{r_\gamma}\gp*{(-\infty, -r_\theta (L)), (-r_\theta (L), B)} + V_{r_{\gamma}}\gp*{[-r_\theta(L), -r_\gamma(L)), (-r_\theta(L), B)} + S.
    \]
    Substituting and factoring yields:
    \[
        \MoveEqLeft e^{\theta T_{r_\gamma}} - e^{\theta T_{r_\theta}}\\
        &\leq e^{\theta \gp*{W(-r_\theta (L)) - r_\theta (L) + V_{r_\gamma}((-\infty, -r_\theta (L)), (-r_\theta(L), B)) + S}}\gp*{e^{\theta V_{r_\gamma}\gp*{[-r_\theta (L), -r_\gamma (L)), (-r_\theta (L), B)}} - 1}\\
        &\leq e^{\theta \gp*{W(-r_\theta (L)) - r_\theta (L) + V_{r_\gamma}((-\infty, -r_\theta (L)), (-r_\theta(L), \infty)) + S}} \gp*{e^{\theta V_{r_\gamma}\gp*{[-r_\theta (L), -r_\gamma (L)), (-r_\theta (L), \infty)}} - 1}.
    \]
     For shorthand, write the condition $\{ W(-r_\theta (L)) > r_\theta (L), r_\theta (L) \leq r_{max} \}$ as $Q$. By independence of the segments of work \george{Haven't added lemma about $A\times B \cap A' \times B'= \emptyset \implies V(A,B) \perp V(A',B')$ yet. Add here or appendix?} the expectations can be split into products as follows: \ziv{I think most of the $\1(Q)$s on the RHS should be conditioning on $Q$ instead, but then most/all of those terms are something independent of $Q$ anyway, so it'll be fine.}
    \[
        \E*{\gp*{e^{\theta T_{r_\gamma}} - e^{\theta T_{r_\theta}}} \1\gp*{Q}} &\leq \E*{e^{\theta S} \given Q}\E*{e^{\theta \gp*{W(-r_\theta (L)) - r_\theta (L)}} \given Q}\\
        &\; \; \; \; \; \E*{e^{\theta V_{r_\gamma}((-\infty, -r_\theta (L)), (-r_\theta(L), \infty))}\given Q}\\
        &\; \; \; \; \; \E*{\gp*{e^{\theta V_{r_\gamma}\gp*{[-r_\theta (L), -r_\gamma (L)), (-r_\theta (L), \infty)}} - 1}\given Q}\P{Q}.
    \]
    The first two terms are upper bounded by the transform $\Tilde{T}_\fcfs$, which converges to a constant as $\theta\to\gamma$. We focus on the last two terms. The term $\E*{e^{\theta V_{r_\gamma}((-\infty, -r_\theta (L)), (-r_\theta(L), \infty))} \given Q}$ is the work-crossing, which is independent of $Q$ and upper bounded by the work-crossing term $\exp\gp*{\lambda \E*{r_\gamma(L) \gp*{\E*{e^{\theta S} \given L} - 1}}}$, which is in turn bounded by \cref{cor:finite_work_crossing_for_opt}.
    
    \george{We need to fix the bound for Poisson arrivals but updating the $r_\theta(L) - r_\gamma(L)$ bound.} Now we focus on the term $\E*{\gp*{e^{\theta V_{r_\theta}\gp*{[-r_\theta (L), -r_\gamma (L)), (-r_\theta (L), \infty)}} - 1} \given Q}$. We can get an upper bound by considering the entire lifetime of arrivals, i.e. bounding by $\E*{\gp*{e^{\theta V_{r_\theta}\gp*{[-r_\theta (L), -r_\gamma (L)], \mathbb{R}}} - 1} \given Q}$. Observe that since the process with boosted arrival times can be seen as a Poisson process, this $V$ term can be seen as the arrivals of a Poisson process in the time interval $r_\theta (L) - r_\gamma (L)$. Then this term can be upper bounded by the transform of arrivals of a Poisson process in the time interval $r_\theta (L) - r_\gamma (L)$, where $L$ is s/t $r_\theta (L) \leq r_{max}$ and whose arrivals have distribution $S$. This transform is simply $e^{\lambda \gp*{r_\theta (L) - r_\gamma (L)} \gp*{\Tilde{S}(-\theta) - 1}}$, which we can bound using \cref{lem:label_bound_rdiff} by
    \[
        e^{\lambda \frac{r_{max}(\gamma - \theta)}{\alpha} \gp*{\Tilde{S}(\theta) - 1}}
    \]
    as $\theta \to \gamma$, by picking some $\alpha$ smaller than $\gamma$. Therefore we have, as $\theta \to \gamma$:
    \[
        (\gamma - \theta)\Tilde{T}_\fcfs(-\theta) &\to C_\fcfs\\
        \E*{e^{\theta V_{r_\gamma}((-\infty, -r_\theta (L)), (-r_\theta(L), \infty))} \given Q } &\leq B\\
        e^{\lambda \gp*{r_\theta (L) - r_\gamma (L)} \gp*{\Tilde{S}(-\theta) - 1}} - 1 &\to 0,
    \]
    which imply that
    \[
        \lim_{\theta\to\gamma} (\gamma - \theta) \E*{\gp*{e^{\theta T_{r_\gamma}} - e^{\theta T_{r_\theta}}} \1\gp*{W(-r_\theta (L)) > r_\theta (L), r_\theta (L) \leq r_{max}}} \leq 0.
    \]
\end{proof}

% \begin{proof}
%     We perform a tagged job analysis. Consider a job arriving into steady state. Let $B$ denote the random time that is the end of the busy period under the non-cheating policy. Under these conditions, $T_{r_\theta}$ can be written as
%     \[
%         T_{r_\theta} &= W(-r_\theta (L)) - r_\theta (L) + V_{r_\theta}((-\infty, -r_\theta (L)), (-r_\theta(L), 0)) + V_{r_\theta}((-\infty, -r_\theta (L)), (0, B)) + S\\
%         &= W(-r_\theta (L)) - r_\theta (L) + V_{r_\theta}((-\infty, -r_\theta (L)), (-r_\theta(L), B)) + S.
%     \]
%     \george{Not sure if we need to explain why we can sum the two $V$'s above (since they cover only the interval strictly before $-r_\theta (L)$, the tagged job is not included). This happens a couple of times in other arguments.} We can upper bound $T_{r_\gamma}$ as
%     \[
%         T_{r_\gamma} &\leq W(-r_\theta (L)) - r_\theta (L) + V_{r_\theta}\gp*{(-\infty, -r_\theta (L)), (-r_\theta (L), B)} + V_{r_\theta}\gp*{[-r_\theta (L), -r_\gamma (L)), (-r_\theta (L), B)} + S
%     \]
%     % \[
%     %     T_{r_\gamma} &\leq W(-r_\theta (L)) - r_\theta (L) + V_{r_\theta}((-\infty, -r_\gamma (L)), (-r_\theta (L), -r_\gamma (L))) + V_{r_\theta}((-\infty, -r_\gamma (L)), (-r_\theta (L), 0))\\
%     %     &\; \; \; \; \; + V_{r_\theta}((-\infty, -r_\gamma (L)), (0, \infty))\\
%     %     &= W(-r_\theta (L)) - r_\theta (L) + V_{r_\theta}((-\infty, -r_\gamma (L)), (-r_\theta (L), -r_\gamma (L))) + V_{r_\theta}\gp{(-\infty, -r_\gamma(L)), (-r_\theta(L), \infty)}\\
%     %     &\leq  W(-r_\theta (L)) - r_\theta (L) + V_{r_\theta}((-\infty, -r_\theta (L)), (-r_\theta (L), -r_\gamma (L))) + V_{r_\theta}\gp{[-r_\theta (L), -r_\gamma (L)), (-r_\theta (L), -r_\gamma (L))}\\
%     %     &\; \; \; \; \; + V_{r_\theta}\gp{(-\infty, -r_\theta (L)), (-r_\theta (L), \infty)} + V_{r_\theta}\gp{[-r_\theta (L), -r_\gamma (L)), (-r_\theta (L), \infty)}.
%     % \]
%     Substituting and factoring yields:
%     \[
%         \MoveEqLeft e^{\theta T_{r_\gamma}} - e^{\theta T_{r_\theta}}\\
%         &\leq e^{\theta \gp*{W(-r_\theta (L)) - r_\theta (L) + V_{r_\theta}((-\infty, -r_\theta (L)), (-r_\theta(L), B)) + S}}\gp*{e^{\theta V_{r_\theta}\gp*{[-r_\theta (L), -r_\gamma (L)), (-r_\theta (L), B)}} - 1}\\
%         &\leq e^{\theta \gp*{W(-r_\theta (L)) - r_\theta (L) + V_{r_\theta}((-\infty, -r_\theta (L)), (-r_\theta(L), \infty)) + S}} \gp*{e^{\theta V_{r_\theta}\gp*{[-r_\theta (L), -r_\gamma (L)), (-r_\theta (L), \infty)}} - 1}.
%     \]
%     For shorthand, write the condition $\{ W(-r_\theta (L)) > r_\theta (L), r_\theta (L) \leq r_{max} \}$ as $Q$. By independence of the segments of work \george{Haven't added lemma about $A\times B \cap A' \times B'= \emptyset \implies V(A,B) \perp V(A',B')$ yet. Add here or appendix?} the expectations can be split into products as follows:
%     \[
%         \E*{\gp*{e^{\theta T_{r_\gamma}} - e^{\theta T_{r_\theta}}} \1\gp*{Q}} &\leq \E*{e^{\theta S} \1\gp*{Q}}\E*{e^{\theta \gp*{W(-r_\theta (L)) - r_\theta (L)}}\1\gp*{Q}}\\
%         &\; \; \; \; \; \E*{e^{\theta V_{r_\theta}((-\infty, -r_\theta (L)), (-r_\theta(L), \infty))}\1\gp*{Q}}\\
%         &\; \; \; \; \; \E*{\gp*{e^{\theta V_{r_\theta}\gp*{[-r_\theta (L), -r_\gamma (L)), (-r_\theta (L), \infty)}} - 1}\1\gp*{Q}}.
%     \]
%     The first two terms are upper bounded by the transform $\Tilde{S}(-\theta)$ and $\Tilde{W} \sim \Tilde{T}_{Q,\fcfs}$, respectively. We focus on the last two terms. By assumption, for some arbitrary $\theta' < \gamma$, we can bound the term $\E*{e^{\theta V_{r_\theta}((-\infty, -r_\theta (L)), (-r_\theta(L), \infty))}\1\gp*{Q}}$ by some $B > 0$ for all $\theta \geq \theta'$. In particular, this means that as $\theta\to\gamma$, the same bound $B$ applies to this term.
    
%     Now we focus on the term $\E*{\gp*{e^{\theta V_{r_\theta}\gp*{[-r_\theta (L), -r_\gamma (L)), (-r_\theta (L), \infty)}} - 1}\1\gp*{Q}}$. We can get an upper bound by considering the entire lifetime of arrivals, i.e. bounding by $\E*{\gp*{e^{\theta V_{r_\theta}\gp*{[-r_\theta (L), -r_\gamma (L)], \mathbb{R}}} - 1} \1\gp*{Q}}$. Observe that since the process with boosted arrival times can be seen as a Poisson process, this $V$ term can be seen as the arrivals of a Poisson process in the time interval $r_\theta (L) - r_\gamma (L)$. Then this term can be upper bounded by the transform of arrivals of a Poisson process in the time interval $r_\theta (L) - r_\gamma (L)$, where $L$ is s/t $r_\theta (L) \leq r_{max}$ and whose arrivals have distribution $S$. This transform is simply $e^{\lambda \gp*{r_\theta (L) - r_\gamma (L)} \gp*{\Tilde{S}(-\theta) - 1}}$, which we can bound using \cref{lem:label_bound_rdiff} by
%     \[
%         e^{\lambda \frac{r_{max}(\gamma - \theta)}{\alpha} \gp*{\Tilde{S}(\theta) - 1}}
%     \]
%     as $\theta \to \gamma$, by picking some $\alpha$ smaller than $\gamma$. Therefore we have, as $\theta \to \gamma$:
%     \[
%         (\gamma - \theta)\Tilde{W}(-\theta)\Tilde{S}(-\theta) &\to C_\fcfs\\
%         \E*{e^{\theta V_{r_\theta}((-\infty, -r_\theta (L)), (-r_\theta(L), \infty))}\1\gp*{Q}} &\leq B\\
%         e^{\lambda \gp*{r_\theta (L) - r_\gamma (L)} \gp*{\Tilde{S}(-\theta) - 1}} - 1 &\to 0,
%     \]
%     which imply that
%     \[
%         \lim_{\theta\to\gamma} (\gamma - \theta) \E*{\gp*{e^{\theta T_{r_\gamma}} - e^{\theta T_{r_\theta}}} \1\gp*{W(-r_\theta (L)) > r_\theta (L), r_\theta (L) \leq r_{max}}} \leq 0.
%     \]
% %     Now we focus on the term $\E*{\gp*{e^{\theta V_{r_\theta}\gp*{[-r_\theta (L), -r_\gamma (L)), (-r_\theta (L), \infty)}} - 1}\1\gp*{Q}}$. We can get an upper bound by considering the entire lifetime of arrivals, i.e. bounding by $\E*{\gp*{e^{\theta V_{r_\theta}\gp*{[-r_\theta (L), -r_\gamma (L)], \mathbb{R}}} - 1} \1\gp*{Q}}$. Observe that since the process with boosted arrival times can be seen as a Poisson process, this $V$ term can be seen as the arrivals of a Poisson process in the time interval $r_\theta (L) - r_\gamma (L)$. Then this term can be upper bounded by the transform of arrivals of a Poisson process in the time interval $r_\theta (L) - r_\gamma (L)$, where $L$ is s/t $r_\theta (L) \leq r_{max}$ and whose arrivals have distribution $S$. This transform is simply $e^{\lambda \gp*{r_\theta (L) - r_\gamma (L)} \gp*{\Tilde{S}(-\theta) - 1}}$, which is bounded by $e^{\lambda \gp*{\sup_L r_\theta (L) - r_\gamma (L)}\gp*{\Tilde{S}(-\theta) - 1}}$ Since $r$ is continuous in $\theta$ for $\theta\geq \theta'$, as $\theta\to\gamma$, $e^{\lambda \gp*{r_\theta (L) - r_\gamma (L)} \gp*{\Tilde{S}(-\theta) - 1}} \to 1$, and we have the following:
% %     \[
% %         (\gamma - \theta)\Tilde{W}(-\theta)\Tilde{S}(-\theta) &\to C_\fcfs\\
% %         \E*{e^{\theta V_{r_\theta}((-\infty, -r_\theta (L)), (-r_\theta(L), \infty))}\1\gp*{Q}} &\leq B\\
% %         e^{\lambda \gp*{r_\theta (L) - r_\gamma (L)} \gp*{\Tilde{S}(-\theta) - 1}} - 1 &\to 0,
% %     \]
% %     which imply that
% %     \[
% %         \lim_{\theta\to\gamma} (\gamma - \theta) \E*{\gp*{e^{\theta T_{r_\gamma}} - e^{\theta T_{r_\theta}}} \1\gp*{W(-r_\theta (L)) > r_\theta (L), r_\theta (L) \leq r_{max}}} \leq 0.
% %     \]
% % \end{proof}
% \end{proof}

\begin{proof}[Proof of \cref{lem:gamma_theta_convergence}]
    Take arbitrary $r_{max} > 0$. We can write:
    \[
        \E*{e^{\theta T_{\cheat{\gamma}}} - e^{\theta T_{\cheat{\theta}}}} &= \E*{\gp*{e^{\theta T_{\cheat{\gamma}}} - e^{\theta T_{\cheat{\theta}}}} \1\gp*{W(-r_\theta (L)) > r_\theta (L), r_\theta (L) \leq r_{max}}}\\
        &\; \; \; \; \; \; + \E*{\gp*{e^{\theta T_{\cheat{\gamma}}} - e^{\theta T_{\cheat{\theta}}}} \1\gp*{W(-r_\theta (L)) \leq r_\theta (L), r_\theta (L) \leq r_{max}}}\\
        &\; \; \; \; \; \; + \E*{\gp*{e^{\theta T_{\cheat{\gamma}}} - e^{\theta T_{\cheat{\theta}}}} \1\gp*{r_\theta (L) > r_{max}}}\\
        &\leq \E*{\gp*{e^{\theta T_{\cheat{\gamma}}} - e^{\theta T_{\cheat{\theta}}}} \1\gp*{W(-r_\theta (L)) > r_\theta (L), r_\theta (L) \leq r_{max}}}\\
        &\; \; \; \; \;  \; + B + \E*{\gp*{e^{\theta T_{\cheat{\gamma}}} - e^{\theta T_{\cheat{\theta}}}} \1\gp*{r_\theta (L) > r_{max}}} \tag{By \cref{lem:cheating_bounded}.}\\
    \]
    Therefore
    \[
        \MoveEqLeft\lim_{\theta\to\gamma} (\gamma - \theta)\E*{e^{\theta T_{\cheat{\gamma}}} - e^{\theta T_{\cheat{\theta}}}}\\
        &\leq A \E*{ \gp*{e^{\theta T_{\cheat{\gamma}}} - e^{\theta T_{\cheat{\theta}}}} \1\gp*{r_\gamma (L) > r_{max}}}\\
        % Known sizes version.
        % \P*{r_\gamma (L) > r_{max}} +\\
        &\; \; \; \lim_{\theta \to \gamma} (\gamma - \theta) \E*{\gp*{e^{\theta T_{\cheat{\gamma}}} - e^{\theta T_{\cheat{\theta}}}} \1\gp*{W(-r_\theta (L)) > r_\theta (L), r_\theta (L) \leq r_{max}}}\\
        &\; \; \; \; \; \;+ (\gamma - \theta) B \tag{By \cref{lem:r>r_max}.}\\
        &\leq A \E*{ \gp*{e^{\theta T_{\cheat{\gamma}}} - e^{\theta T_{\cheat{\theta}}}} \1\gp*{r_\gamma (L) > r_{max}}} \tag{By \cref{lem:gamma_theta_convergence}.}
        % &\leq A \P*{r_\gamma (L) > r_{max}}. \tag{By \cref{lem:gamma_theta_convergence}.}
    \]
    Since our choice of $r_{max} > 0$ was arbitrary and $r_{max} \to \infty$ implies $A \E*{ \gp*{e^{\theta T_{\cheat{\gamma}}} - e^{\theta T_{\cheat{\theta}}}} \1\gp*{r_\gamma (L) > r_{max}}} \to 0$, we have
    % Known sizes version.
    % Since our choice of $r_{max} > 0$ was arbitrary, and $r_{max} \to \infty$ implies $\P*{r_\gamma(L) > r_{max}} \to 0$, we have
    \[
        \limsup_{\theta\to\gamma} (\gamma - \theta) \E*{e^{\theta T_{\cheat{\gamma}}} - e^{\theta T_{\cheat{\theta}}}} \leq 0,
    \]
    as desired.
\end{proof}

\subsection{Proof of optimality of the optimal boost policy.}

\begin{proof}[Proof of \cref{thm:optimality_thm}.]
\Cref{lem:legit_cheating_convergence, lem:gamma_theta_convergence} allow us to prove optimality of the optimal boost policy. We want to show for any policy $\pi$, that\[
    \frac{1}{\gamma}\lim_{\theta\to\gamma} (\gamma - \theta) \E*{e^{\theta T_\pi} - e^{\theta T_\boost{\gamma}}} \geq 0.
\] It therefore suffices to show that \[
    \liminf_{\theta\to\gamma} (\gamma - \theta) \E*{e^{\theta T_\pi} - e^{\theta T_\boost{\gamma}}} \geq 0.
\] We can decompose the LHS as \[
    \liminf_{\theta\to\gamma} (\gamma - \theta) \gp*{\E*{e^{\theta T_\pi} - e^{\theta T_\cheat{\theta}}} - \E*{e^{\theta T_\boost{\gamma}} - e^{\theta T_\cheat{\theta}}}}. 
\] Now we have \[
    \MoveEqLeft
    \liminf_{\theta\to\gamma} (\gamma - \theta) \gp*{\E*{e^{\theta T_\pi} - e^{\theta T_\cheat{\theta}}} - \E*{e^{\theta T_\boost{\gamma}} - e^{\theta T_\cheat{\theta}}}}\\
    &\geq \liminf_{\theta\to\gamma} (\gamma - \theta) \E*{e^{\theta T_\pi} - e^{\theta T_\cheat{\theta}}} - \limsup_{\theta\to\gamma} (\gamma - \theta) \E*{e^{\theta T_\boost{\gamma}} - e^{\theta T_\cheat{\theta}}}.
\] For the first term, we know from \cref{sec:sample_path} that both $(\gamma - \theta)$ and $\E*{e^{\theta T_\pi} - e^{\theta T_\cheat{\theta}}} \geq 0$ for any $\theta$, so the $\liminf$ must be $\geq 0$. The second term we can further decompose as \[
    \limsup_{\theta \to \gamma} (\gamma - \theta) \gp*{\E*{e^{\theta T_\boost{\gamma}} - e^{\theta T_\cheat{\gamma}}} + \E*{e^{\theta T_\cheat{\gamma}} - e^{\theta T_\cheat{\theta}}}}.
\] Applying \cref{lem:legit_cheating_convergence, lem:gamma_theta_convergence} to both terms, we know that the $\limsup$ of both terms is $\leq 0$. Therefore \[
    \liminf_{\theta\to\gamma} (\gamma - \theta) \gp*{\E*{e^{\theta T_\pi} - e^{\theta T_\cheat{\theta}}} - \E*{e^{\theta T_\boost{\gamma}} - e^{\theta T_\cheat{\theta}}}} \geq 0,
\] as desired.
\end{proof}

% In this section, we prove that $\boost{\gamma}$, the boost policy that uses \cref{eq:optimal_boost_function}, attains a strongly optimal asymptotic tail coefficient. Formally, we have the following theorem:

% \begin{theorem}\label{thm:optimality_thm}
%     Suppose that $S$ is a Class~I job size distribution, with asymptotic tail decay rate $\gamma$, and let $C_\pi$ denote the asymptotic coefficient, as in \cref{eq:asymptotic_constant_def}. Then for any work-conserving, nonanticipative policy $\pi$, \[
%         C_\pi - C_\boost{\gamma} \geq 0.
%     \]
% \end{theorem}

% To show that this achieves the best possible constant, we compare to the $\cheat{\gamma}$ policy, which allows jobs to be served before their actual arrival time. The results from \cref{sec:sample_path} show that $\cheat{\gamma}$ minimizes the metric $\E*{e^{\theta T_{r_\gamma}}}$ for any sequence of jobs. \george{This is the lemma: "All policies $\pi$ have $\E*{e^{\theta T_\pi} - e^{\theta T_{\cheat{\theta}}}} \geq 0$, for any $\theta$." It should be detailed in \cref{sec:sample_path}.}

% We will first show that $\boost{\gamma}$'s performance approaches $\cheat{\gamma}$'s performance, as $\theta\to\gamma$. Then we will show that $\cheat{\gamma}$'s performance approaches the lower bound of the limiting sequence of optimal policies for each $\theta$; that is, as $\theta\to\gamma$, the performance of $\cheat{\gamma}$ matches that given by $\frac{1}{\gamma}\lim_{\theta \to \gamma} (\gamma - \theta) \E{e^{\theta T_\cheat{\theta}}}$. These are formally stated below:

% \begin{lemma}\label{lem:boost_to_cheat}
%     \[
%     \limsup_{\theta \to\gamma} (\gamma - \theta) \E*{e^{\theta T_\boost{\gamma}} - e^{\theta T_\cheat{\gamma}}} \leq 0.
%     \]
% \end{lemma}

% \begin{lemma}\label{lem:cheat_seq_convergence}
%     \[
%         \limsup_{\theta\to\gamma} (\gamma - \theta) \E*{e^{\theta T_\cheat{\gamma}} - e^{\theta T_\cheat{\theta}}}\leq 0.
%     \]
% \end{lemma}

% Below, we prove \cref{lem:boost_to_cheat, lem:cheat_seq_convergence}. We begin with several useful definitions.

% \begin{definition}\label{def:epl_eps}
%     A job $S$ is $\epl$ if $r_{\gamma - \epsilon}(S) \leq \frac{1}{\sqrt{\epsilon}}$. A job is $\eps$ if it is not $\epl$.
% \end{definition}

% \begin{definition}\label{def:V}
%     $V_\beta(B, A)$ is the amount of work with arrival time in $A$ that has a boosted arrival time in $B$, where jobs of size $S$ receive boost $r_\beta(S)$.
% \end{definition}

% \subsection{Proof of \cref{lem:boost_to_cheat}}

% We begin with some necessary lemmas.

% \begin{lemma}\label{lem:eps_small}
%     Consider policies $\pi\in \{\cheat{\beta}, \boost{\beta}\}$, where $\beta > 0$. Then \[
%         \E*{e^{\theta T_\pi} \1(\epl)} \leq \E*{e^{\theta T_\pi}} \leq \E*{e^{\theta T_\pi} \mid \epl},
%     \] and the difference between $\E*{e^{\theta T_\pi} \1(\epl)}$ and $\E*{e^{\theta T_\pi} \mid \epl}$ goes to $0$ as $\epsilon \to 0$.
% \end{lemma}

% \begin{proof}
%     \george{This argument needs to be formalized. Put proof in appendix if too long/irrelevant?} The first inequality is immediate since $e^{(\cdot)}$ is nonnegative. We focus on the second inequality. By the law of total expectation, \[
%         \E*{e^{\theta T_\pi}} = \E*{e^{\theta T_\pi} \mid \eps}\P*{\eps} + \E*{e^{\theta T_\pi}\1(\epl)}.
%     \] Since $\E*{e^{\theta T_\pi} \mid \eps}$ is stochastically dominated by $\E*{e^{\theta T_\pi}}$, we have the following sequence: \[
%         \E*{e^{\theta T_\pi}} &\leq \E*{e^{\theta T_\pi}}\P*{\eps} + \E*{e^{\theta T_\pi}\1(\epl)}\\
%         \E*{e^{\theta T_\pi}}\gp*{1 - \P*{\eps}} &\leq \E*{e^{\theta T_\pi}\1(\epl)}\\
%         \E*{e^{\theta T_\pi}}\P*{\epl} &\leq \E*{e^{\theta T_\pi} \mid \epl} \P*{\epl}\\
%         \E*{e^{\theta T_\pi}}\P*{\epl} &\leq \E*{e^{\theta T_\pi} \mid \epl} \P*{\epl}\\
%         \E*{e^{\theta T_\pi}} &\leq \E*{e^{\theta T_\pi} \mid \epl}.
%     \]

%     We also observe by the definition of $\epl$ that as $\epsilon\to 0$, $\P*{\epl} \to 1$, since $\frac{1}{\sqrt{\epsilon}}\to \infty$ as $\epsilon\to 0$. This implies that $\E*{e^{\theta T_\pi} \mid \epl} - \E*{e^{\theta T_\pi} \1(\epl)}\to 0$.
% \end{proof}

% \george{Adjust the below lemmas to apply to $\cheat{\beta}$ for arbitrary $\beta\in[\gamma-\delta,\gamma]$, where $0 < \delta < \gamma$. Need this lemma for part of a later argument. Should work just fine.}

% \begin{lemma}\label{lem:U_leq_r_lem}
%     There is a $C < \infty$ s/t the following statements hold:
%     \*[(1)]
%     \* \[
%         \E*{\E*{e^{\theta T_\cheat{\gamma}} \1\gp*{W(-r_{\gamma - \epsilon}(s)) \leq r_{\gamma - \epsilon}(s), \epl} \mid S = s}} \leq C
%     \]
%     \* \[
%         \E*{\E*{e^{\theta T_\boost{\gamma}} \1\gp*{W(-r_{\gamma - \epsilon}(s)) \leq r_{\gamma - \epsilon}(s), \epl} \mid S = s}} \leq C
%     \]
%     \*/
% \end{lemma}

% \begin{lemma}\label{lem:legit_leq_cheat}
%     \[
%         \E*{\E*{e^{\theta T_\boost{\gamma}} \1\gp*{W(-r_{\gamma - \epsilon}(s)) > r_{\gamma - \epsilon}(s), \epl} \mid S = s}} \leq\\
%         \E*{\E*{e^{\theta T_\cheat{\gamma}} \1\gp*{W(-r_{\gamma - \epsilon}(s)) > r_{\gamma - \epsilon}(s), \epl} \mid S = s}}
%     \]
% \end{lemma} The proofs of \cref{lem:U_leq_r_lem, lem:legit_leq_cheat} are given in the Appendix. \george{Add proofs to appendix.}

% \begin{proof}[Proof of \cref{lem:boost_to_cheat}]
%     We consider arbitrary $\epsilon > 0$, and a tagged job coming into a steady-state system. Denote as shorthand $D_\theta = e^{\theta T_\boost{\gamma}} - e^{\theta T_\cheat{\gamma}}$. We have the following: \[
%         \MoveEqLeft
%         \E*{D_\theta}\\
%         &= \E*{D_\theta\1(\epl)} + \E*{D_\theta \1(\eps)}\\
%         \tag{Where $g(\epsilon) \to 0$ as $\epsilon\to 0$, by \cref{lem:eps_small}.}
%         &\leq \E*{D_\theta \1(\epl)} + g(\epsilon)\\
%         &= \E*{\E*{D_\theta \1(\epl, W(-r_{\gamma - \epsilon}(s)) > r_{\gamma - \epsilon}(s)) \mid S = s}} +\\
%         &\; \; \; \; \; \; \; \; \E*{\E*{D_\theta \1(\epl, W(-r_{\gamma - \epsilon}(s)) \leq r_{\gamma - \epsilon}(s)) \mid S = s}} + g(\epsilon)\\
%         \tag{By \cref{lem:U_leq_r_lem}.}
%         &\leq \E*{\E*{D_\theta \1(\epl, W(-r_{\gamma - \epsilon}(s)) > r_{\gamma - \epsilon}(s)) \mid S = s}} + C + g(\epsilon).
%     \] Using this, we can write \[
%         \MoveEqLeft
%         \frac{1}{\gamma}\limsup_{\theta\to\gamma} (\gamma - \theta) \E*{e^{\theta T_\boost{\gamma}} - e^{\theta T_\cheat{\gamma}}} \leq\\ 
%         &\frac{1}{\gamma}\limsup_{\theta\to\gamma} (\gamma - \theta) \gp*{C + g(\epsilon) + \E*{\E*{D_\theta \1(\epl, W(-r_{\gamma - \epsilon}(s)) > r_{\gamma - \epsilon}(s)) \mid S = s}}}.
%     \] Focus on the $\limsup$ of the RHS. As $\theta\to\gamma$, the $\limsup$ is $\leq 0$ for all three terms. The first two are constant wrt $\theta$ and the last term is $\leq 0$ due to \cref{lem:legit_leq_cheat}.

%     % Alternate proof (maybe shorter?) involves showing for legit and cheating separately that under {W <= r}, the expectation E{e^{\theta T}} is finite for both. Then showing that under {W > r}, E{e^{\theta T_L}} = E{e^{\theta T_C}} by way of a work-crossing argument.
% \end{proof}

% \subsection{Proof of \cref{lem:cheat_seq_convergence}.}
% To prove \cref{lem:cheat_seq_convergence} we need the following:

% \begin{lemma}\label{lem:epl_cheat_convergence}
%     For arbitrary $\epsilon > 0$ and any $\theta\in[\gamma - \epsilon, \gamma]$, there is a $f(\epsilon)$ where $f(\epsilon)\to 0$ as $\epsilon \to 0$ and a $C > 0$ (both independent of $\theta$) s/t \[
%         (\gamma - \theta) \E*{\E*{\gp*{e^{\theta T_{\cheat{\gamma}}} - e^{\theta T_{\cheat{\theta}}}} \1(W(-r_\theta(s)) > r_\theta(s), \epl) \mid S = s}} \leq C f(\epsilon).
%     \]
% \end{lemma} The proof of \cref{lem:epl_cheat_convergence} is given in the Appendix. \george{Add proof to the appendix.}

% \begin{proof}[Proof of \cref{lem:cheat_seq_convergence}.]
%     We consider arbitrary $\epsilon > 0$, and a tagged job coming into a steady-state system. In this proof, denote as shorthand $D_\theta = e^{\theta T_\cheat{\gamma}} - e^{\theta T_\cheat{\theta}}$. We have the following: \[
%         \E*{D_\theta} &= \E*{D_\theta \1(\epl)} + \E*{D_\theta \1(\eps)}\\
%         \tag{Where $g(\epsilon)\to 0$ as $\epsilon \to 0$, by \cref{lem:eps_small}.}
%         &\leq \E*{D_\theta \1(\epl)} + g(\epsilon)\\
%         &= \E*{\E*{D_\theta \1(W(-r_{\gamma - \epsilon}(s)) > r_{\gamma - \epsilon}(s), \epl) \mid S = s}} +\\
%         &\; \; \; \; \; \; \; \; \E*{\E*{D_\theta \1(W(-r_{\gamma - \epsilon}(s)) \leq r_{\gamma - \epsilon}(s), \epl) \mid S = s}} + g(\epsilon)\\
%         \tag{By \cref{lem:U_leq_r_lem}.}
%         &\leq \E*{\E*{D_\theta \1(W(-r_{\gamma - \epsilon}(s)) > r_{\gamma - \epsilon}(s), \epl) \mid S = s}} + C + g(\epsilon),
%     \] where $C > 0$. This yields \[
%         \limsup_{\theta \to \gamma} (\gamma - \theta) \E*{D_\theta} \leq \limsup_{\gamma\to\theta} (\gamma - \theta) \E*{\E*{D_\theta \1(W(-r_{\gamma - \epsilon}(s)) > r_{\gamma - \epsilon}(s), \epl) \mid S = s}} + C + g(\epsilon).
%     \] Observe that the last two terms are constant wrt $\theta$, so the $\limsup$ is $\leq 0$. For the first term, by \cref{lem:epl_cheat_convergence} there exists a $C' > 0$ and $f(\epsilon)$ s/t \[
%         (\gamma - \theta)\E*{\E*{D_\theta \1(W(-r_{\gamma - \epsilon}(s)) > r_{\gamma - \epsilon}(s), \epl) \mid S = s}} \leq C' f(\epsilon),
%     \] for all $\theta \in [\gamma - \epsilon, \gamma]$. But our choice of $\epsilon > 0$ was arbitrary, and $f(\epsilon) \to 0$ as $\epsilon\to 0$, so that $\limsup$ of $(\gamma - \theta)\E*{\E*{D_\theta \1(W(-r_{\gamma - \epsilon}(s)) > r_{\gamma - \epsilon}(s), \epl) \mid S = s}}$  must be $\leq 0$.
% \end{proof}


==> old/outlines/abstract_outline.tex <==
\* The problem
\** Overall motivation and setting
\*** Scheduling to optimize response time tail matters for meeting SLOs in practice
\*** We study this problem in a queueing setting with light-tailed job sizes (a.k.a. service times)
\*** To make the question theoretically tractable, we study the asymptotics of the response time tail
\** Background
\*** Not that many policies known with good tail asymptotics
\*** FCFS is optimal up to a constant factor
\*** Only recently were policies demonstrated that improve FCFS's constant
\** The actual questions
\*** Theoretical: how to get the best asymptotic tail constant?
\*** Semi-practical: how much better is the best constant than FCFS's?
\*** Practical: does the policy that does so also have good ``pre-asymptotic'' performance, e.g. T99?

\* The solution / our contributions
\** Our results
\*** We characterize the optimal tail constant
\*** We design the first policy that achieves that tail constant
\*** Improvement can be as much as 30\%
\** The policy
\*** Family of policies called \emph{boost policies}
\*** Idea: like FCFS, but pretending that small jobs arrived earlier than they actually did

\* The impact, or some other cool thing
\** We show via simulation that boost policy has state-of-the-art ``pre-asymptotic'' performance
\** The policy is simple enough to potentially be implemented in systems such as network switches
\** Our results apply to models with known or partially known job sizes
\*** Partially known size optimality assumes nonpreemptive scheduling

\*/


==> old/outlines/conclusion_outline.tex <==
\* Summarize what we did
\* Discuss potential practical impact
\** PIFO \citep{sivaraman_programmable_2016, alcoz_sppifo_2020}
\* Future theoretical directions
\** Somehow handle things like bounded Pareto?
\*** ``At first'' heavy-tailed, ``eventually'' light-tailed
\** Study asymptotic slowdown tail?
\*** Dramatically shifts focus on what jobs matter in both heavy-tailed and light-tailed settings
\** Tradeoff between $\E{T_\pi}$ and $C_\pi$?
\** Tail scheduling with multiple servers
\*** M/G/$k$
\*** Dispatching with scheduling at each server
\*** Dispatching with FCFS at each server \citep{xie_heavytraffic_2023, hyytia_optimal_2024}
\** Non-Poisson arrivals
\*** What to use for $\gamma$?
\*/


==> old/outlines/intro_outline.tex <==
\subsubsection*{Outline}
\* \emph{High-level motivation}
\** Trying to minimize $\P{T > t}$ for a range of thresholds~$t$
\*** Especially care about large~$t$: want to avoid very long delays
\*** Some stuff about importance of tails in scheduling in practical systems, e.g. networks
\** Turn this goal into a well-posed problem: schedule to optimize the behavior in $t \to \infty$ limit
\*** Want it to be good for practical~$t$, too
\*** Want it to be implementable in practice, e.g. on network hardware
\** In this paper, we solve one such theoretical problem
\*** And it is good for practical~$t$, too
\*** And it is simple enough to be practical
\* \emph{General problem background}
\** Problem we consider: tail optimality in M/G/1
\*** (Maybe forward ref to model section)
\** Two worlds: heavy-tailed and light-tailed
\*** Heavy-tailed: SRPT is good for both mean and tail
\*** Light-tailed: SRPT is good for mean but \emph{pessimal} for tail
\** Our focus: light-tailed world
\*** Practical example: ``millisecond scale'' jobs/flows
\*** Maybe see Nudge paper for more
\** What tail of response time looks like in light-tailed world: $C_\pi = \lim_{t \to \infty} e^{\gamma t} \P{T > t}$
\*** See model section for assumptions under which $C_\pi$ exists
\*** E.g. $C_\srpt = \infty$, but $C_\fcfs$ is finite
\* \emph{Our specific goal}
\** Minimize $C_\pi$ in light-tailed world
\*** Called strong asymptotic tail optimality
\*** Open problem!
\** What's known about it
\*** Initial conjecture that FCFS was strongly optimal
\*** Counterexample: $C_\nudge < C_\fcfs$
\* \emph{Our new idea}
\** Explain boost policies
\** Explain why it's the right idea
\* \emph{Contributions} \ziv{also an outline of the paper}
\** Can maybe actually state main theorems here
\** (\cref{sec:model}) Propose boost policies
\** (\dots) Prove things
\** (\cref{sec:simulation}) Simulate things
\** (\cref{sec:heavy-tailed_strong_optimality}) Bonus: strong tail optimality in heavy-tailed case
\*/

Scratch:
\* Making the Nudge idea more flexible:
\** Accounting for both arrival times and job size information.
\** Allowing jobs to move in front of a variable number of jobs
\* Positioning the paper
\** Not just Nudge~2.0
\** Solves the strong optimality problem
\*** What the best possible is
\*** How to achieve it
\** Practicality
\*** Simple enough to be implemented
\*** Network switches? Ask Nate Foster or Anshuman Mohan
\**** Boost policies are PIFO
\**** Sample paper: \url{https://www.cs.cornell.edu/~kozen/Papers/PIFO.pdf}
\*/


==> old/outlines/main_results_outline.tex <==
Key ideas (policy):
\* Optimizing tail aysmptotics is basically equivalent to optimizing transform
\* Interchange argument for optimizing transform
\** Look at two jobs with their arrival times and sizes
\** Ask which order is best
\** Boost policy falls out
\* Formalized via sample-path analysis in \cref{sec:sample_path}
\*/

Key ideas (proofs):
\* Optimality proof ideas
\** The idea of cheating policies and cheating jobs
\** The batch policy and assumption of cheating jobs gives (kinda) a lower bound
\** Asymptotically, the legit policy matches the cheating policy
\** To get the actual lower bound, look at sequence of metrics, i.e. $\theta\to\gamma$
\* Transform key ideas
\** Work crossing quantity
\** Comparison to FCFS in terms of work crossing
\*/

Outline of the proofs:
\* Start with MGF analysis
\** Applies to any boost policy
\* Then sample-path analysis
\** Introduces optimal boost policy, cheating policies
\* Then optimality proof
\** Combines ideas from MGF analysis with specifics about the optimal boost policy
\*/

==> old/outlines/model_outline.tex <==
System model:
\* M/G/1 with known job sizes, light-tailed distribution
\** Define Class~I light-tailed distributions
\* Performance metric: asymptotic tail constant
\** Define response time
\** Define $\gamma$ as root of MGF equation
\** Express $C_\pi$ as a $\theta \to \gamma$ limit of the response time MGF
\*/

Boost policies:
\* What is a boost policy?
\** Define it
\** Define boost function~$r(s)$
\* What should the boost function look like?
\** Monotonic, specifically nonincreasing
\** Safety condition: $s r(s) \, \1(s \leq 1)$ uniformly bounded
\*** Ensures $\E{S r(S)}$ is finite for all job size distributions~$S$
\*** (The $\leq 1$ could be $\leq c$ for any constant~$c$)
\* $\beta$-optimal boost function: \[r_\beta(s) = \frac{1}{\beta} \log \frac{1}{1 - \exp(-\beta s)}\]
\** Most important case is when $\beta = \gamma$
\* Preemption or not?
\** What preemptive boost policy means
\** What nonpreemptive boost policy means
\** State that it doesn't matter
\*** Briefly explain why
\* Which of our results cover which types of boost policies
\** \Cref{sec:tail_asymptotics} is for generic boost functions
\** \Cref{sec:sample_path, sec:optimality} are for the $\gamma$-optimal boost function
\** All are for either preemptive or nonpreemptive versions
\*/

==> old/outlines/prior_work_outline.tex <==
\* Asymptotic tails in queues
\** Adam and Bert's paper
\*** And other background, e.g. Onno's survey
\** Open question: strong optimality in the light-tailed regime
\* Nudge
\** What Nudge is
\*** Isaac's paper
\*** Benny's paper
\** What's missing: accounting for arrival times
\** Something Nudge does that we don't do: looking theoretically at pre-limit thresholds
\*** We just look at this in simulation
\*/

==> old/outlines/scratch_outline.tex <==
\subsection{Notation}

\* Model
\** $\lambda$: arrival rate
\** $S$: job size distribution
\** $W$: stationary work distribution of M/G/1 with arrival rate~$\lambda$ and size distribution~$S$
\** $\gamma$: least real pole of $\E{e^{\theta W}}$
\** Assumptions
\*** $\gamma$ is a ``simple'' pole/singularity
\*** Sufficient to assume that $S$ is a class~I distribution
\* Batch problem
\** For each job~$i$:
\*** $a_i$: arrival time
\*** $S_i \sim (S \given l_i)$: service time
\*** $D_i$: departure time
\*** $T_{\pi, i} = D_{\pi, i} - a_i$
\*** $l_i$: label
\*** $b_i = b(l_i)$: boost
\** $\calI$: instance
\** $K_\theta^\pi(\calI) = \sum_{i = 1}^n \E{e^{\theta T^\pi_i}}$: $\theta$-cost under policy~$\pi$ of instance~$\calI$
\* $b$: boost function
\** $b(l)$: boost of a job with label~$l$
\** $b_\theta$: $\theta$-optimal boost function
% \* $\bExtra$: extra boost function
% \** $\bExtra(l, u)$: extra boost (in addition to $b(l)$) of a job with label~$l$ and attained service~$u$
% \** Requirements:
% \*** $\bExtra(l, 0) = 0$
% \*** $\bExtra(l, u) \geq 0$
% \** Allowed to have $\bExtra(l, u) = \infty$, i.e. we can prevent preemption
\* MGF exponent parameters
\** $\theta$: generic parameter for the MGF
\** $\gamma$: pole of MGF of $W$
\* Tagged job analysis
\** $S$: job's size
\** $L$: job's label
\** $B = b(L)$: job's boost
\*** $B_\theta = b_\theta(L)$: job's boost with $\theta$-optimal boost policy
\** Convention: tagged job's \emph{boosted} arrival time is~$0$
\** $W$: work in (legit) system at time~$0$
\** $V(u)$: work with arrival time in $[0, u]$ and boosted arrival time $\leq u$ with generic boost function~$b$
\*** $V_\theta(t)$: same, but with boost function~$b_\theta$
\** $T^\pi$: response time of the tagged job under policy~$\pi$
\*** $\pi = \fcfs$: first-come, first-served
\*** $\pi = \boost{}$: generic boost function~$b$, generic boost function~$\bExtra$
\*** $\pi = \cheat{}$: generic boost function~$b$ with cheating
\*** $\pi = \boost{\theta}$: boost function~$b_\theta$, generic extra boost function~$\bExtra$
\*** $\pi = \cheat{\theta}$: boost function~$b_\theta$ with cheating
\*/


\subsection{Definitions}

\* Batch problem
\** $\theta$-cost $K_\theta$
\** Instance / batch of jobs
\** Batch policy
\* M/G/1 model
\* Boost policies for the M/G/1
\* Work crossing amount
\*/


\section{Very scratch}


% \begin{proof}
    % It suffices to show that if under the current policy $\pi$, jobs do not depart in order of ascending $a_i - r_\theta(l_i)$, we can improve the $\theta$-cost of the policy $\pi$. Suppose that the $i$th and $i+1$th departure have $a_i - r_\theta(l_i) > a_{i+1} - r_\theta(l_{i+1})$, and that $i+1$ starts service immediately after $i$ departs (if it did not, we could immediately improve the $\theta$-cost by allowing it to start service immediately after $i$ departs, since $\pi$ can be a cheating policy).

    % If we swap the departures of these two jobs, the response time of the other jobs remains unaffected (recall that under cheating policies like \cheat{\theta} we can serve jobs before their arrivals, so this is always valid). Denote the service start time of the $i$th departure to be $I$. The response times of the original departures can be written as $\exp\gp{\theta \gp{I + S_i - a_i}}$ and $\exp\gp{\theta \gp*{I + S_i + S_{i+1} - a_{i+1}}}$. The response times of the new departures are $\exp\gp{\theta \gp*{I + S_{i+1} - a_{i+1}}}$ and $\exp\gp{\theta \gp*{I + S_i + S_{i+1} - a_i}}$, so it suffices to show that the expected sum of the response times of the new departures is no larger than the sum of the response times of the original departures if $a_i - r_\theta(l_i) \leq a_{i+1} - r_\theta(l_{i+1})$. Let $\mathbf{l} = \{l_1,\ldots,l_n\}$. We have
    % \[
    %     a_i - r_\theta(l_i) &\geq a_{i+1} - r_\theta(l_{i+1})\\
    %     a_i - \frac{1}{\theta}\log\gp*{\frac{1}{1 - \frac{1}{\E*{e^{\theta S_i} \given l_i}}}} &\geq a_{i+1} - \frac{1}{\theta}\log\gp*{\frac{1}{1 - \frac{1}{\E*{e^{\theta S_{i+1}} \given l_{i+1}}}}}\\
    %     \theta a_i + \log\gp*{1 - \frac{1}{\E*{e^{\theta S_i} \given l_i}}} &\geq \theta a_{i+1} + \log\gp*{1 - \frac{1}{\E*{e^{\theta S_{i+1}} \given l_{i+1}}}}\\
    %     e^{\theta a_i}\gp*{1 - \frac{1}{\E*{e^{\theta S_i} \given l_i}}} &\geq e^{\theta a_{i+1}}\gp*{1 - \frac{1}{\E*{e^{\theta S_{i+1}} \given l_{i+1}}}}\\
    %     \frac{\E*{e^{\theta S_i} \given l_i} - 1}{e^{-\theta a_i}\E*{e^{\theta S_i} \given l_i}} &\geq \frac{\E*{e^{\theta S_{i+1}} \given l_{i+1}} - 1}{e^{-\theta a_{i+1}}\E*{e^{\theta S_{i+1}} \given l_{i+1}}}\\
    %     \frac{e^{-\theta a_i}\E*{e^{\theta S_i} \given l_i}}{1 - \E*{e^{\theta S_i} \given l_i}} &\geq \frac{e^{-\theta a_{i+1}}\E*{e^{\theta S_{i+1}} \given l_{i+1}}}{1 - \E*{e^{\theta S_{i+1}} \given l_{i+1}}}
    % \]
    % \[
    %     e^{-\theta a_i}\E*{e^{\theta S_i} \given l_i}\gp*{1 - \E*{e^{\theta S_{i+1}} \given l_{i+1}}} &\geq e^{-\theta a_{i+1}}\E*{e^{\theta S_{i+1}} \given l_{i+1}}\gp*{1 - \E*{e^{\theta S_i} \given l_i}}\\
    %     e^{-\theta a_i}\E*{e^{\theta S_i} \given l_i} + e^{-\theta a_{i+1}}\E*{e^{\theta S_{i+1}} \given l_{i+1}}\E*{e^{\theta S_i} \given l_i} &\geq e^{-\theta a_{i+1}}\E*{e^{\theta S_{i+1}} \given l_{i+1}}\\
    %     &\; \; \; \; \; + e^{-\theta a_i}\E*{e^{\theta S_i} \given l_i}\E*{e^{\theta S_{i+1}} \given l_{i+1}}\\
    %     e^{-\theta a_i}\E*{e^{\theta S_i} \given \mathbf{l}} + e^{-\theta a_{i+1}}\E*{e^{\theta S_i} \given \mathbf{l}}\E*{e^{\theta S_{i+1}} \given \mathbf{l}} &\geq e^{-\theta a_{i+1}}\E*{e^{\theta S_{i+1}} \given \mathbf{l} }\\
    %     &\; \; \; \; \; + e^{-\theta a_i}\E*{e^{\theta S_{i+1}} \given \mathbf{l}}\E*{e^{\theta S_i} \given \mathbf{l}}\\
    %     e^{-\theta a_i}\E*{e^{\theta I} \given \mathbf{l}}\E*{e^{\theta S_i} \given \mathbf{l}}&\\
    %     + e^{-\theta a_{i+1}} \E*{e^{\theta I} \given \mathbf{l}}\E*{e^{\theta S_i} \given \mathbf{l}}\E*{e^{\theta S_{i+1}} \given \mathbf{l}} &\geq e^{-\theta a_{i+1}}\E*{e^{\theta I} \given \mathbf{l}}\E*{e^{\theta S_{i+1}} \given \mathbf{l}}\\
    %     &\; \; \; \; \; + e^{-\theta a_i}\E*{e^{\theta I} \given \mathbf{l}}\E*{e^{\theta S_i} \given \mathbf{l}}\E*{e^{\theta S_i}\given \mathbf{l}}\\
    %     \E*{e^{\theta\gp*{-a_i + I + S_i}} + e^{\theta \gp*{-a_{i+1} + I + S_i + S_{i+1}}} \given \mathbf{l}} &\geq \E*{e^{\theta \gp*{-a_{i+1} + I + S_{i+1}}} + e^{\theta \gp*{-a_i + I + S_i + S_{i+1}}}\given\mathbf{l}},
    % \]
    % where the last line is by the independence of the individual jobs. This shows that swapping the $i$th and $i+1$th departure decreases $\theta$-cost. We can continue to swap any pair of jobs that have out-of-order $a - b_\theta(l)$ and decrease it. In particular, the policy that serves jobs in order of increasing $a - b_\theta(l)$ (i.e. exactly the $\cheat{\theta}$ policy) must have $\theta$-cost no worse than any other policy that has the same information as given for this batch.
% \end{proof}

% \begin{corollary}
%     When job sizes are known, the \cheat{\theta} policy minimizes $\theta$-cost in the preemptive batch scheduling problem.
% \end{corollary}

% \begin{proof}
%     Under known job sizes, \cheat{\theta} serves jobs in $\calI$ in the same order as the Weighted Discounted Shortest Processing Time first (WDSPT) rule, with weights equal to $\exp\gp{-\theta a_i}$ and negative discount factor $\theta$ for each job $i$. The proof is an interchange argument identical to \citep[Theorem 3.1.6]{pinedo_scheduling_2016}, with the signs for the discount factor and objective flipped.
% \end{proof}

% \begin{proof}
%     Consider the $i$th job to complete. Suppose that this job experienced a preemption. Since job sizes are known, we know at any time what job is receiving service. In particular we know when the last segment of job $i$ completes and departs. We can shift the order of work so that job $i$ is not preempted, remains the $i$th job to depart, and without increasing the response time of any job. In particular, any work between the last segment of job $i$ and an earlier segment can be shifted in front of that earlier segment. Applying this to all jobs, we have transformed our policy $\pi$ into a (possibly cheating) nonpreemptive policy that has $\theta$-cost at least as good as $\pi$. We then apply \cref{thm:optimal_batch_policy} to minimize $\theta$-cost.
% \end{proof}

% \subsection{Work crossing}

% A critical piece of bounding $T_\cheat{}$ and $T_\boost{}$ is quantifying how much work with arrival time behind a job will be served, due to having lower boosted arrival time. We analyze this quantity, which we call the \emph{work-crossing}, and define it formally below. 

% \begin{definition}\label{def:work_crossing}
%     Consider an arbitrary time, and denote it as time $0$. The \emph{work-crossing} up to time $u$, written as $V(u)$, is the amount of work with arrival time in the interval $(0, u)$ and boosted arrival time before time $0$. 
% \end{definition}

% For example, $V(\infty)$ is simply all the work that arrives after time $0$ with boosted arrival time before time $0$. Observe that the work-crossing is defined relative to a start time - we make this explicit where necessary.

% \begin{lemma}\label{lem:optimal_work_crossing_finite}
%     For any $u$,
%     \[
%         \exp\gp*{\lambda \E*{b_\gamma(L) \gp*{\E*{e^{\gamma S} \given L} - 1}\1\gp{b_\gamma(L) \leq u}}} < \infty.
%     \]
% \end{lemma}

% \begin{proof}
%     First, we can drop the indicator $\1\gp{b_\gamma(L) \leq u}$ to get an upper bound. Recall that $\frac{\lambda}{\gamma} = \frac{1}{\E*{\exp\gp{\gamma S} - 1}} = \frac{1}{\E*{\E*{\exp\gp{\gamma S} \given L}} - 1}$, and let $w(L) = \E*{\exp\gp{\gamma S} \given L}$ and $g(L) = w(L) - 1$. Substituting for $\lambda$, we get
%     \[
%         \exp\gp*{\E*{\frac{\gamma}{\E*{\E*{\exp\gp{\gamma S} \given L} - 1}} b_\boost{\gamma}(L) \gp*{\E*{\exp\gp{\gamma S} \given L} - 1}}}.
%     \]
%     Let $f_{L'}(l) = f(l)g(l)$ be the $L'$-weighted pdf, and observe that we can write the above as taking the expectation wrt $L'$, i.e.
%     \[
%         \exp\gp*{\E_{L'}*{\gamma b_\gamma(L)}}.
%     \]
%     Applying Jensen's inequality, we have
%     \[
%         \exp\gp*{\E_{L'}*{\gamma b_\gamma(L)}} &\leq \E_{L'}*{\exp\gp*{\log\gp*{\frac{1}{1 - \frac{1}{\E*{\exp\gp{\gamma S} | L}}}} }}\\
%         &= \E_{L'}*{\gp*{\frac{1}{1 - \frac{1}{\E*{\exp\gp{\gamma S} | L}}}}}\\
%         &= \E*{\frac{\E*{\exp\gp{\gamma S} \given L} - 1}{\E*{\E*{\exp\gp{\gamma S} \given L} - 1}} \gp*{\frac{1}{1 - \frac{1}{\E*{\exp\gp{\gamma S} | L}}}}}\\
%         &= \frac{\E*{\exp\gp{\gamma S}}}{\E*{\exp\gp{\gamma S}} - 1}\\
%         &= \frac{\lambda}{\gamma}\E*{\exp\gp{\gamma S}}.
%     \]
%     We know that $\E*{\exp\gp{\gamma S}}$ is finite, so we are done.
% \end{proof}

% \begin{lemma}\label{lem:work_crossing_expression}
%     For boost functions s/t the expression in \cref{lem:optimal_work_crossing_finite} is finite, we have:
%     \[
%         \E*{\exp\gp{\theta V(u)}} = \exp\gp*{\lambda \E*{B\gp*{\E*{\exp\gp{\theta S} \given L} - 1}}}
%     \]
% \end{lemma}

% \begin{proof}
%     \ziv{The formula we were looking for is related to Campbell's formula \citep[Proposition~2.7]{last_lectures_2017}}

%     We can compute the work-crossing by looking at arrivals with label $L$, and splitting across all labels. For a given label $L = l$, the amount of work that crosses time $t$ given boost function $b$ is given by the number of arrivals of a Poisson process with rate $\lambda f(l) dl$ and over time period $b(l)$. The arrivals have distribution $S \given l$, and we include all $l$ s/t $b(l) \leq u$.

%     We can therefore compute the work-crossing transform by integrating over all $l$ for the merged Poisson process. \george{Here we are assuming that $L$ is a continuous rv and $b(L)$ is continuous in $L$ (but nothing about the monotonicity of $b(L)$). Not sure how to formalize if we want to use a Lebesgue integral here instead, but I think we want some lower bounded estimate that converges).} In what follows below, let $\Delta l = u / n$, $X_{i,k} \sim S \given i\Delta l, N_i \sim \text{Pois}(\lambda f(l_i) b(l_i))$, where $l_i = \arg\inf_{l_i\in [i\Delta l, (i+1)\Delta l]} f(l_i)b(l_i)$. We have:
%     \[
%         \exp\gp*{\lambda \E*{b(L) \gp*{\E*{e^{\theta S} \given L} - 1}\1\gp{b(L) \leq u}}} &= \exp\gp*{\int \lambda f(l) b(l) \gp*{\E*{e^{\theta S} \given l} - 1}\1\gp{b(l) \leq u}dl}\\
%         &= \lim_{n\to\infty} \exp\gp*{\sum_{i=1}^n \lambda f(i\Delta l) b(i\Delta l) \gp*{\E*{e^{\theta S} | i\Delta l} - 1}}\\
%         &= \lim_{n\to\infty} \prod_{i=1}^n \exp\gp*{\lambda f(i\Delta l) b(i\Delta l) \gp*{\E*{e^{\theta S} | i\Delta l} - 1}} \tag{Definition of the transform of a Poisson process.}\\
%         &= \lim_{n\to\infty} \prod_{i=1}^n \E*{\exp\gp*{\theta \sum_{k=1}^{N_i} X_{i,k}}} \tag{By independence of the Poisson processes.}\\
%         &= \lim_{n\to\infty} \E*{\exp\gp*{\theta \sum_{i=1}^n \sum_{k=1}^{N_i} X_{i,k}}}\\
%         &= \E*{ \lim_{n\to\infty} \exp\gp*{\theta \sum_{i=1}^n \sum_{k=1}^{N_i} X_{i,k}}} \tag{\george{DCT?}}\\
%         &= \E*{\exp\gp*{\theta V(u)}} 
%     \]
% \end{proof}


% \subsection{Analysis}

% Moved to section 3.
% \begin{lemma}\label{lem:boost_response_time_bounds}
%     Let $W$ be the amount of work in the system at the boosted arrival time of a tagged job that has true arrival time before the tagged job's boosted arrival time. Then:
%     \[
%         T_\boost{}, T_\cheat{} \in [W - B + V(W) + S, (W - B)^+ + V(\infty) + S]
%     \]
% \end{lemma}

% \begin{proof}
%     We perform a tagged job analysis, and begin with the lower bound. As convention, we will let the boosted arrival time of the tagged job be time $0$ (so that the job's arrival time is at time $B$). Consider a job arriving to the steady-state system. For $T_\boost{}$, it arrives at time $B$, and sees work at least $(W - B)^+ \geq W - B$. Next we will show that $T_\boost{}$ cannot start service at time earlier than time $W$ after its boosted arrival time. If $W \geq B$, then $T_\boost{}$ can enter service no sooner than after all of $W$ completes, which would be at time $W$ or later. If $W < B$, observe that $T_\boost{}$ does not arrive until time $B$, so it cannot start service until after $W$. Therefore, $V(W)$ will arrive before $T_\boost{}$ enters service, and so will depart ahead of $T_\boost{}$. So $T_\boost{}$ must be at least $W - B + V(W) + S$, as desired.

%     Now consider $T_\cheat{}$. It arrives at time $0$, which is earlier than its original arrival time by no more than $B$, and sees at least work $W + V(W)$. We know that $V(W)$ is guaranteed to arrive because there is at least work until time $W$ after the boosted arrival time of the tagged job that goes in front of it. The job must wait at least for $W + V(W)$ to finish before it can enter service, so $W + V(W) - B + S$ will be a lower bound.

%     Next we show the upper bound. For $T_\boost{}$, if $W \geq B$, then service is provided only to work in $W$ or $V(B)$ until the arrival of the tagged job at time $B$. The amount of work in front of the job at this point is $W + V(B) - B$. There may be work in the future that will go in front of the job - we can upper bound this work by allowing all jobs that could possibly preceed it to do so, i.e. we replace $V(B)$ with an upper bounding $V(\infty)$. By the time of the tagged job's arrival, then, the work it has to wait for is upper bounded by $W + V(\infty) - B$, so $W + V(\infty) - B + S$ is an upper bound. if $W < B$, the job can still receive service no earlier than time $B$, the time of its arrival. To get an upper bound, we can assume any jobs that arrive between $0$ and $B$ receive no service until time $B$. Then our tagged job must wait for jobs that arrived after time $0$ but have boosted arrival earlier than $0$, along with work in the future that will go in front of the job. This amount of work can be upper bounded by $V(\infty)$. So in this case $(W - B)^+ + V(\infty) + S$ is still an upper bound.

%     For $T_\cheat{}$, if $W \geq B$, then the tagged job cannot start service until after time $B$. All the work that boosts past time $0$ can also be upper bounded still by $V(\infty)$, so the bound of $W - B + V(\infty) + S$ is still valid. If $W < B$, we can still upper bound the response time by forcing the job to wait until time $B$. The job must then wait for jobs that have boosted arrival earlier than $0$, which can be upper bounded by $V(\infty)$. In this case $(W - B)^+ + V(\infty) + S$ is still an upper bound.
% \end{proof}

% \begin{definition}
%     \[
%         C_\pi &= \frac{1}{\gamma} \lim_{\theta\to\gamma} \gp{\gamma - \theta} \E*{\exp\gp{\theta T_\pi}}.
%     \]
% \end{definition}

% \begin{lemma}\label{lem:general_transform}
%     Suppose that the transform $\E*{\exp\gp{\gamma V(\infty)}}$ is finite. Then:
%     \[
%         C_\boost{} = C_\cheat{} = C_W \, \E*{\exp\gp*{\gamma \gp*{S - B}}} \, \E*{\exp\gp*{\gamma V(\infty)}}
%     \]
% \end{lemma}

% \begin{proof}
%     From \cref{lem:boost_response_time_bounds}, both $T_\boost{}$ and $T_\cheat{}$ can be lower and upper bounded, respectively, by $W - B + V(W) + S$ and $(W - B)^+ + S + V(\infty)$. This means that both $\E*{\exp\gp*{\theta T_\boost{}}}$ and $\E*{\exp\gp*{\theta T_\cheat{}}}$ fall within
%     \[
%         \sqgp[\Big]{\E*{\exp\gp[\big]{\theta \gp[\big]{W - B + V(W) + S}}}, \E*{\exp\gp[\big]{\theta \gp[\big]{(W - B)^+ + V(\infty) + S}}}}.
%     \]
%     Now it suffices to show that
%     \[
%         \liminf_{\theta\to\gamma}(\gamma - \theta) \E*{\exp\gp*{\theta \gp*{W - B + V(W) + S}}} &\geq C_\fcfs \frac{\E*{\exp\gp*{\gamma\gp*{S - B}}}\E*{\exp\gp*{\gamma V\gp{\infty}}}}{\E*{\exp\gp{\gamma S}}}\\
%         \limsup_{\theta\to\gamma} (\gamma - \theta) \E*{\exp\gp*{\theta \gp*{(W - B)^+ + V(\infty) + S}}} &\leq C_\fcfs \frac{\E*{\exp\gp*{\gamma\gp*{S - B}}}\E*{\exp\gp*{\gamma V\gp{\infty}}}}{\E*{\exp\gp{\gamma S}}}.
%     \]
    
%     For lower bound, consider arbitrary $u > 0$. For this $u$, we have
%     \[
%         \MoveEqLeft\liminf_{\theta\to\gamma}(\gamma - \theta) \E*{\exp\gp*{\theta \gp*{W - B + V(W) + S}}}\\
%         &\geq \liminf_{\theta\to\gamma}(\gamma - \theta) \E*{\exp\gp*{\theta \gp*{W - B + V(W) + S}}\1\gp{W > u}}\\
%         &\geq \liminf_{\theta\to\gamma}(\gamma - \theta) \E*{\exp\gp*{\theta \gp*{W - B + V(u) + S}}\1\gp{W > u}}\\
%         &= \liminf_{\theta\to\gamma} (\gamma - \theta) \E*{\exp\gp*{\theta W}\1\gp{W > u}}\E*{\exp\gp*{\theta \gp{S - B}}}\E*{\exp{\theta V(u)}}\\
%         &= C_W\E*{\exp\gp{\gamma\gp{S - B}}}\E*{\exp{\gamma V(u)}}.
%     \]
%     Since this holds for any $u$, it must hold for $C_W\E*{\exp\gp{\gamma\gp{S - B}}}\E*{\exp{\gamma V(\infty)}}$, as desired.
    
%     For the upper bound, observe that
%     \[
%         \MoveEqLeft\limsup_{\theta\to\gamma} (\gamma - \theta) \E*{\exp\gp*{\theta \gp*{(W - B)^+ + V(\infty) + S}}}\\
%         &\leq \limsup_{\theta\to\gamma} (\gamma - \theta) \E*{\gp*{\exp\gp*{\theta \gp{W - B}} + 1}\exp\gp*{\theta \gp{V(\infty) + S}}} \tag{$e^{x^+} \leq e^x + 1$.}\\
%         &= \limsup_{\theta\to\gamma} (\gamma - \theta) \gp*{\E*{\exp\gp*{\theta \gp{W - B + V(\infty) + S}}} + \E*{\exp\gp*{\theta\gp{V(\infty) + S}}}}.
%     \]
%     We analyze the first and second terms now. The first term is given by
%     \[
%         \MoveEqLeft\limsup_{\theta\to\gamma} (\gamma - \theta) \E*{\exp\gp*{\theta \gp{W - B + V(\infty) + S}}}\\
%         &= \limsup_{\theta\to\gamma} (\gamma - \theta) \E*{\exp\gp{\theta W}}\E*{\exp\gp{\theta\gp{S - B}}}\E*{\exp\gp{\theta V\gp{\infty}}}\\
%         &= C_W\E*{\exp\gp{\gamma\gp{S - B}}}\E*{\exp\gp{\gamma V(\infty)}}.
%     \]
%     The second term is given by
%     \[
%         \limsup_{\theta\to\gamma} (\gamma - \theta) \E*{\exp\gp*{\theta\gp{V(\infty) + S}}} &= 0,
%     \]
%     yielding the desired inequality.
% \end{proof}

% \subsection{Optimality}

% \begin{definition}
%     \[
%         C^* = \liminf_{\theta\to\gamma} \gp{\gamma - \theta} \E*{\exp\gp{\theta T_\cheat{\theta}}}
%     \]
% \end{definition}

% \begin{theorem}
%     \[
%         C^* = C_\boost{\gamma}.
%     \]
% \end{theorem}

% \begin{proof}
%     From \cref{lem:boost_response_time_bounds}, we know that $T_\cheat{\theta} \geq W - B_\theta + V_\theta(W) + S$. We can lower bound this further by $W - B_\theta + V_\gamma(W) + S$. This means that
%     \[
%         \E*{\exp\gp*{\theta T_\cheat{\theta}}} &\geq \E*{\exp\gp*{\theta \gp*{W - B_\theta + V_\gamma(W) + S}}}\\
%         &\geq \E*{\exp\gp*{\theta \gp*{W - B_\theta + V_\gamma(W) + S}}\1\gp*{W > u}}\\
%         &\geq \E*{\exp\gp*{\theta \gp*{W - B_\theta + V_\gamma(u) + S}}\1\gp*{W > u}}
%     \]
%     for arbitrary $u$. By independence of the $W, B_\theta, V_\gamma(u), S$, we can decompose the lower bound as
%     \[
%         \E*{\exp\gp*{\theta W}\1\gp*{W > u}}\E*{\exp\gp*{\theta \gp{S - B_\theta}}}\E*{e^{\theta V_\gamma(u)}}.
%     \]
%     For arbitrary $u$, since $B_\theta$ is monotonically decreasing in $\theta$, we can write
%     \[
%         \liminf_{\theta\to\gamma} (\gamma - \theta) \E*{\exp\gp*{\theta T_\cheat{\theta}}} &\geq \liminf_{\theta\to\gamma} (\gamma - \theta)\E*{\exp\gp*{\theta W}\1\gp*{W > u}}\E*{\exp\gp*{\theta \gp{S - B_\theta}}}\E*{e^{\theta V_\gamma(u)}}\\
%         &\geq C_W\E*{\exp\gp*{\gamma\gp*{S - B_\gamma}}}\E*{\exp\gp*{\gamma V_\gamma(u)}}
%     \]
%     and since the choice of $u$ is arbitrary, in particular it holds that
%     \[
%         \liminf_{\theta\to\gamma} (\gamma - \theta) \E*{\exp\gp*{\theta T_\cheat{\theta}}} &\geq C_W\E*{\exp\gp*{\gamma\gp*{S - B_\gamma}}}\E*{\exp\gp*{\gamma V_\gamma(\infty)}}.
%     \]
%     From \cref{lem:optimal_work_crossing_finite}, we know that $\E*{\exp\gp*{\gamma V_\gamma(\infty)}}$ is finite, and applying \cref{lem:general_transform} to \boost{\gamma} gives exactly this expression for $C_\boost{\gamma}$, so we are done.
% \end{proof}

% \begin{theorem}
%     Unless \boost{\gamma} assigns all labels (outside a set of measure zero) the same boost,
%     \[
%         C_\boost{\gamma} < C_\fcfs.
%     \]
% \end{theorem}

% \begin{proof}
%     The result of \cref{lem:general_transform,lem:optimal_work_crossing_finite} allows us to write \[
%         \frac{C_{\boost{\gamma}}}{C_{\fcfs}} \leq \frac{\E*{\exp\gp{\gamma \gp*{S - b_\gamma(L)}}} \frac{\lambda}{\gamma} \E{\exp\gp{\gamma S}} }{\E*{\exp\gp{\gamma S}}}.
%     \]
%     Recall that in \cref{lem:optimal_work_crossing_finite} the inequality arises from the use of Jensen's inequality, so that the inequality is strict unless the internal term is constant (i.e. $b_\boost{\gamma}(L)$ is constant across $L$).
    
%     Now consider the term $\E*{\exp\gp{\gamma \gp*{S - b_\gamma (L)}}}$. We have the following:
%     \[
%         \E*{\exp\gp{\gamma \gp*{S - b_\gamma(L)}}} &= \E*{\exp\gp{\gamma S} \exp\gp{-\gamma b_\gamma (L)}}\\
%         &= \E*{\exp\gp{\gamma S} \gp*{1 - \frac{1}{\E*{\exp\gp{\gamma S} \given L}}}}\\
%         &= \E*{ \E*{\exp\gp{\gamma S} \given L} \gp*{1 - \frac{1}{\E*{\exp\gp{\gamma S} \given L}}}} \tag{Tower rule.}\\
%         &= \frac{\gamma}{\lambda}.
%     \]
%     Plugging in for these two terms, we get that
%     \[
%         \frac{C_{\boost{\gamma}}}{C_{\fcfs}} \leq 1,
%     \]
%     with strict inequality unless the boost is constant across labels, as desired.
% \end{proof}



==> old/outlines/simulation_outline.tex <==
Ideas:
\* Policies to simulate
\** FCFS
\** SRPT
\** Nudge/Nudge-K
\*** Also maybe Nudge-(K,L) for some definition of that?
\** Boost
\*** Optimal boost function $r_\gamma$
\*** Slightly-off boost function $r_\beta$
\*** Generic boost function, e.g. $r(s) = 1/s$
\** Cheating
\* Questions to answer
\** How much better is optimal boost?
\** How robust to parameter?
\** Tradeoff between $\E{T_\pi}$ and $C_\pi$
\** Cheating???
\*/

Outline:
\* What is this section, and what questions will it answer?
\** Will list the questions below
\* What are the policies that appear in this section?
\** Just make clear which future subsections each policy appears in to help reader skip what they don't care about yet
\* How well does the optimal boost policy perform?
\** How much better than FCFS, Nudge, etc.?
\** How do practical tail ratios compare to asymptotic?
\** Any rule of thumb for the benefit of optimal boost?
\*** E.g. $T_{99}$ and above all decrease by some fixed amount, approximately
\** How does the distribution affect the benefit of boost policies?
\* How to make the decisions that go into the boost policy?
\** Parameter setting
\*** Compare robustness to inverse boost and/or Nudge-$k$?
\** Tradeoff between $\E{T_\pi}$ and $C_\pi$
\** Preemptive vs. nonpreemptive (vs. cheating?)
\* What about unknown sizes?
\** Size noise
\** Multiple classes with unknown sizes
\*/


==> old/outlines/tail_asymptotics_outline.tex <==
\* Expression for $\frac{C_\pi}{C_{FCFS}}$:
\** Lemma: $r(S) - A(r(S)) \to 0$ as $\theta\to\gamma$ for the tagged job.
\** For $\epsilon$-large jobs, $T_{FCFS} = W(-r_{\gamma - \epsilon}(S)) - r_{\gamma - \epsilon}(S) + A(r_{\gamma - \epsilon}(S)) + S = W(-r_{\gamma - \epsilon}(S)) + S$.
\** For $\epsilon$-large jobs, $T_r = W(-r_{\gamma - \epsilon}(S)) - r_{\gamma - \epsilon}(S) + S + V((-\infty, a - r(S)), (a - r_{\gamma - \epsilon}(S), D))$, where $D$ is the departure time of the tagged job $S$.
\*** $V(\cdots)$ is equivalent to all the arrivals in the gap $a - r_{\gamma - \epsilon}(S)$ to $a - r(S)$ (which is empty if $r(S)$ boosts ahead of $a - r_{\gamma - \epsilon}(S)$), plus the work-crossing until its departure, i.e. $V((-\infty, a - r(S)), (a - r(S), D))$.
\*** As $\theta\to\gamma$, the work in front of $S$ goes to $\infty$, so the departure time goes to $\infty$. Therefore $V((-\infty, a - r(S)), (a - r(S), D)) \to V((-\infty, a - r(S)), (a - r(S), \infty))$. \george{Do we need to be more formal than this?}
\** Lemma: Fix arbitrary $\epsilon > 0$. Then \[\lim_{\theta\to\gamma} (\gamma - \theta) \E{e^{\theta T_r} \1(\epsilon\text{-large})} = \lim_{\theta\to\gamma} (\gamma - \theta) \E{e^{\theta(W + S)} \1(\epsilon\text{-large})} \E{e^{\gamma WC(r)} \1(\epsilon\text{-large})} \E{e^{-\gamma r_{\gamma - \epsilon}(S)} \1(\epsilon\text{-large})} \]
\* Second lemma: 
\*/

==> old/preamble.tex <==
%%%%%%%%%%%%%%%%%% TUTORIAL %%%%%%%%%%%%%%%%%%


%%%%%% Easy equations

% \[eq\]: easy equations
% - Automatically chooses between equation, align, and gather
% - Only numbers lines that have a \label
% - If using \tag, put it right after \label, as in \label{...} \tag{...}


%%%%%% Easy lists

% \*: easy list macro, used as follows
%
% \* hello
% \* world
% \** use multiple * for sublists
% \** like this
% \* back to top level
% \* use a / to end the list
% \*/
%
% Can also use an optional argument to use numbers/letters, e.g.
%
% \*[(a)] labeled (a)
% \* labeled (b)
% \** no label in this sublist
% \* labeled (c)
% \**[(i)] labeled (i)
% \** labeled (ii)
% \*/
%
% More generally, use [] to pass any options the enumitem package supports.
%
% Optional feature: explicit start/end:
%
% - Explicit start: use \*[...], \**[...], etc. with no text after.
%   - Should be followed by another \*, \**, etc.
%   - This is mostly useful if you want to pass options in a separate line
% - Explicit end: use \**/, \***/, etc.
%   - This lets you have a sublist in the middle of an item
%
% Example:
%
% \*[(a), beginpenalty=10000]
% \* this is the first item, labeled (a)
% \** the list options got their own line
% \* this one is (b), and there's a sublist
% \**[beginpenalty=10000]
% \** with
% \** some
% \** stuff
% \**/ but now we resume item (b) from the outer list
% \* before finally going to (c)
% \*/


%%%%%% Delimiters with \gp, \sqgp, etc.

% All the delimiter commands work the same way. Using \gp as an example:
% - \gp{x} is normal parens around x
% - \gp*{x} automatically sizes the parens (like \left and \right would)
% - \gp[\big]{x} manually sizes the parens; \Big, \bigg, and \Bigg work, too
% See mathtools documentation for more details

% Delimiters defined:
% - \gp or \pgp: parentheses, ( . )
% - \sqgp or \bgp: square brackets, [ . ]
% - \curlgp or \Bgp: curly braces, { . }
% - \vgp: absolute value, | . |
% - \Vgp: norm, || . ||
% - \agp: angle brackets, < . >
% - \P: probability, P[ . ]
% - \E: expectation, E[ . ]
% - \Var: variance, Var[ . ]
% \P, \E, and \Var also support subscripts and superscripts before the */[\big]/etc.
% - Example: \P_x[\big]{...}
% Helpers:
% - \mid, \given: automatically resized divider |, works inside any of the above


%%%%%%%%%%%%%%%% END TUTORIAL %%%%%%%%%%%%%%%%


\usepackage[capitalize]{cleveref}
\usepackage[shortlabels]{enumitem}
\usepackage{etoolbox}
\usepackage{mathtools}
\usepackage{xifthen}
\usepackage{xparse}


\makeatletter


% cleveref settings

\crefname{equation}{\@gobble}{\@gobble}
\Crefname{equation}{Equation}{Equations}
\newcommand{\crefrangeconjunction}{--}
\newcommand{\creflastconjunction}{, and~}
% Let autonum know about \Cref.
% \autonum@generatePatchedReferenceCSL{Cref}
% Allow spaces between labels in \cref and \Cref.
% (This is an egreg stackexchange answer.)
\ExplSyntaxOn
\cs_set_eq:Nc \bers_cref:nn { @cref }
\cs_generate_variant:Nn \bers_cref:nn { nx }
\cs_set_protected:cpn { @cref } #1 #2
 {
  \seq_set_split:Nnn \l_bers_cref_seq { , } { #2 }
  \bers_cref:nx { #1 } { \seq_use:Nn \l_bers_cref_seq { , } }
 }
\seq_new:N \l_bers_cref_seq
\ExplSyntaxOff

\newcommand{\cCrefname}[3]{\crefname{#1}{#2}{#3}\Crefname{#1}{#2}{#3}}
\newcommand{\crefShorten}{%
  % \renewcommand{\crefpairconjunction}{, }
  % \renewcommand{\crefmiddleconjunction}{, }
  % \renewcommand{\creflastconjunction}{, }
  % \renewcommand{\crefpairgroupconjunction}{; }
  % \renewcommand{\crefmiddlegroupconjunction}{; }
  % \renewcommand{\creflastgroupconjunction}{; }
  \cCrefname{chapter}{Ch.}{Chs.}%
  \cCrefname{section}{\textsection}{\textsection\textsection}%
  \cCrefname{subsection}{\textsection}{\textsection\textsection}%
  \cCrefname{subsubsection}{\textsection}{\textsection\textsection}%
  \cCrefname{paragraph}{\textparagraph}{\textparagraph\textparagraph}%
  \cCrefname{subparagraph}{\textparagraph}{\textparagraph\textparagraph}%
  \cCrefname{appendix}{Appx.}{Appxs.}%
  \cCrefname{table}{Tab.}{Tabs.}%
  \cCrefname{figure}{Fig.}{Figs.}%
  \Crefname{equation}{Eq.}{Eqs.}%
  \cCrefname{theorem}{Thm.}{Thms.}%
  \cCrefname{lemma}{Lem.}{Lems.}%
  \cCrefname{proposition}{Prop.}{Props.}%
  \cCrefname{corollary}{Cor.}{Cors.}%
  \cCrefname{definition}{Def.}{Defs.}%
  \cCrefname{assumption}{Asm.}{Asms.}%
  \cCrefname{remark}{Rmk.}{Rmks.}%
}


% Easy lists with \*.
% Start list with \* (possibly with optional argument), end with \*/.
% Sublists with more stars, e.g. \***.
% Optional argument has one of two effects:
% - At beginning of a (sub)list, it sets the optional arguments for the list environment
%   - Using enumitem's shortlabels option, can do e.g. \*[1.] or \**[(a)] to enumerate sublists
% - For all itmes, it sets the optional argument for the \item
% - The first item in a (sub)list can have both optional arguments: first environment, then \item
\let\@oldstar\*
\newlist{easylist@env}{enumerate}{8}
\setlist[easylist@env,1]{label=\labelitemi}
\setlist[easylist@env,2]{label=\labelitemii}
\setlist[easylist@env,3]{label=\labelitemiii}
\setlist[easylist@env,4]{label=\labelitemiv}
\setlist[easylist@env,5]{label=\labelitemi}
\setlist[easylist@env,6]{label=\labelitemii}
\setlist[easylist@env,7]{label=\labelitemiii}
\setlist[easylist@env,8]{label=\labelitemiv}
\newcounter{easylist@prev}\setcounter{easylist@prev}{0}
\newcounter{easylist@this}\setcounter{easylist@this}{1}
\newcounter{easylist@diff}\setcounter{easylist@diff}{0}
\renewrobustcmd{\*}{\@ifstar{\easylist@star}{\easylist@nostar}}
\newcommand{\easylist@star}{\addtocounter{easylist@this}{1}\*}
\newcommand{\easylist@nostar}{%
  \def\easylist@type{{easylist@env}}%
  \ifthenelse{\value{easylist@this}>\value{easylist@prev}}{%
    \@ifnextchar{[}{\easylist@settype}{\easylist@checkend}%
  }{%
    \easylist@checkend%
  }
}
\def\easylist@settype[#1]{%
  \def\easylist@type{{easylist@env}[#1]}%
  \easylist@checkempty%
}
\newcommand{\easylist@checkempty}{%
  \@ifnextchar{\*}{%
    \easylist@go{}%
  }{%
    \easylist@go{\item}%
  }%
}
\newcommand{\easylist@checkend}{%
  \@ifnextchar{/}{%
    \ifthenelse{\value{easylist@this}>\value{easylist@prev}}{%
      \PackageError{prelude}{attempted to end easy list at too high a level}{}%
    }{}%
    \addtocounter{easylist@this}{-1}%
    \expandafter\easylist@go{}\@gobble%
  }{%
    \easylist@go{\item}%
  }%
}
\newcommand{\easylist@go}[1]{%
  \setcounter{easylist@diff}{\value{easylist@this}}%
  \addtocounter{easylist@diff}{-\value{easylist@prev}}%
  % I think I don't like this in the end....
  % \ifthenelse{\value{easylist@diff}>0 \AND \boolean{vmode}}{\leavevmode}{}%
  \whiledo{\value{easylist@diff}>1}{%
    \addtocounter{easylist@diff}{-1}%
    \begin{easylist@env}%
    \item
  }%
  \ifthenelse{\value{easylist@diff}=1}{%
    \addtocounter{easylist@diff}{-1}%
    \expandafter\begin\easylist@type%
  }{}%
  \whiledo{\value{easylist@diff}<0}{%
    \addtocounter{easylist@diff}{1}%
    \end{easylist@env}%
  }%
  \setcounter{easylist@prev}{\value{easylist@this}}%
  \setcounter{easylist@this}{1}%
  \ifthenelse{\value{easylist@prev}>0}{#1}{}%
}

% Compatibility with cleveref
\newcommand{\enumcCrefname}[1]{%
  \crefname{#1}{}{}
  \Crefname{#1}{Item}{Items}}

\enumcCrefname{easylist@envi}
\enumcCrefname{easylist@envii}
\enumcCrefname{easylist@enviii}
\enumcCrefname{easylist@enviv}
\enumcCrefname{easylist@envv}
\enumcCrefname{easylist@envvi}
\enumcCrefname{easylist@envvii}
\enumcCrefname{easylist@envviii}


% Easy equations with \[ and \]
% - Automatically chooses between equation, align, and gather
% - Automatically numbers only labeled equations
\def\[#1\]{%
  \begingroup%
  \let\cref@old@label@in@display\easyeq@label@in@display%
  \noexpandarg\IfSubStr{#1}{\allowdisplaybreaks}{\allowdisplaybreaks}{}%
  \noexpandarg\IfSubStr{#1}{&}{\begin{align*}#1\end{align*}}{%
    \noexpandarg\IfSubStr{#1}{\\}{\begin{gather*}#1\end{gather*}}{%
      \begin{equation*}#1\end{equation*}}}%
  \endgroup%
  \ignorespaces%
}
\AtBeginDocument{%
  \let\old@label@in@display\cref@old@label@in@display%
}
\def\easyeq@label@in@display#1{%
  \old@label@in@display{#1}%
  \@ifnextchar{\tag}{}{\yestag}%
}

% \yestag adds a number to just one line of an align* (or gather*, or even equation*).
% Used in easy equations.
% The \cref@currentlabel hackery makes this work with sort&compress in cleveref.
% See https://tex.stackexchange.com/questions/545726/labelcref-doesnt-like-my-user-defined-command.
\newcommand{\yestag@cref@format}{[equation][\arabic{equation}][\thesection]} % number in section
%\newcommand{\yestag@cref@format}{[equation][\theequation][]} % number globally
\newcommand*\yestag@make@df@tag@@[1]{%
  \cref@old@make@df@tag@@{#1}%
  \let\cref@old@df@tag\df@tag
  \expandafter\gdef\expandafter\df@tag\expandafter{%
    \cref@old@df@tag
    \def\cref@currentlabel{\yestag@cref@format#1}%
  }%
}
\newcommand*\yestag@make@df@tag@@@[1]{%
  \cref@old@make@df@tag@@@{#1}%
  \let\cref@old@df@tag\df@tag
  \expandafter\gdef\expandafter\df@tag\expandafter{%
    \cref@old@df@tag
    \toks@\@xp{\p@equation{#1}}%
    \edef\cref@currentlabel{\yestag@cref@format\the\toks@}%
  }%
}
\newcommand{\yestag}{%
  \refstepcounter{equation}%
  \begingroup%
    \let\make@df@tag@@\yestag@make@df@tag@@
    \let\make@df@tag@@@\yestag@make@df@tag@@@
  \tag{\theequation}%
  \endgroup%
}


% Delimiters

\newcommand{\mvert}{|}
\newcommand{\given}{\nonscript\;\mvert\nonscript\;\mathopen{}}
\renewcommand{\mid}{\given}
\newcommand{\resizegiven}{%
  \renewcommand{\given}{\nonscript\;\delimsize\mvert\nonscript\;\mathopen{}}}
% \gp or \pgp: group surrounded by parens
\DeclarePairedDelimiterX\gp[1](){\resizegiven #1}
\let\pgp\gp
% \sqgp or \bgp: like \gp, but with square brackets
\DeclarePairedDelimiterX\sqgp[1][]{\resizegiven #1}
\let\bgp\sqgp
% \curlgp or \Bgp: like \gp, but with curly braces
\DeclarePairedDelimiterX\curlgp[1]\{\}{\resizegiven #1}
\let\Bgp\curlgp
% \vgp: like \gp, but with vertical bars (e.g. for absolute value)
\DeclarePairedDelimiterX\vgp[1]\lvert\rvert{\resizegiven #1}
% \Vgp: like \gp, but with double vertical bars (e.g. for norms)
\DeclarePairedDelimiterX\Vgp[1]\lVert\rVert{\resizegiven #1}
% \agp: like \gp, but with angle brackets
\DeclarePairedDelimiterX\agp[1]\langle\rangle{\resizegiven #1}
% \floor and \ceil: like \gp, but floor and ceiling functions
\DeclarePairedDelimiterX\floor[1]\lfloor\rfloor{\resizegiven #1}
\DeclarePairedDelimiterX\ceil[1]\lceil\rceil{\resizegiven #1}


% x\afterScripts{y}_a^b -> x_a^b y
% Useful when y is one of \gp, \sqgp, etc.
\newcommand{\afterScripts}[1]{%
  \@ifnextchar_{\afterScripts@sub{#1}}{%
    \@ifnextchar^{\afterScripts@sup{#1}}{%
      #1}}}
\def\afterScripts@sub#1_#2{_{#2}\afterScripts{#1}}
\def\afterScripts@sup#1^#2{^{#2}\afterScripts{#1}}

\undef\P
\newrobustcmd{\P}{\mathbf{P}\afterScripts{\bgp}}
\newrobustcmd{\E}{\mathbf{E}\afterScripts{\bgp}}
\newcommand{\Var}{\mathbf{Var}\afterScripts{\bgp}}


\makeatother


==> old/tail_asymptotics.tex <==
\george{Adding work-crossing lemmas here for now.}
We begin with some lemmas for a quantity we call the work-crossing - the amount of work that boosts pasts a given time $t$. The lemmas below hold for any combination of open/closed intervals, so we omit brackets for clarity.

\begin{lemma}\label{lem:w1_wc_decomp}
    Let $V_r(a,b;c,d)$ be the work that has arrival time between $c$ and $d$ and has boosted arrival time between $a$ and $b$, given that the work boosts using boost function $r$. Suppose that $c < d' < d$ and $a < b' < b$. Then we have:
    \[
        V_r(a,b;c,d) = V_r(a,b';c,d) + V_r(b',b;c,d)\\
        V_r(a,b;c,d) = V_r(a,b;c,d') + V_r(a,b;d',d).
    \]
\end{lemma}

\begin{proof}
    The RHS of the first equality is simply the amount of work that arrives between $c, d$ that has boosted arrival time in $a, b'$ plus the amount of work that arrives between $c, d$ that has boosted arrival time in $b', b$. Since a job cannot boost both in between $a,b'$ and between $b',b$, this sums to the total amount of work that boosts between $a,b$.

    Similarly, the RHS of the second equality is the amount of work that arrives between $c,d'$ that boosts into $a,b$ plus the amount of work that arrives between $d', d$ that boosts into $a,b$. Since a job can only arrive in one of the two periods, this sums to the total amount of work between $c,d$ that boosts between $a,b$.
\end{proof}

\begin{lemma}\label{lem:w2_v_independence}
    Consider $V_r(a,b;c,d)$ and $V_r(a',b';c',d')$ s/t either $a,b$ and $a',b'$ are disjoint or $c,d$ and $c',d'$ are disjoint. Then $V_r(a,b;c,d) \perp V_r(a',b';c',d')$.
\end{lemma}

\begin{proof}
    Suppose a job $j$ arrives between $c,d$ and has boosted arrival time in $a,b$. $j$ cannot be captured in $a',b' \times c',d'$, because if it has boosted arrival time in $a',b'$, then $c,d$ and $c',d'$ must be disjoint by assumption, so $j$ does not arrive between $c',d'$. Similarly, if it arrives between $c',d'$, then by assumption it cannot have boosted arrival time in $a,b$. This means that we can construct independent increments of arrivals containing only jobs described by $V_r(a,b;c,d)$, and similarly for $V_r(a',b';c',d')$.
\end{proof}

\begin{lemma}\label{lem:w3_wc_poisson_splitting}
    \george{What's the right way to write this?}
    For any $t$, $V_r(-\infty, t; t, \infty)$ is distributed as the number of arrivals of a Poisson process with rate $\lambda df_L$ over time period $r(L)$, call this $X_r$.
\end{lemma}

\begin{proof}
    $V_r(-\infty, t;, t, \infty)$ is all the work that arrives after time $t$ and boosts in front of time $t$. This can be computed by considering the arrivals for each label $l$, and merging the arrival processes for all labels $l$. The arrival process for a label $l$ that crosses time $t$ is simply a Poisson process with rate $\lambda df_L(l)$ with time period $r(l)$, where arrivals have distribution $S_l$ given the label $l$.
\end{proof}

\george{Put the main result here first?}

In this section we derive a closed-form expression (\cref{lem:transform_ratio}) for the tail constant for any generic boost function. This allows us to easily compare the asymptotic performance for boost functions against FCFS or other policies. We then use this to prove \cref{thm:optimal_boost_ratio}, which shows that the optimal boost function has smaller asymptotic tail constant than FCFS. We start by proving the following lemma:

We start by proving the following work-crossing lemma, which gives an expression for the total amount of work that boosts pasts any time $t$.

\begin{lemma}\label{lem:work_crossing}
    % Let $V_r(B, A)$ be the amount of work that arrives in period $A$ that has boosted arrival time in period $B$, given the boost function $r$. Let the arrival rate be $\lambda$, and $\theta \leq \gamma$. Then
    % \[
    %     \E*{\exp\gp*{\theta V_r((-\infty, t), [t, \infty))}} = \exp\gp*{\lambda \E*{r(L)\gp*{\E*{e^{\theta S} \given L} - 1}}}.
    % \]
    \[
        \E*{\exp\gp*{\theta X_r}} = \exp\gp*{\lambda \E*{r(L)\gp*{\E*{e^{\theta S} \given L} - 1}}}.
    \]
\end{lemma}

\begin{proof}
    % We can compute the work-crossing by looking at arrivals with label $L$, and splitting across all labels. For a given label $L = l$, the amount of work that crosses time $t$ given boost function $r$ is given by the number of arrivals of a Poisson process with rate $\lambda f(l) dl$ and over time period $r(l)$. The arrivals have distribution $S \given l$.

    We can therefore compute the work-crossing transform by integrating over all $l$ for the merged Poisson process. In what follows below, let $\Delta l = b / n$. We have:
    \[
        \E*{\exp\gp*{\theta V_r(-\infty, t ; t, \infty)}} &= \E*{\lim_{b\to\infty} \lim_{n\to\infty} \exp\gp*{\sum_{i=1}^n \theta \gp*{S \given i\Delta l} \text{Pois}(\lambda f(i\Delta l), r(i\Delta l))}}\\
        &= \lim_{b\to\infty} \lim_{n\to\infty} \E*{\exp\gp*{\sum_{i=1}^n \theta \gp*{S \given i\Delta l} \text{Pois}(\lambda f(i\Delta l), r(i\Delta l))}} \tag{\george{Need to justify limit interchange here somehow?}}\\
        &= \lim_{b\to\infty} \lim_{n\to\infty} \prod_{i=1}^n \E*{\exp\gp*{\theta \gp*{S \given i\Delta l} \text{Pois}(\lambda f(i\Delta l), r(i\Delta l))}} \tag{By independence of the Poisson processes.}\\
        &= \lim_{b\to\infty} \lim_{n\to\infty} \prod_{i=1}^n \exp\gp*{\lambda f(i\Delta l) r(i\Delta l) \gp*{\E*{e^{\theta S} | i\Delta l} - 1}} \tag{Definition of the transform of a Poisson process.}\\
        &= \lim_{b\to\infty} \lim_{n\to\infty} \exp\gp*{\sum_{i=1}^n \lambda f(i\Delta l) r(i\Delta l) \gp*{\E*{e^{\theta S} | i\Delta l} - 1}}\\
        &= \exp\gp*{\int \lambda f(l) r(l) \gp*{\E*{e^{\theta S} \given l} - 1}dl}\\
        &= \exp\gp*{\lambda \E*{r(L) \gp*{\E*{e^{\theta S} \given L} - 1}}}.
    \]
\end{proof}

\begin{lemma}\label{lem:w5_finite_work_crossing}
    Consider the optimal boost function. We have:
    \[
        \lim_{u\to\infty} \E*{e^{\gamma V_r\gp*{-\infty, t; t,u}}} = \E*{e^{\gamma X_r}} < \infty.
    \]
\end{lemma}

\begin{proof}
    Observe that $e^{\gamma V_r \gp*{-\infty, t; t,u}}$ is monotonically increasing in $u$ since, for $u' < u$, all the work that arrives in $t,u$ that boosts into $-\infty, t$ includes all the work that arrives in $t,u'$ that boosts into $-\infty,t$. Moreover, by Monotone Convergence Theorem the LHS equals
    \[
        \E*{\lim_{u\to\infty} e^{\gamma V_r\gp*{-\infty, t; t,u}}} = \E*{e^{\gamma X_r}}.
    \]
    Now we will show that $\E*{e^{\gamma X_r}}$ is indeed finite for the optimal boost function $\boost{\gamma}$. Recall that $\frac{\lambda}{\gamma} = \frac{1}{\E*{e^{\gamma S} - 1}} = \frac{1}{\E*{\E*{e^{\gamma S} \given L}} - 1}$, and let $w(L) = \E*{e^{\gamma S} \given L}$ and $g(L) = w(L) - 1$. Substituting for $\lambda$, we get
    \[
        \exp\gp*{\E*{\frac{\gamma}{\E*{\E*{e^{\gamma S} \given L} - 1}} r_\boost{\gamma}(L) \gp*{\E*{e^{\gamma S} \given L} - 1}}}.
    \]
    Let $f_{L'}(l) = f(l)g(l)$ be the $L'$-weighted pdf, and observe that we can write the above as taking the expectation wrt $L'$, i.e.
    \[
        \exp\gp*{\E_{L'}*{\gamma r_\boost{\gamma}(L)}}.
    \]
    Applying Jensen's inequality, we have
    \[
        \exp\gp*{\E_{L'}*{\gamma r_\boost{\gamma}(L)}} &\leq \E_{L'}*{\exp\gp*{\log\gp*{\frac{1}{1 - \frac{1}{\E*{e^{\gamma S} | L}}}} }}\\
        &= \E_{L'}*{\gp*{\frac{1}{1 - \frac{1}{\E*{e^{\gamma S} | L}}}}}\\
        &= \E*{\frac{\E*{e^{\gamma S} \given L} - 1}{\E*{\E*{e^{\gamma S} \given L} - 1}} \gp*{\frac{1}{1 - \frac{1}{\E*{e^{\gamma S} | L}}}}}\\
        &= \frac{\E*{e^{\gamma S}}}{\E*{e^{\gamma S}} - 1}\\
        &= \frac{\lambda}{\gamma}\E*{e^{\gamma S}}.
    \]
    We know that $\E*{e^{\gamma S}}$ is finite, so we are done.
\end{proof}

% \begin{lemma}\label{lem:label_finite_work_crossing}
%     For boost functions of the form
%     \[
%         r_\boost{\beta}(L) = \frac{1}{\beta}\log\gp*{\frac{1}{1 - \frac{1}{\E*{e^{\beta S} | L}}}},
%     \]
%     with $\beta\in (\gamma/2, \gamma]$, and for any $\theta\in [\gamma/2,\gamma]$, the work-crossing exists (i.e. the expectation is finite).
% \end{lemma}

% \begin{proof}
%     It suffices to bound the expectation $\E*{r(L)\gp*{\E*{e^{\theta S} \given L} - 1}}$.

%     Consider first an arbitrary label $l$. If $\beta \leq \theta$, from \cref{lem:boost_convergence_in_param} we can derive an upper bound for $\E*{e^{\theta S} \given L}$:
%     \[
%         r_\beta(l) - r_\theta(l) &\leq \frac{r_\beta(l)}{\beta}(\theta - \beta)\\
%         r_\beta(l)\frac{2\beta - \theta}{\beta} &\leq r_\theta (l)\\
%         r_\beta(l)\frac{2\beta - \theta}{\beta} &\leq \frac{1}{\theta}\log\gp*{\frac{1}{1 - \frac{1}{\E*{e^{\theta S} \given l}}}}\\
%         e^{\theta r_\beta(l)\frac{2\beta - \theta}{\beta}} &\leq \frac{1}{1 - \frac{1}{\E*{e^{\theta S} \given l}}}\\
%         e^{-\theta r_\beta(l)\frac{2\beta - \theta}{\beta}} &\geq \frac{1}{1 - \frac{1}{\E*{e^{\theta S} \given l}}}\\
%         \frac{1}{\E*{e^{\theta S} \given l}} &\geq 1 - e^{-\theta r_\beta(l)\frac{2\beta - \theta}{\beta}}\\
%         \E*{e^{\theta S} \given l} &\leq \frac{1}{1 - e^{-\theta r_\beta(l) \frac{2\beta - \theta}{\beta}}}.
%     \]
%     Fix some $B > 0$, and decompose the desired expectation as:
%     \[
%         \E*{r_\beta(L) \gp*{\E*{e^{\theta S} \given L} - 1}} &= \E*{r_\beta(L) \gp*{\E*{e^{\theta S} \given L} - 1} \1\gp*{r_\beta(L) \leq B}} + \E*{r_\beta(L) \gp*{\E*{e^{\theta S} \given L} - 1} \1\gp*{r_\beta(L) > B}}.
%     \]
%     For the term $r_\beta(L) > B$, we observe that
%     \[
%         \E*{r_\beta(L) \gp*{\E*{e^{\theta S} \given L} - 1} \1\gp*{r(L) > B}} \leq \E*{r_\beta(L) \gp*{\frac{1}{1-e^{-\theta r_\beta(L) \frac{2\beta - \theta}{\beta}}} - 1} \1\gp*{r_\beta(L) > B}},
%     \]
%     and observe that $r_\beta(l) \gp*{\frac{1}{1-e^{-\theta r_\beta(l) \frac{2\beta - \theta}{\beta}}} - 1}$ is monotonically decreasing and goes to $0$ as $r_\beta(l) \to \infty$, if $\beta > \theta/2$. Therefore, it is bounded on the set $\1\gp*{r_\beta(L) > B}$, so the expectation is finite.
%     For the term $r_\beta(L) \leq B$, we have
%     \[
%         \E*{r_\beta(L) \gp*{\E*{e^{\theta S} \given L} - 1} \1\gp*{r_\beta(L) \leq B}} &\leq B\E*{\E*{e^{\theta S} \given L} - 1}\\
%         &\leq B \E*{e^{\theta S} - 1}\\
%         &\leq B \Tilde{S}(-\theta).
%     \]
%     Since the transform of $S$ is finite for Class~I distributions for any $\theta$, this term is also bounded.

%     Now consider the case that $\beta > \theta$. In this case we have:
%     \[
%         \E*{r_\beta(L) \gp*{\E*{e^{\theta S}\given L} - 1}} \leq \E*{r_\beta(L) \gp*{\E*{e^{\gamma S} \given L} - 1}},
%     \]
%     and we have reduced to the $\beta \leq \theta$ case.
% \end{proof}

% This is the known sizes version.

% \begin{lemma}\label{lem:finite_work_crossing}
%     \george{Adapt this to say that we can get a bound that works for arbitrary $\theta' < \gamma$, and that this bound is sufficient for all $\theta\in[\theta', \gamma]$, which is what we had in the notes. This is so we can } For boost functions of the form
%     \[
%         r_\boost{\beta}(L) = \frac{1}{\beta}\log\gp*{\frac{1}{1 - \frac{1}{\E*{e^{\beta S} | L}}}},
%     \] where $L$ is the job's size (i.e. the known-size case), the work-crossing exists (i.e. the expectation is finite).
% \end{lemma}

% \begin{proof}
%     Because $L$ is the job's size, the work-crossing can be written as
%     \[
%         \exp\gp*{\lambda \E*{r_\boost{\beta}(S) \gp*{e^{\theta S} - 1}}}.
%     \]
%     It suffices to show that the expectation $\E*{r_\boost{\beta}(S) \gp*{e^{\theta S} - 1}}$ is bounded. We will first show that $r_\boost{\beta}(s)\gp*{e^{\theta s} - 1} \to 0$ as $s\to 0$. We can write the product as
%     \[
%         \frac{r_\boost{\beta}(s)}{\frac{1}{e^{\theta s} - 1}}.
%     \]
%     Applying L'Hopital's rule, we observe that the ratio of the derivatives \george{Need to recalc this (incorrect) but still goes to 0.} is given by
%     \[
%         \frac{\frac{1}{1 - e^{\beta s}}}{\theta e^{\theta s}},
%     \]
%     where it can be seen as $s \to 0$ that the top goes to $0$ and the bottom goes to $1$.

%     We can decompose the expectation as follows:
%     \[
%         \E*{r_\boost{\beta}(S) \gp*{e^{\theta S} - 1}} = \E*{r_\boost{\beta}(S)\gp*{e^{\theta S} - 1} \1\gp*{S \leq B}} + \E*{r_\boost{\beta}(S)\gp*{e^{\theta S} - 1}\1\gp*{S > B}}.
%     \]
%     We have $\E*{r_\boost{\beta}(S)\gp*{e^{\theta S} - 1} \1\gp*{S \leq B}} \leq C$, since, by the above, the product $r_\boost{\beta}(s) \gp*{e^{\theta s} - 1}$ is bounded on some interval $s\in (0, B)$. \george{In particular, since $r_\boost{\beta}$ is decreasing in $\beta$, this interval should work for all $\beta' > \beta$, though I'm not sure if we need that here. Perhaps written as a corollary?} Observing that $r_\boost{\beta}$ is monotonically decreasing in $s$, we can bound the second term as follows:
%     \[
%         \E*{r_\boost{\beta}(S)\gp*{e^{\theta S} - 1}\1\gp*{S > B}} &\leq \E*{r_\boost{\beta}(S)e^{\theta S}\1\gp*{S > B}}\\
%         &\leq \E*{r_\boost{\beta}(B)e^{\theta S}}\\
%         &\leq r_\boost{\beta}(B)\E*{e^{\theta S}}.
%     \]
%     Since the transform of $S$ is finite for Class~I distributions for any $\theta$, this bounds the second term. Therefore, the expectation is bounded, so the work-crossing is bounded, as desired.
% \end{proof}

\begin{lemma}\label{lem:r>r_max}
    Consider a boost policy using boost function $r$, the response time under boost policy $r$ to be $T_r$, and some positive number $r_{max}$. Suppose that the work-crossing is finite. Then there is a constant $A > 0$ s/t:
    \[
        \lim_{\theta \to \gamma} (\gamma - \theta)\E*{e^{\theta T_r}\1(r(L) > r_{max})} \leq A \E*{e^{\theta S} \1\gp*{r(L) > r_{max}}},
    \]
    which goes to $0$ as $r_{max} \to \infty$.
\end{lemma}

\begin{proof}
    Observe that the response time of the job is upper bounded by the amount of work in the system at its arrival time, plus the job size, plus the work-crossing amount at the arrival time. That is, we can write
    \[
        T_r \leq W + S + V_r\gp*{(-\infty, 0), (0, \infty)},
    \]
    which implies
    \[
        \E*{e^{\theta T_r}\1\gp*{r > r_{max}}} &\leq \E*{e^{\theta \gp*{W + S + V_r\gp*{(-\infty, 0), (0, \infty)}}}\1\gp*{r(L) > r_{max}}}\\
        &\leq \E*{e^{\theta W}}\E*{e^{\theta S} \1\gp*{r(L) > r_{max}}} B \tag{By independence, and finiteness of work-crossing.}\\
    \]
    Observe that as $\theta\to\gamma$, the last line becomes
    \[
        \frac{C_\fcfs}{\E*{e^{\gamma S}}} B \E*{e^{\gamma S} \1\gp*{r(L) > r_{max}}},
    \]
    which is equivalent to
    \[
        \frac{C_\fcfs}{\E*{e^{\gamma S}}} B \E*{\E*{e^{\gamma S} \given r(L)} \1\gp*{r(L) > r_{max}}}.
    \]
    Since $\E*{e^{\gamma S}}$ is finite, this goes to $0$ as $r_{max} \to \infty$.
\end{proof}

% This is for the known sizes case.

% \begin{lemma}\label{lem:r>r_max}
%     Consider a boost policy using boost function $r$, the response time under boost policy $r$ to be $T_r$, and some positive number $r_{max}$. Suppose that the work-crossing is finite. Then there is a constant $A > 0$ s/t:
%     \[
%         \lim_{\theta \to \gamma} (\gamma - \theta)\E*{e^{\theta T_r}\1(r(L) > r_{max})} \leq A\P*{r(L) > r_{max}}.
%     \]
% \end{lemma}

% \george{Need to check whether the proof for this is correct + sufficiently formal.}
% \begin{proof}
%     Observe that the response time of the job is upper bounded by the amount of work in the system at its arrival time, plus the job size, plus the work-crossing amount at the arrival time. That is, we can write
%     \[
%         T_r \leq W + S + V_r\gp*{(-\infty, 0), (0, \infty)},
%     \]
%     which implies
%     \[
%         \E*{e^{\theta T_r}\1\gp*{r > r_{max}}} &\leq \E*{e^{\theta \gp*{W + S + V_r\gp*{(-\infty, 0), (0, \infty)}}}}\\
%         &\leq \E*{e^{\theta \gp*{W + S + V_r\gp*{(-\infty, 0), (0, \infty)}}} \given r > r_{max}}\P*{r > r_{max}}\\
%         &\leq \E*{e^{\theta W} \given r > r_{max}}\E*{e^{\theta S} \given r > r_{max}} B \P*{r > r_{max}} \tag{By independence, and finiteness of work-crossing.}\\
%         &\leq \E*{e^{\theta W}}\E*{e^{\theta S}}B \P*{r > r_{max}}.
%     \]
%     In the last line we can drop the condition for $W$ because it is independent of the boost applied to the job, and we observe that $\E*{e^{\theta S} \given r > r_{max}} \leq \E*{e^{\theta S}}$. \george{I think this statement is clearly true for monotonic boost functions but is harder to see for labels.} Multiplying by $(\gamma - \theta)$ and taking $\theta\to\gamma$ yields the upper bound
%     \[
%         C_\fcfs B \P*{r > r_{max}},
%     \]
%     as desired.
% \end{proof}

\begin{lemma}\label{lem:cheating_bounded}
    Let $W(-a)$ be the amount of work that arrives by time $a$ before the current time, and suppose that the work-crossing for $r$ is finite. \george{We need this because the work-crossing computation doesn't use the $r(L) \leq r_{max}$ condition (we have to sum up the work that can arrive over all possible boosts). Fundamentally it doesn't change the final result since the work-crossing is indeed finite for e.g. optimal boost.} Then there is a constant $B > 0$ s/t:
    \[
       \E*{e^{\theta T_r} \1\gp*{W(-r(L)) \leq r(L), r(L) \leq r_{max}}} \leq B.
    \]
\end{lemma}

\begin{proof}
    The response time $T_r$ can be upper bounded by the amount of work-crossing over time $-r(L)$ and the size of the job itself. Specifically, for any fixed $L = l$ we have $T_r \leq V_r((-\infty, -r(l)), (-r(l), \infty)) + S$. Let the condition $C_l = \{W(-r(l)) \leq r(l), r(l) \leq r_{max}\}$ This yields the following:
    \[
        \E*{\E*{e^{\theta T_r} \1\gp*{C_l} \given L = l}} &\leq \E*{\E*{e^{\theta \gp*{V_r((-\infty, -r(l)), (-r(l), \infty)) + S}} \given L = l, C_l}}\\
        &= \E*{\E*{e^{\theta S} \given L = l, C_l} \E*{e^{\theta V_r((-\infty, -r(l)), (-r(l), \infty))} \given L = l, C_l}}\\
        &= \E*{\E*{e^{\theta S} \given L = l, C_l} \E*{e^{\theta V_r((-\infty, -r(l)), (-r(l), \infty))}}}\\
        &\leq \Tilde{S}(-\theta)\exp\gp*{\lambda \E*{r(L) \gp*{\E*{e^{\theta S} | L}} - 1}}.
    \]
    The first term on the RHS is just the transform of the job size distribution, and the second term is just the work-crossing, which is bounded by assumption, so we are done.

    \george{If we use the condition $W(-r_{max}) \leq r_{max})$, then we get a bound that looks like $T_r \leq V_r((-\infty, -r(L)), [-r_{max}, \infty)) + S$, which translates to an upper bound that looks like $\frac{\Tilde{S}(-\theta)}{e^{\lambda r_{max}(1 - \Tilde{S}(-\theta))}}$ plus some work-crossing term. If it's sufficient to take $\theta\to\gamma$ for fixed $r_{max}$ then take $r_{max}\to\infty$ then this becomes $0$ due to the $(\gamma - \theta)$ term.}
\end{proof}

\begin{lemma}\label{lem:transform}
    Consider a boost policy with boost function $r$. Then:
    \[
        \lim_{\theta\to\gamma} (\gamma - \theta) \E*{e^{\theta T_r}} = C_\fcfs \frac{\E*{e^{\gamma \gp*{S - r(L)}}}e^{\lambda \E*{r(L) \gp*{\E*{e^{\gamma S} \given L} - 1}}}}{\E*{e^{\gamma S}}}.
    \]
    In particular, $(\gamma - \theta) \E*{e^{\theta T_r}} = (1 - o(1)) C_\fcfs \frac{\E*{e^{\gamma \gp*{S - r(L)}}}e^{\lambda \E*{r(L) \gp*{\E*{e^{\gamma S} \given L} - 1}}}}{\E*{e^{\gamma S}}}$.
\end{lemma}

\begin{proof}
    Observe that we can fix some $r_{max} > 0$ and decompose the expectation $\E*{e^{\theta T_r}}$ as follows:
    \[
        \E*{e^{\theta T_r}} &= \E*{e^{\theta T_r} \1\gp*{W(-r(L)) > r(L), r(L) \leq r_{max}}}\\
        &\; \; \; \; + \E*{e^{\theta T_r} \1\gp*{W(-r(L)) \leq r(L), r(L) \leq r_{max}}} + \E*{e^{\theta T_r}\1\gp*{r(L) > r_{max}}}\\
        &\leq \E*{e^{\theta T_r} \1\gp*{W(-r(L)) > r(L), r(L) \leq r_{max}}} + B + \E*{e^{\theta T_r}\1\gp*{r(L) > r_{max}}}. \tag{Apply \cref{lem:cheating_bounded}.}
    \]
    We focus on the first term and perform a tagged job analysis. In this case we can upper bound the response time for the job's arrival by $W(-r(L)) - r(L) + S + V_r((-\infty, -r(L)), (-r(L), \infty))$, where $W(-r(L)) - r(L) + V_r((-\infty -r(L)), (-r(L), 0))$ is all the work that arrives before the job which will be served before it, and $V_r((-\infty, -r(L)), (0, \infty))$ is an upper bound on the work that arrives after the job which will be served before it. The exact expression is $V_r((-\infty, -r(L)), (0, D))$, where $D$ is the departure time of the job. In particular, observe that as $\theta\to\gamma$, the work in front of time $-r(L)$ becomes infinite, so that the departure time goes to $\infty$ and the upper bound becomes tight. Letting $C_L = \{W(-r(L)) > r(L), r(L) \leq r_{max}\}$, Now we have:
    \[
        \MoveEqLeft\E*{e^{\theta \gp*{W(-r(L)) - r(L) + S + V_r((\infty, -r(L)), (-r(L), \infty))}} \1\gp*{C_L}}\\
        &= \E*{e^{\theta W(-r(L))}\given C_L}\E*{e^{\theta \gp*{S - r(L)}}\given C_L}\E*{e^{\theta V_r((\infty, -r(L)), (-r(L), \infty))} \given C_L}\P{C_L}\\
        &= \E*{e^{\theta W(-r(L))}\given C_L}\E*{e^{\theta \gp*{S - r(L)}} \given C_L}e^{\lambda \E*{r(L) \gp*{\E*{e^{\theta S} \given L} - 1}}}\P{C_L} \tag{\Cref{lem:work_crossing}, and independence of the work-crossing.}
    \]
    This means that
    \[
        \E*{e^{\theta T_r}} &\leq \E*{e^{\theta W(-r(L))}\given C_L}\P{C_L}\E*{e^{\theta \gp*{S - r(L)}} \given C_L}\P{C_L}e^{\lambda \E*{r(L) \gp*{\E*{e^{\theta S} \given L} - 1}}}\P{C_L}^{-1}\\
        &\; \; \; \; + B + \E*{e^{\theta T_r}\1\gp*{r(L) > r_{max}}}.
    \]
    We multiply both sides by $(\gamma - \theta)$ and take the limit $\theta\to\gamma$. Observe that this means $\P*{W(-r(L)) > r(L))} \to 1$. Then we have \george{Editing in progress for this set of limits.}:
    \[
        \P{C_L} &\to \P{r(L) \leq r_{max}}\\
        (\gamma - \theta)\E*{e^{\theta W(-r(L))} \given C_L}\P{C_L} &\to \frac{C_\fcfs}{\E*{e^{\gamma S}}}\\
        \E*{e^{\theta \gp*{S - r(L)}} \given C_L}\P{C_L} &\to \E*{e^{\gamma \gp*{S - r(L)}} \1\gp*{r(L) \leq r_{max}}}\\
        e^{\lambda \E*{r(L) \gp*{\E*{e^{\theta S} \given L} - 1}}} &\to e^{\lambda \E*{r(L) \gp*{\E*{e^{\gamma S} \given L} - 1}}}\\
        (\gamma - \theta)B &\to 0\\
        (\gamma - \theta)\E*{e^{\theta T_r}\1\gp*{r(L) > r_{max}}} &\leq B\E*{e^{\gamma T_r}\1\gp*{r(L) > r_{max}}}.
        % Using known sizes P(r > r_max) bound.
        % (\gamma - \theta)\E*{e^{\theta T_r}\1\gp*{r(L) > r_{max}}} &\leq A\P*{r(L) > r_{max}} \to 0.
    \]
    This yields
    \[
        \lim_{\theta\to\gamma} (\gamma - \theta) \E*{e^{\theta T_r}} = C_\fcfs \frac{\E*{e^{\gamma \gp*{S - r(L)}} \1\gp*{r(L) \leq r_{max}}}e^{\lambda \E*{r(L) \gp*{\E*{e^{\gamma S} \given L} - 1}}}}{\P{r(L) \leq r_{max}}\E*{e^{\gamma S}}} + B\E*{e^{\gamma T_r}\1\gp*{r(L) > r_{max}}},
    \]
    % Using known sizes P(r > r_max) bound.
    % \[
    %     \lim_{\theta\to\gamma} (\gamma - \theta) \E*{e^{\theta T_r}} = C_\fcfs \frac{\E*{e^{\gamma \gp*{S - r(L)}}}e^{\lambda \E*{r(L) \gp*{\E*{e^{\gamma S} \given L} - 1}}}}{\E*{e^{\gamma S}}} + A \P*{r(L) > r_{max}},
    % \]
    and since our choice of $r_{max}$ is arbitrary, we take $r_{max} \to \infty$ so that $\E*{e^{\gamma T_r}\1\gp*{r(L) > r_{max}}} \to 0$ and $\E*{e^{\gamma \gp*{S - r(L)}} \1\gp*{r(L) \leq r_{max}}} \to \E*{e^{\gamma \gp*{S - r(L)}}}$, and $\P{r(L) \leq r_{max}} \to 1$, yielding the desired result.
\end{proof}

% \begin{lemma}\label{lem:arrival_boost_cancellation}
%     Let $A(r(S))$ be the arrivals that occur in the time period of length $r(S)$. As $\theta\to\gamma$, $\E{e^{\theta \gp*{-r(S) + A\gp*{r(S)}}}} \to 1$.
% \end{lemma}

% \begin{proof}
%     The arrivals in a time period of $A(r(S))$ are Poisson distributed. The transform is therefore given by: \[\E{e^{\theta A(r(S))}} = e^{-\lambda r(S)\gp*{1 - \E{e^{\theta S}}}}.\]

%     Observe that $\Tilde{S}(-\theta) = \E{e^{\theta S}}$, and that $\gamma$ is defined as the value of $\theta$ s/t $\theta = -\lambda + \lambda \Tilde{S}(-\theta)$. Therefore as $\theta\to\gamma$, $e^{-\lambda r(S)\gp*{1 - \E{e^{\theta S}}}}$ becomes $e^{\gamma r(S)}$. Then, $\E{e^{\theta \gp*{-r(S) + A(r(S))}}}$ becomes
%     \[
%         \E{e^{-\theta r(S)}e^{\gamma r(S)}},
%     \]
%     which goes to $1$.
% \end{proof}

% With \cref{lem:arrival_boost_cancellation}, we can prove the following:

% \begin{lemma}\label{lem:transform_ratio}
%     For arbitrary $\epsilon > 0$, define the event $L = \{ \epsilon\text{-large}, W(-r_{\gamma - \epsilon}(S)) > r_{\gamma - \epsilon}(S) \}$, define $WC(r) = V((-\infty, a - r(S)), (a - r(S), \infty))$. Let $C_{r} = \frac{1}{\gamma}\lim_{\theta\to\gamma} (\gamma - \theta) \E*{ e^{\theta T_{r}}}$ and $C_{FCFS} = \frac{1}{\gamma}\lim_{\theta \to \gamma} (\gamma - \theta) \E*{e^{\theta T_{FCFS}}}$. Then:
%     \[
%         \label{eq:transform_ratio}
%         \frac{C_r}{C_{FCFS}} = \frac{\E*{e^{\gamma (S - r(S))}} e^{\lambda\E*{r(S)\gp*{e^{\gamma S} - 1}}}}{\E*{e^{\gamma S}}}
%     \]
% \end{lemma}

% \begin{proof}
%     Consider an arbitrary boost function $r$. The response time of a tagged job that is $\epsilon$-large with at least $W(-r_{\gamma - \epsilon}(S))$ work at time $-r_{\gamma - \epsilon}(S)$ before its arrival is given by 1) the amount of work from before $-r_{\gamma - \epsilon}(S)$ left at arrival time ($W(-r_{\gamma - \epsilon}(S)) - r_{\gamma - \epsilon}(S)$), 2) arrivals in the time period $-r_{\gamma - \epsilon}(S)$ to $-r(S)$, i.e. $A(r_{\gamma - \epsilon}(S) - r(S))$, 3) the job itself $S$ and 4) work that arrives after $S$ arrives and before it departs, and also boosts in front of it. Therefore the response time can be written as:
%     \[
%         T_r = W(-r_{\gamma - \epsilon}(S)) - r_{\gamma - \epsilon}(S) + A(r_{\gamma - \epsilon}(S) - r(S)) + S + V((-\infty, a - r(S)), (a - r(S), D)),
%     \]
%     where $D$ is the departure time of the job $S$. As $\theta\to\gamma$, the work in front of time $r_{\gamma - \epsilon}(S)$ before the arrival time of $S$ becomes infinite, so the departure time $D$ goes to infinity. (\george{Do we need a formal argument for this?}) Therefore, $V((-\infty, a - r(S)), (a - r(S), D)) \to WC(r)$. Using this decomposition of the response time, we can write $\lim_{\theta\to\gamma} (\gamma - \theta)\E*{e^{\theta T_r} \1(L)}$ as follows:
%     \[
%         \MoveEqLeft
%         \lim_{\theta\to\gamma} (\gamma - \theta) \E{e^{\theta (W(-r_{\gamma - \epsilon}(S)) - r_{\gamma - \epsilon}(S) + A(r_{\gamma - \epsilon}(S) - r(S)) + S + V((-\infty, a - r(S)), (a - r(S), D)))} \1(L)}\\
%         &= \lim_{\theta\to\gamma} (\gamma - \theta)\E{e^{\theta \gp*{W(-r_{\gamma - \epsilon}(S))+S}} e^{\theta \gp*{-r_{\gamma - \epsilon}(S) + A(r_{\gamma - \epsilon}(S) - r(S))}} e^{\theta V((-\infty, a - r(S)), (a - r(S), D))} \1(L)}\\
%         &\leq \lim_{\theta\to\gamma} (\gamma - \theta) \E{e^{\theta \gp*{W(-r_{\gamma - \epsilon}(S))+S}} e^{\theta \gp*{-r_{\gamma - \epsilon}(S) + A(r_{\gamma - \epsilon}(S) - r(S))}} e^{\theta WC(r)} \1(L)}\\
%         &= \lim_{\theta\to\gamma} (\gamma - \theta) \E{e^{\theta \gp*{W(-r_{\gamma - \epsilon}(S))+S}} e^{\theta \gp*{-r_{\gamma - \epsilon}(S) - r(S) + r(S) + A(r_{\gamma - \epsilon}(S) - r(S))}} e^{\theta WC(r)} \1(L)}\\
%         &= \E{e^{\gamma WC(r)} \1(L)} \lim_{\theta \to \gamma} (\gamma - \theta)\E{e^{\theta \gp*{W(-r_{\gamma - \epsilon}(S))}} e^{\theta \gp*{S - r(S) - r_{\gamma-\epsilon}(S) + r(S) A(r_{\gamma - \epsilon}(S) - r(S))}} \1(L)}.
%         % &= C_{FCFS}\E{e^{\gamma r(S)}} e^{\lambda\E*{r(S)\gp*{e^{\gamma S} - 1}}}.
%     \]

%     We make the following observations:
%     \* The choice of $\epsilon > 0$ was arbitrary.
%     \* As $\theta \to \gamma$, $W(-r_{\gamma - \epsilon}(S)) > r_{\gamma - \epsilon}(S)$ will hold a.s. for all $\epsilon$-large $S$, since $W(-r_{\gamma - \epsilon}(S)) \to \infty$.
%     \* Since $V\gp*{(-\infty, a - r(S)), (a - r(S), D)} \to WC(r)$ as $\theta\to\gamma$ the upper bound above becomes tight as $\theta \to \gamma$.
%     \* Taking the limit in the last line we can apply \cref{lem:arrival_boost_cancellation}. 
%     \*/

%     \george{This requires the work-crossing lemma, so we'll need to throw a ref in here once that's added.} Therefore we can write the last equation above as \[\frac{C_{FCFS}\E{e^{-\gamma (S - r(S))}} e^{\lambda \E*{r(S)\gp*{e^{\gamma S} - 1}}}}{\E{e^{\gamma S}}} .\]
    
%     This yields the ratio of the asymptotic coefficients as \[\frac{\E*{e^{\gamma (S - r(S))}} e^{\lambda\E*{r(S)\gp*{e^{\gamma S} - 1}}}}{\E*{e^{\gamma S}}} ,\]

%     as desired.
% \end{proof}

\Cref{lem:transform} provides us a way to quickly check the asymptotic performance of any generic boost function by numerically computing its tail ratio relative to FCFS. We use it here to prove the following theorem:

\begin{theorem}\label{thm:optimal_boost_ratio_labels}
    Let $C_{\boost{\gamma}} = \frac{1}{\gamma}\lim_{\theta \to \gamma} (\gamma - \theta) \E{e^{\theta T_{\boost{\gamma}}}}$, where $\boost{\gamma}$ is the optimal boost function given labels $L$ and $C_{\fcfs}$ be defined as in \cref{lem:transform}. Then
    \[
        \label{eq:opt_boost_ratio_improvement}
        \frac{C_{\boost{\gamma}}}{C_{\fcfs}} \leq 1.
    \]
\end{theorem}

\begin{proof}
    The result of \cref{lem:transform} allows us to write \[
        \frac{C_{\boost{\gamma}}}{C_{\fcfs}} = \frac{\E*{e^{\gamma \gp*{S - r_\gamma(L)}}} e^{\lambda \E*{r_\gamma(L) \gp*{\E*{e^{\gamma S} \given L} - 1}}} }{\E*{e^{\gamma S}}}.
    \]
    We first consider the work-crossing term. Recall that $\frac{\lambda}{\gamma} = \frac{1}{\E*{e^{\gamma S} - 1}} = \frac{1}{\E*{\E*{e^{\gamma S} \given L}} - 1}$, and let $w(L) = \E*{e^{\gamma S} \given L}$ and $g(L) = w(L) - 1$. Substituting for $\lambda$, we get
    \[
        \exp\gp*{\E*{\frac{\gamma}{\E*{\E*{e^{\gamma S} \given L} - 1}} r_\boost{\gamma}(L) \gp*{\E*{e^{\gamma S} \given L} - 1}}}.
    \]
    Let $f_{L'}(l) = f(l)g(l)$ be the $L'$-weighted pdf, and observe that we can write the above as taking the expectation wrt $L'$, i.e.
    \[
        \exp\gp*{\E_{L'}*{\gamma r_\boost{\gamma}(L)}}.
    \]
    Applying Jensen's inequality, we have
    \[
        \exp\gp*{\E_{L'}*{\gamma r_\boost{\gamma}(L)}} &\leq \E_{L'}*{\exp\gp*{\log\gp*{\frac{1}{1 - \frac{1}{\E*{e^{\gamma S} | L}}}} }}\\
        &= \E_{L'}*{\gp*{\frac{1}{1 - \frac{1}{\E*{e^{\gamma S} | L}}}}}\\
        &= \E*{\frac{\E*{e^{\gamma S} \given L} - 1}{\E*{\E*{e^{\gamma S} \given L} - 1}} \gp*{\frac{1}{1 - \frac{1}{\E*{e^{\gamma S} | L}}}}}\\
        &= \frac{\E*{e^{\gamma S}}}{\E*{e^{\gamma S}} - 1}\\
        &= \frac{\lambda}{\gamma}\E*{e^{\gamma S}}.
    \]
    Now we consider the term $\E*{e^{\gamma \gp*{S - r_\gamma (L)}}}$. We have the following:
    \[
        \E*{e^{\gamma \gp*{S - r_\gamma(L)}}} &= \E*{e^{\gamma S} e^{-\gamma r_\gamma (L)}}\\
        &= \E*{e^{\gamma S} \gp*{1 - \frac{1}{\E*{e^{\gamma S} \given L}}}}\\
        &= \E*{ \E*{e^{\gamma S} \given L} \gp*{1 - \frac{1}{\E*{e^{\gamma S} \given L}}}} \tag{Tower rule.}\\
        &= \frac{\gamma}{\lambda}.
    \]
    Plugging in for these two terms, we get that
    \[
        \frac{C_{\boost{\gamma}}}{C_{\fcfs}} \leq 1,
    \]
    as desired.
\end{proof}

% Known sizes version.

% \begin{theorem}\label{thm:optimal_boost_ratio}
%     Let $C_{\boost{\gamma}} = \frac{1}{\gamma}\lim_{\theta \to \gamma} (\gamma - \theta) \E{e^{\theta T_{\boost{\gamma}}}}$, where $\boost{\gamma}$ is the optimal boost function for known job sizes, and $C_{\fcfs}$ be defined as in \cref{lem:transform}. Then
%     \[
%         \label{eq:opt_boost_ratio_improvement}
%         \frac{C_{\boost{\gamma}}}{C_{\fcfs}} \leq 1.
%     \]
% \end{theorem}

% \begin{proof}
%     The result of \cref{lem:transform} allows us to write \[
%         \frac{C_{\boost{\gamma}}}{C_{\fcfs}} = \frac{\E*{e^{\gamma \gp*{S - r_\gamma(S)}}} e^{\lambda \E*{r_\gamma(S) \gp*{e^{\gamma S} - 1}}} }{\E*{e^{\gamma S}}}.
%     \]
%     Recalling the form of $r_\gamma(S) = \frac{1}{\gamma}\log\gp*{\frac{1}{1 - e^{-\gamma S}}}$, we have the following:
%     \[
%         \E*{e^{\gamma \gp*{S - r_\gamma(S)}}} &= \E*{e^{\gamma S} e^{-\log\gp*{\frac{1}{1 - e^{-\gamma S}}}}}\\
%         &= \E*{e^{\gamma S} e^{\log\gp*{1 - e^{-\gamma S}}}}\\
%         &= \E*{e^{\gamma S}\gp*{1 - e^{-\gamma S}}}\\
%         &= \E*{e^{\gamma S} - 1}\\
%         \label{eq:opt_boost_ratio_term_1}
%         &= \frac{\gamma}{\lambda},
%     \]
%     where we have used the definition of $\gamma$ in the last step. Next, we define $\E_\gamma{\cdot}$ as the expectation taken with respect to the pdf $f_\gamma(s) = \frac{e^{\gamma s} - 1}{\E*{e^{\gamma S} - 1}}f(s)$, where $f(s)$ is the pdf of $S$. This gives us the following:
%     \[
%         e^{\lambda \E*{r_\gamma(S) \gp*{e^{\gamma S} - 1}}} &= e^{\frac{\lambda}{\gamma}\E*{\gp*{e^{\gamma S} - 1} \log\gp*{\frac{1}{1 - e^{-\gamma S}}}}}\\
%         &= e^{\E_{\gamma}*{\log\gp*{\frac{1}{1 - e^{-\gamma S}}} }}\\
%         &\leq \E_{\gamma}*{\frac{1}{1 - e^{-\gamma S}}}\\
%         &= \frac{\lambda}{\gamma}\E*{\frac{e^{\gamma S} - 1}{1 - e^{-\gamma S}}}\\
%         \label{eq:opt_boost_ratio_term_2}
%         &= \frac{\lambda}{\gamma}\E*{e^{\gamma S}}.
%     \]
%     Plugging in \cref{eq:opt_boost_ratio_term_1} and \cref{eq:opt_boost_ratio_term_2} into \cref{lem:transform} yields:
%     \[
%         \frac{C_{\boost{\gamma}}}{C_{\fcfs}} &\leq \frac{\frac{\gamma}{\lambda} \frac{\lambda}{\gamma} \E*{e^{\gamma S}} }{\E*{e^{\gamma S}}}\\
%         &= 1,
%     \]
%     as desired.
% \end{proof}

\begin{corollary}\label{cor:finite_work_crossing_for_opt}
    For the optimal boost function
    \[
        r_{\boost{\gamma}}(L) = \frac{1}{\gamma}\log\gp*{\frac{1}{1 - \frac{1}{\E*{e^{\gamma S} \given L}}}},
    \]
    the work-crossing is upper bounded by $\frac{\lambda}{\gamma}\E*{e^{\gamma S}}$ and therefore finite.
\end{corollary}

\begin{proof}
    Following \cref{lem:work_crossing},
    \[
        \E*{\exp\gp*{\theta V_{r_{\boost{\gamma}}}\gp*{(-\infty, t), [t,\infty)}}} &= \exp\gp*{\lambda \E*{r_{\boost{\gamma}}(L) \gp*{\E*{e^{\theta S} \given L} - 1}}}\\
        &\leq \exp\gp*{\lambda \E*{r_{\boost{\gamma}}(L)} \gp*{\E*{e^{\gamma S} \given L} - 1}}\\
        &= \frac{\lambda}{\gamma}\E*{e^{\gamma S}}. \tag{By the proof of \cref{thm:optimal_boost_ratio_labels}.}
    \]
\end{proof}
